Deep Structural Estimation: With an Application to Option Pricing

We propose a novel structural estimation framework in which we train a surrogate of an economic model with deep neural networks. Our methodology alleviates the curse of dimensionality and speeds up the evaluation and parameter estimation by orders of magnitudes, which significantly enhances one's ability to conduct analyses that require frequent parameter re-estimation. As an empirical application, we compare two popular option pricing models (the Heston and the Bates model with double-exponential jumps) against a non-parametric random forest model. We document that: a) the Bates model produces better out-of-sample pricing on average, but both structural models fail to outperform random forest for large areas of the volatility surface; b) random forest is more competitive at short horizons (e.g., 1-day), for short-dated options (with less than 7 days to maturity), and on days with poor liquidity; c) both structural models outperform random forest in out-of-sample delta hedging; d) the Heston model's relative performance has deteriorated significantly after the 2008 financial crisis.

==> sec/intro_old.tex <==
%V1
%Motivated by empirical observations, contemporary economics and finance models use an ever-increasing set 
of endogenous and exogenous state variables as well as free parameters. This growing complexity produced great successes, with new models having better in-sample fit than their predecessors, and sometimes solving old academic puzzles. Economists tend to discuss these successes through a single estimation of the parameters and an in-sample analysis. This approach avoids estimating the models' parameters and states multiple times on multiple datasets which allows a comparative analysis of different models, a thorough out-of-sample analysis, and a discussion of the parameters' stability.  Indeed, repeated confrontations of the model to data may be infeasible as the computational cost of a calibration grows exponentially with the models' dimensionality. 


% V2
Motivated by empirical observations, contemporary models in economics, econometrics and finance use an ever-increasing set of endogenous and exogenous state variables as well as free parameters. 
This high level of level of sophistication turned out to be huge success: state-of-the-art models allow for instance substantially better in-sample fit than their predecessors, and sometimes even can answer long-standing open puzzles such as \fixmeAntoine{list them here}. 

\fixmeAntoine{This section should be twisted. First, say that estimation is often done only once because its expensive to do so. It is expensive to do so becaue of the curse of dim. Then you should say why it would be important to re-evaluate multiple times.}
To analyze those successes, researchers mostly rely on a single estimation of the parameters and in-sample analysis\fixmeAntoine{this sentence is is blurry and not proper English, what do we want to say? Analyze successes???}. This approach avoids the re-estimation of a particular model on multiple datasets necessary to a comparative analysis of different models, a thorough out-of-sample analysis, and a discussion of the parameters' stability. This partial analysis may be a necessity for complex structural models. Indeed, repeated confrontations of the model to data can be infeasible as the computational cost estimating parameters and states grows exponentially with a model's dimensionality. This limitation is problematic, as pure in-sample analysis in finance and economics can lead to false conclusions which do not generalize on new sample~\citep[see, e.g.,][]{10.1093/rfs/hhm014}. Thus, computational costs can seriously hinder economists' capacity to discuss, analyze, and compare structural models.


To resolve this issue, we introduce \textit{deep structural estimation}: A generic framework to calibrate and estimate structural models in economics and finance.
At its core, it re-purposes the concept of surrogate models that is commonly applied for instance in physics and engineering in the context of financial models.\footnote{The physics and engineering literature use Gaussian processes as surrogate models~\citep[see, e.g.,][]{williams2006gaussian,tripathy2016gaussian,bilionis2012multi,bilionis2013multi,chen2015uncertainty}, radial basis functions~\citep{park1991universal}, or relevance vector machines~\citep{bilionis2012multidimensional}. Recently, following the developments in optimization and artificial intelligence theory and advancements in computer hardware leading to the widespread availability of graphic processing units (GPUs)\footnote{For more details on how contemporary hardware can applied to problems in economics and finance, see~\citep[see, e.g.,][]{IPDPS2018,aldrich2011}, and references therein.}, researchers have turned their attention towards \textit{deep neural networks} \citep[see, e.g.,][]{tripathy2018deep,liu2019neural}.} 
We apply deep neural networks to create surrogates of financial or economics structural model---that is, a function that takes the same input as the original model and yields the same output at a significantly lower computational cost, thus alleviating the curse of dimensionality~\citep{Bellman1961AdaptiveTour}.

This paper demonstrates the usefulness \fixmeAntoine{this is to weak of a statement. Our paper's objective does not want to show only the usefulness of a method transferred from another science filed. We need to be more pronounced. Why would we otherwise ever get published a referee would ask himself. I would rather say: ADOPTING this techlology to the context of finance (implying that we need to work quite hard, a straight forward application is not possible) we can tackle issues not possible prior to our work.} of cheap-to-evaluate surrogate models in economics and finance by using deep neural  networks in context of state-of-the-art structural models of options pricing. \fixmeAntoine{here, we really should have a list of points. i), ii), iii). We should }


We show our surrogate's quality on simulated data by showing we can re-estimate the correct model's parameter from a simulated panel of options at significantly lower computational costs. 
We discuss the network's architecture and training procedure, which produces the best results, namely deep architectures---up to ten layers deep in combinations swish activation function\footnote{For details on the swish activation function, see~\cite{Ramachandran2017SwishAS}.}, and a low learning rate with the ADAM algorithm\fixmeAntoine{the low learning rate here needs a clarification; else, the last part needs to be removed because its non-scientific statement.}. 
Next, we show the benefit of our \textit{deep structural estimation} methodology by conducting a thorough analysis of multiple option pricing models---that is,\fixmeAntoine{list them here}. Finally, we discuss the novel insight produced by our analysis of the option pricing models' performance, and the deeper understanding of the economic mechanisms behind said performance or lack thereof. 
\fixmeAntoine{the above's paragraph should be more explicit what is novel in our analysis over the previous literature.}


We focus our attention on two option pricing models. The first is the Brownian motion with stochastic volatility, or Heston model (HM) \citep{heston1993closed}. The second is the Bate model with double jumps diffusion process (BDJ) \citep[][]{bates1996jumps,sepp2003pricing}. 
We can view both models as extensions of the first no-arbitrage pricing model for options, the Black-Scholes-Merton model (BSM) \citep{merton1973theory}. All three models assume that agents can perfectly replicate the options' payoff by re-balancing a portfolio of the underlying asset and a risk-free bond. The models only differ in their definition of the underlying asset's stochastic process. The HM replace the static volatility assumption of the BSM with stochastic volatility. The BDJ adds to the HM stochastic process Poisson distributed jump to the underlying asset's stochastic process. Both developments followed two empirical facts: 1) BSM's assumption of a smooth stochastic process with fixed volatility does not correspond to empirical realities. 2) the BSM fails to explain the cross-section of option prices. Indeed, the cross-section of option Black-Scholes implied volatility\footnote{The the literature defines the BSIV for a given option as the volatility values with which the BSM price prediction is equal to the market price.} (BSIV) produce a smile or a skew with in and out-of-the-money contracts having higher BSIVs than at-the-money options. 

The development of these pricing models and their capacity to best explain the cross-section of options' BSIV is considered one of financial theory great success. Perhaps surprisingly, despite these models' undeniable importance, market participants have not widely accepted them, and many sophisticated financial agents keep using the simpler BSM with ad-hoc tweaks and improvements \citep{berkowitz2009justifications}. This puzzling fact suggests that in-sample-performance and a model's capacity to resolve academic puzzles may not be sufficient to judge structural model performances. 
 
We investigate the out-of-sample performance of these asset pricing models through a process, common in the machine learning literature, called cross-validation \citep[see, e.g.,][]{10.5555/1162264}). It consists of estimating the model parameters on a sample and testing the performance on another, then repeating the operation multiple times on different training and testing samples. The literature suggests splitting the sample randomly with cross-sectional data, while with time-series, it may be preferable to move a fixed-size training window across time, testing the model on the data after the training set~\citep[see, e.g,][]{gu2018empirical}. This time series approach allows the researcher to simulate a real-time application of the model---that is, calibrating the model on available data and testing it on future observations. 

We use a panel of S\&P500 European options in the last 20 years to re-estimate the models' state and parameters daily, restricting the training sample to options BSIV on that particular day. First, we look at the time-series variation of the model parameters. We use the statistical method developed in \cite{andersen2015parametric} to test whether the models' parameters are statistically different from one day to the next. We reject the hypothesis that the parameters are drawn from the same distribution (TODO ADD STATS), and the rejection rate is larger for days at the end of the sample when the sample size is larger.\footnote{TODO: add a note on sample size across time}

Next, we look at the in and out-of-sample predicting power of the models. We wish to discuss the models against each other as well as a non-parametric benchmark. To do so, we use a random forest regressor. This relatively simple machine learning technique has the merit of both being computational cheap and requiring a minimum amount of tuning. We train a random forest on every day of the sample, restricting the models' input to the data used to calibrate the structural model. Therefore, both our non-parametric benchmarks and the two structural models: a) have access to the same information, b) try to minimize the same objective in-sample, and c) have the same performance measure in and out-of-sample.

In-sample, the random forest outperforms both models, while the structural model with more degrees of freedom (BDJ) outperforms the HM. As expected, the model's in-sample performance is directly related to the number of degrees of freedom. 

To discuss in depth the model's performance, we propose two definition of out-of-sample: \textit{state-blind}, and \textit{state-oracle}. In both versions, we estimate the model's parameter on a day $t$, and try to predict the options' cross-section at time $t+\tau$. In the \textit{state-blind} setting, we estimate the model states---that is, the risk-free rate and the current volatility level $v$---on day $t$, and we use the model's process and parameter to predict the expected values of the states at time $t+\tau$. In the \textit{state-oracle} set-up, we estimate the models' parameters at time $t$, but we take the state obtained by estimating the models' parameter and state at time $t+\tau$. Therefore, the \textit{state-blind} out-of-sample performance measures compare the cross-section at time $t+\tau$ to the models' prediction at time $t$, while the \textit{state-oracle} out-of-sample approach compares the market prices to the model's predictions conditional on knowing the states at time $t+\tau$. (TODO, maybe, add what both add in terms of information). For both cases, we look at a time-horizons $\tau$ ranging from 1 to 30. 

In the \textit{state-blind} case, the BDJ does outperform the HM for all values of $\tau$. However, the random-forest outperforms the BDJ and HM on a short time horizon, $\tau\in[1,2]$ but is outperformed by the BDJ for a longer time horizon. This perhaps surprising results (TODO add discussion)

Under the \textit{state-oracle} definition of out-of-sample, TODO: ADD DISCUSSION

TODO: add discussion on the range

TODO: then add the discussion with longer training range (when results here)

TODO: Add the discussion on DELTA reg (when here) 


Our paper's contribution to the literature is X-fold. First, we framework to re-purpose the surrogate technology in the context of financial and economic model: \textit{deep structural calibration}. We demonstrate this framework's viability with simulated data and discuss the best architecture and training procedure for surrogates of complex models. Our methodology makes possible a thorough analysis of complex structural models. In-sample analysis can be complemented by an out-of-sample analysis, which can provide additional insight into the models' performance.
Furthermore, we show how surrogate technology facilitates discussion of parameter stability. Indeed, with a cheaper cost, the model can be systematically re-estimated on multiple samples. This method allows the creation of a time-series of the model's estimated parameter, which we can then use to test the models' robustness. 



Second, we contribute to the option pricing literature by (TODO when results finalized)

Third, TODO, but probably a twist on providing an answer to the puzzling fact that market participants do not care for complex models. 

Fourth, TODO, but probably the discussion of the delta



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
The remainder of this article is organized as follows.
Section~\ref{sec:Literature} provides a brief overview of the related
literature. In Section~\ref{sec:methodology} explains the basic methodology.
In Section~\ref{sec:Result}, we apply our computational technology to two types of test cases: first, a controlled environment of simulated data. Second, to a panel of option data\fixmeAntoine{clarify}. 
Finally, Section~\ref{sec:Conclusion} concludes.



%To discuss the merit of a finance model, cross-validation presents two qualities which are typically lacking the in-sample analysis. First, since we estimate the model's parameters multiple times, the process produces a time-series of optimal model parameters. Most models rely on strong assumptions about parameter stability. Assumptions that we can test when we calibrate the model on multiple subsamples. 
%Second, by discussing performance out-of-sample, we can diminish the risk of overfitting. This concept, frequently used in the machine learning literature, captures phenomena where a model can precisely explain a particular dataset, but the model's performance does not generalize out-of-sample. In the context of structural models, such overfitting can occur with some parameter's value that overfits a specific pattern in the data or the model itself. Indeed when a model fails to explain a particular dataset, it is natural to attempt to improve the model by adding a set of parameters or states. In-sample, measures of fit will always increase with the models' degrees of freedom, but out-of-sample performance may decrease in case of overfitting. Reduced-form analysis solves this problem with strong statistical assumptions allowing economists to test rigorously any new parameters' explanatory power. 



==> table/bate_par_range.tex <==
\begin{tabular}{lrr}
\toprule
{} &  $\underline{x}^{(i)}$ &  $\bar{x}^{(i)}$ \\
$i$              &                        &                  \\
\midrule
strike           &                  60.00 &           140.00 \\
rf               &                   0.00 &             0.05 \\
T                &                   1.00 &           260.00 \\
kappa            &                   0.10 &             5.00 \\
theta            &                   0.05 &             0.70 \\
v0               &                   0.10 &             0.90 \\
sigma            &                   0.10 &             3.00 \\
rho              &                  -0.95 &            -0.00 \\
lambda_parameter &                   0.05 &             3.00 \\
nu               &                  -0.40 &             0.40 \\
delta            &                   0.05 &             0.60 \\
\bottomrule
\end{tabular}


==> table/bdjm_par_range <==
\begin{tabular}{lrr}
\toprule
{} &  $\underline{x}^{(j)}$ &  $\bar{x}^{(j)}$ \\
$j$       &                        &                  \\
\midrule
m         &                  -9.00 &            5.000 \\
$rf$      &                   0.00 &            0.075 \\
dividend  &                   0.00 &            0.050 \\
$v_t$     &                   0.01 &            0.900 \\
$T$       &                   1.00 &          365.000 \\
$\kappa$  &                   0.10 &           50.000 \\
$\theta$  &                   0.01 &            0.900 \\
$\sigma$  &                   0.10 &            5.000 \\
$\rho$    &                  -1.00 &           -0.000 \\
$\lambda$ &                   0.00 &            4.000 \\
$\nu_1$   &                   0.00 &            0.400 \\
$\nu_2$   &                   0.00 &            0.400 \\
p         &                   0.00 &            1.000 \\
\bottomrule
\end{tabular}


==> table/blind_oos_mean.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  HM. blind &  BDJM. blind &  RF. blind \\
\midrule
1  &    0.01649 &      0.01538 &    0.01497 \\
2  &    0.01889 &      0.01799 &    0.01853 \\
3  &    0.02057 &      0.01972 &    0.02077 \\
4  &    0.02187 &      0.02097 &    0.02212 \\
5  &    0.02300 &      0.02213 &    0.02323 \\
6  &    0.02395 &      0.02293 &    0.02451 \\
7  &    0.02478 &      0.02387 &    0.02561 \\
8  &    0.02545 &      0.02451 &    0.02638 \\
9  &    0.02605 &      0.02519 &    0.02746 \\
10 &    0.02674 &      0.02567 &    0.02905 \\
11 &    0.02753 &      0.02684 &    0.03006 \\
12 &    0.02824 &      0.02761 &    0.03124 \\
13 &    0.02883 &      0.02812 &    0.03212 \\
14 &    0.02932 &      0.02861 &    0.03260 \\
15 &    0.02981 &      0.02909 &    0.03284 \\
16 &    0.03025 &      0.02942 &    0.03327 \\
17 &    0.03065 &      0.02975 &    0.03349 \\
18 &    0.03097 &      0.03020 &    0.03352 \\
19 &    0.03130 &      0.03058 &    0.03344 \\
20 &    0.03177 &      0.03102 &    0.03356 \\
21 &    0.03223 &      0.03155 &    0.03425 \\
22 &    0.03258 &      0.03199 &    0.03452 \\
23 &    0.03294 &      0.03246 &    0.03463 \\
24 &    0.03336 &      0.03260 &    0.03466 \\
25 &    0.03379 &      0.03315 &    0.03512 \\
26 &    0.03421 &      0.03346 &    0.03568 \\
27 &    0.03464 &      0.03390 &    0.03614 \\
28 &    0.03507 &      0.03430 &    0.03670 \\
29 &    0.03549 &      0.03463 &    0.03744 \\
30 &    0.03585 &      0.03516 &    0.03821 \\
\bottomrule
\end{tabular}


==> table/blind_oos_q10.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  HM. blind &  BDJM. blind &  RF. blind \\
\midrule
1  &    0.00659 &      0.00565 &    0.00445 \\
2  &    0.00715 &      0.00626 &    0.00571 \\
3  &    0.00754 &      0.00663 &    0.00636 \\
4  &    0.00788 &      0.00679 &    0.00664 \\
5  &    0.00807 &      0.00712 &    0.00675 \\
6  &    0.00823 &      0.00723 &    0.00730 \\
7  &    0.00837 &      0.00755 &    0.00783 \\
8  &    0.00852 &      0.00761 &    0.00795 \\
9  &    0.00870 &      0.00773 &    0.00806 \\
10 &    0.00886 &      0.00795 &    0.00829 \\
11 &    0.00901 &      0.00827 &    0.00873 \\
12 &    0.00900 &      0.00818 &    0.00898 \\
13 &    0.00912 &      0.00823 &    0.00908 \\
14 &    0.00919 &      0.00824 &    0.00923 \\
15 &    0.00926 &      0.00830 &    0.00921 \\
16 &    0.00941 &      0.00842 &    0.00948 \\
17 &    0.00930 &      0.00833 &    0.00961 \\
18 &    0.00945 &      0.00841 &    0.00933 \\
19 &    0.00952 &      0.00861 &    0.00922 \\
20 &    0.00974 &      0.00861 &    0.00948 \\
21 &    0.00970 &      0.00878 &    0.00961 \\
22 &    0.00984 &      0.00902 &    0.00977 \\
23 &    0.00992 &      0.00907 &    0.00991 \\
24 &    0.01001 &      0.00924 &    0.00977 \\
25 &    0.00992 &      0.00923 &    0.00978 \\
26 &    0.01004 &      0.00933 &    0.01005 \\
27 &    0.01011 &      0.00942 &    0.01045 \\
28 &    0.00994 &      0.00935 &    0.01023 \\
29 &    0.01010 &      0.00958 &    0.01029 \\
30 &    0.01025 &      0.00969 &    0.01045 \\
\bottomrule
\end{tabular}


==> table/blind_oos_q50.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  HM. blind &  BDJM. blind &  RF. blind \\
\midrule
1  &    0.01203 &      0.01114 &    0.01008 \\
2  &    0.01365 &      0.01289 &    0.01292 \\
3  &    0.01485 &      0.01402 &    0.01473 \\
4  &    0.01570 &      0.01505 &    0.01566 \\
5  &    0.01649 &      0.01608 &    0.01632 \\
6  &    0.01700 &      0.01671 &    0.01733 \\
7  &    0.01753 &      0.01699 &    0.01830 \\
8  &    0.01800 &      0.01756 &    0.01861 \\
9  &    0.01848 &      0.01804 &    0.01930 \\
10 &    0.01918 &      0.01867 &    0.02037 \\
11 &    0.01998 &      0.01969 &    0.02108 \\
12 &    0.02032 &      0.02001 &    0.02205 \\
13 &    0.02063 &      0.02033 &    0.02286 \\
14 &    0.02077 &      0.02073 &    0.02280 \\
15 &    0.02128 &      0.02089 &    0.02298 \\
16 &    0.02131 &      0.02124 &    0.02341 \\
17 &    0.02138 &      0.02129 &    0.02359 \\
18 &    0.02156 &      0.02154 &    0.02342 \\
19 &    0.02183 &      0.02176 &    0.02334 \\
20 &    0.02217 &      0.02172 &    0.02354 \\
21 &    0.02237 &      0.02197 &    0.02388 \\
22 &    0.02276 &      0.02239 &    0.02399 \\
23 &    0.02282 &      0.02227 &    0.02401 \\
24 &    0.02318 &      0.02270 &    0.02401 \\
25 &    0.02348 &      0.02283 &    0.02429 \\
26 &    0.02352 &      0.02304 &    0.02480 \\
27 &    0.02404 &      0.02349 &    0.02517 \\
28 &    0.02441 &      0.02393 &    0.02556 \\
29 &    0.02446 &      0.02402 &    0.02593 \\
30 &    0.02455 &      0.02420 &    0.02620 \\
\bottomrule
\end{tabular}


==> table/blind_oos_q90.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  HM. blind &  BDJM. blind &  RF. blind \\
\midrule
1  &    0.02914 &      0.02774 &    0.02875 \\
2  &    0.03440 &      0.03356 &    0.03572 \\
3  &    0.03783 &      0.03777 &    0.03959 \\
4  &    0.04103 &      0.04030 &    0.04286 \\
5  &    0.04274 &      0.04204 &    0.04512 \\
6  &    0.04535 &      0.04471 &    0.04791 \\
7  &    0.04695 &      0.04608 &    0.04979 \\
8  &    0.04808 &      0.04759 &    0.05087 \\
9  &    0.04975 &      0.04957 &    0.05282 \\
10 &    0.05152 &      0.05051 &    0.05720 \\
11 &    0.05260 &      0.05189 &    0.05968 \\
12 &    0.05333 &      0.05355 &    0.06115 \\
13 &    0.05454 &      0.05424 &    0.06205 \\
14 &    0.05621 &      0.05523 &    0.06336 \\
15 &    0.05741 &      0.05629 &    0.06412 \\
16 &    0.05911 &      0.05794 &    0.06591 \\
17 &    0.06018 &      0.05828 &    0.06676 \\
18 &    0.06038 &      0.05902 &    0.06607 \\
19 &    0.06184 &      0.05989 &    0.06646 \\
20 &    0.06280 &      0.06133 &    0.06619 \\
21 &    0.06316 &      0.06143 &    0.06769 \\
22 &    0.06447 &      0.06412 &    0.06832 \\
23 &    0.06460 &      0.06398 &    0.06892 \\
24 &    0.06629 &      0.06505 &    0.06928 \\
25 &    0.06726 &      0.06663 &    0.06952 \\
26 &    0.06877 &      0.06751 &    0.07173 \\
27 &    0.07070 &      0.06904 &    0.07261 \\
28 &    0.07136 &      0.06982 &    0.07418 \\
29 &    0.07270 &      0.07115 &    0.07536 \\
30 &    0.07378 &      0.07299 &    0.07829 \\
\bottomrule
\end{tabular}


==> table/blind_oos_q95.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  HM. blind &  BDJM. blind &  RF. blind \\
\midrule
1  &    0.08023 &      0.07592 &    0.08211 \\
2  &    0.09035 &      0.09190 &    0.09417 \\
3  &    0.09920 &      0.09701 &    0.10536 \\
4  &    0.10619 &      0.10362 &    0.11031 \\
5  &    0.11082 &      0.10332 &    0.11848 \\
6  &    0.11471 &      0.10701 &    0.12366 \\
7  &    0.11881 &      0.10895 &    0.12535 \\
8  &    0.12363 &      0.11742 &    0.12598 \\
9  &    0.12419 &      0.11918 &    0.14410 \\
10 &    0.13028 &      0.11767 &    0.14764 \\
11 &    0.13173 &      0.12393 &    0.15295 \\
12 &    0.13803 &      0.13214 &    0.16283 \\
13 &    0.14159 &      0.13509 &    0.16246 \\
14 &    0.14539 &      0.14343 &    0.16649 \\
15 &    0.14528 &      0.13886 &    0.16936 \\
16 &    0.14673 &      0.14280 &    0.17197 \\
17 &    0.15286 &      0.14548 &    0.17111 \\
18 &    0.15801 &      0.15168 &    0.17824 \\
19 &    0.16423 &      0.15293 &    0.18055 \\
20 &    0.16528 &      0.15465 &    0.17873 \\
21 &    0.16940 &      0.16704 &    0.17513 \\
22 &    0.17055 &      0.16441 &    0.17990 \\
23 &    0.16993 &      0.16837 &    0.17904 \\
24 &    0.16991 &      0.16505 &    0.18019 \\
25 &    0.16906 &      0.16322 &    0.17738 \\
26 &    0.17482 &      0.16176 &    0.17842 \\
27 &    0.17379 &      0.16258 &    0.18079 \\
28 &    0.16828 &      0.16194 &    0.17744 \\
29 &    0.17262 &      0.16769 &    0.18607 \\
30 &    0.17750 &      0.18037 &    0.19084 \\
\bottomrule
\end{tabular}


==> table/lag_reg_hbL1.tex <==
\begin{tabular}{lccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &     \phantom{*}0.494*** &    \phantom{*}0.3956*** &    \phantom{*}0.3748*** &    \phantom{*}0.3652*** &    \phantom{*}0.3596*** \\
             &     (0.0112)\phantom{*} &    (0.0127)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &    \phantom{*}0.1987*** &    \phantom{*}0.1571*** &    \phantom{*}0.1429*** &    \phantom{*}0.1387*** \\
             &                         &    (0.0127)\phantom{**} &    (0.0136)\phantom{**} &    (0.0137)\phantom{**} &    (0.0137)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.1046*** &    \phantom{*}0.0705*** &    \phantom{*}0.0619*** \\
             &                         &                         &    (0.0128)\phantom{**} &    (0.0137)\phantom{**} &    (0.0138)\phantom{**}\smallskip \\
$y_{t-4}$    &                         &                         &                         &    \phantom{*}0.0912*** &    \phantom{*}0.0691*** \\
             &                         &                         &                         &    (0.0129)\phantom{**} &    (0.0137)\phantom{**}\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &    \phantom{*}0.0606*** \\
             &                         &                         &                         &                         &    (0.0129)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes \\
CD           &                 98.4131 &                 138.329 &                 143.378 &                 145.319 &                 145.898 \\
\medskip\\
Observations &                   6,021 &                   6,019 &                   6,016 &                   6,012 &                   6,007 \\
$R^2$        &                  0.5287 &                  0.5473 &                  0.5522 &                  0.5559 &                  0.5574 \\
\bottomrule
\end{tabular}


==> table/lag_reg_hbL30.tex <==
\begin{tabular}{lccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &    \phantom{*}0.5834*** &    \phantom{*}0.4879*** &    \phantom{*}0.4745*** &    \phantom{*}0.4701*** &          \phantom{*}0.4664*** \\
             &    (0.0105)\phantom{**} &    (0.0128)\phantom{**} &    (0.0129)\phantom{**} &    (0.013)\phantom{***} &          (0.013)\phantom{***}\smallskip \\
$y_{t-2}$    &                         &     \phantom{*}0.164*** &    \phantom{*}0.1249*** &    \phantom{*}0.1181*** &          \phantom{*}0.1145*** \\
             &                         &     (0.0128)\phantom{*} &    (0.0142)\phantom{**} &    (0.0143)\phantom{**} &          (0.0143)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.0806*** &    \phantom{*}0.0545*** &          \phantom{*}0.0466*** \\
             &                         &                         &    (0.0129)\phantom{**} &    (0.0143)\phantom{**} &          (0.0144)\phantom{**}\smallskip \\
$y_{t-4}$    &                         &                         &                         &    \phantom{*}0.0548*** &  \phantom{*}0.0232\phantom{*} \\
             &                         &                         &                         &    (0.013)\phantom{***} &                      (0.0143)\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &          \phantom{*}0.0674*** \\
             &                         &                         &                         &                         &          (0.013)\phantom{***} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                           Yes \\
CD           &                 80.5765 &                 124.747 &                 132.506 &                 135.711 &                       137.098 \\
\medskip\\
Observations &                   5,965 &                   5,963 &                   5,960 &                   5,956 &                         5,951 \\
$R^2$        &                  0.4199 &                  0.4354 &                  0.4389 &                  0.4404 &                        0.4428 \\
\bottomrule
\end{tabular}


==> table/lag_reg_hbL5.tex <==
\begin{tabular}{lccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &    \phantom{*}0.4688*** &    \phantom{*}0.4131*** &    \phantom{*}0.4045*** &    \phantom{*}0.3998*** &    \phantom{*}0.3937*** \\
             &    (0.0114)\phantom{**} &    (0.0128)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &    \phantom{*}0.1189*** &    \phantom{*}0.0894*** &    \phantom{*}0.0833*** &      \phantom{*}0.08*** \\
             &                         &    (0.0128)\phantom{**} &    (0.0139)\phantom{**} &    (0.0139)\phantom{**} &                (0.0139)\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.0715*** &    \phantom{*}0.0442*** &     \phantom{*}0.037*** \\
             &                         &                         &    (0.0129)\phantom{**} &    (0.0139)\phantom{**} &     (0.0139)\phantom{*}\smallskip \\
$y_{t-4}$    &                         &                         &                         &    \phantom{*}0.0676*** &     \phantom{*}0.0327** \\
             &                         &                         &                         &    (0.0129)\phantom{**} &     (0.0139)\phantom{*}\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &    \phantom{*}0.0876*** \\
             &                         &                         &                         &                         &    (0.0129)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes \\
CD           &                 93.5054 &                 128.144 &                 135.502 &                 138.945 &                 140.324 \\
\medskip\\
Observations &                   6,012 &                   6,010 &                   6,007 &                   6,003 &                   5,998 \\
$R^2$        &                  0.4053 &                  0.4135 &                  0.4164 &                   0.419 &                  0.4235 \\
\bottomrule
\end{tabular}


==> table/lag_reg_obL1.tex <==
\begin{tabular}{lccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} &       \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &               -0.249*** &              -0.2609*** &              -0.2611*** &                    -0.2611*** &                    -0.2618*** \\
             &     (0.0125)\phantom{*} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &          (0.0129)\phantom{**} &          (0.0129)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &               -0.048*** &              -0.0486*** &                    -0.0481*** &                    -0.0481*** \\
             &                         &     (0.0129)\phantom{*} &    (0.0133)\phantom{**} &          (0.0134)\phantom{**} &          (0.0133)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &      -0.0022\phantom{*} &  \phantom{*}0.0003\phantom{*} &  \phantom{*}0.0031\phantom{*} \\
             &                         &                         &                (0.0129) &                      (0.0134) &                      (0.0134)\smallskip \\
$y_{t-4}$    &                         &                         &                         &             \phantom{*}0.0101 &            \phantom{*}0.0249* \\
             &                         &                         &                         &                       (0.013) &                      (0.0134)\smallskip \\
$y_{t-5}$    &                         &                         &                         &                               &          \phantom{*}0.0571*** \\
             &                         &                         &                         &                               &          (0.0129)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                           Yes &                           Yes \\
CD           &                 44.0862 &                 50.8611 &                 54.4218 &                       56.2808 &                       57.2613 \\
\medskip\\
Observations &                   6,021 &                   6,019 &                   6,016 &                         6,012 &                         6,007 \\
$R^2$        &                  0.0978 &                  0.0997 &                  0.0994 &                        0.0992 &                        0.1021 \\
\bottomrule
\end{tabular}


==> table/lag_reg_obL30.tex <==
\begin{tabular}{lccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &    \phantom{*}0.7538*** &    \phantom{*}0.6834*** &    \phantom{*}0.6799*** &     \phantom{*}0.682*** &    \phantom{*}0.6802*** \\
             &    (0.0085)\phantom{**} &    (0.0129)\phantom{**} &    (0.013)\phantom{***} &     (0.013)\phantom{**} &    (0.013)\phantom{***}\smallskip \\
$y_{t-2}$    &                         &    \phantom{*}0.0935*** &    \phantom{*}0.0682*** &    \phantom{*}0.0717*** &     \phantom{*}0.074*** \\
             &                         &    (0.0129)\phantom{**} &    (0.0157)\phantom{**} &    (0.0157)\phantom{**} &     (0.0157)\phantom{*}\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.0372*** &    \phantom{*}0.0734*** &    \phantom{*}0.0757*** \\
             &                         &                         &    (0.013)\phantom{***} &    (0.0157)\phantom{**} &    (0.0157)\phantom{**}\smallskip \\
$y_{t-4}$    &                         &                         &                         &              -0.0534*** &               -0.0321** \\
             &                         &                         &                         &    (0.013)\phantom{***} &     (0.0157)\phantom{*}\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &               -0.0314** \\
             &                         &                         &                         &                         &     (0.013)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes \\
CD           &                 8.21062 &                 16.5301 &                 18.5439 &                 19.3449 &                 19.9107 \\
\medskip\\
Observations &                   5,965 &                   5,963 &                   5,960 &                   5,956 &                   5,951 \\
$R^2$        &                  0.5685 &                  0.5722 &                  0.5727 &                  0.5739 &                  0.5742 \\
\bottomrule
\end{tabular}


==> table/lag_reg_obL5.tex <==
\begin{tabular}{lccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &    \phantom{*}0.1679*** &    \phantom{*}0.1885*** &    \phantom{*}0.1704*** &    \phantom{*}0.1472*** &    \phantom{*}0.1573*** \\
             &    (0.0127)\phantom{**} &    (0.0128)\phantom{**} &    (0.0128)\phantom{**} &    (0.0128)\phantom{**} &    (0.0129)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &              -0.1233*** &              -0.0956*** &              -0.1107*** &              -0.1029*** \\
             &                         &    (0.0128)\phantom{**} &    (0.0129)\phantom{**} &    (0.0128)\phantom{**} &    (0.0129)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &               -0.147*** &                -0.12*** &              -0.1129*** \\
             &                         &                         &     (0.0128)\phantom{*} &                (0.0128) &    (0.0129)\phantom{**}\smallskip \\
$y_{t-4}$    &                         &                         &                         &              -0.1581*** &              -0.1676*** \\
             &                         &                         &                         &    (0.0128)\phantom{**} &    (0.0129)\phantom{**}\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &    \phantom{*}0.0647*** \\
             &                         &                         &                         &                         &    (0.0129)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes \\
CD           &                 16.3345 &                 17.9059 &                  19.353 &                  19.617 &                 20.0191 \\
\medskip\\
Observations &                   6,012 &                   6,010 &                   6,007 &                   6,003 &                   5,998 \\
$R^2$        &                  0.0287 &                  0.0433 &                  0.0638 &                  0.0871 &                  0.0908 \\
\bottomrule
\end{tabular}


==> table/lag_reg_panel_1.tex <==
\begin{tabular}{lccccc}
\toprule \multicolumn{6}{c}{\parboxc{c}{0.7cm}{Panel A: $y_t = (\sqrt{MSE_{DBJM}}-\sqrt{MSE_{HM}})$}} \\\hline
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &     \phantom{*}0.494*** &    \phantom{*}0.3956*** &    \phantom{*}0.3748*** &    \phantom{*}0.3652*** &    \phantom{*}0.3596*** \\
             &     (0.0112)\phantom{*} &    (0.0127)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &    \phantom{*}0.1987*** &    \phantom{*}0.1571*** &    \phantom{*}0.1429*** &    \phantom{*}0.1387*** \\
             &                         &    (0.0127)\phantom{**} &    (0.0136)\phantom{**} &    (0.0137)\phantom{**} &    (0.0137)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.1046*** &    \phantom{*}0.0705*** &    \phantom{*}0.0619*** \\
             &                         &                         &    (0.0128)\phantom{**} &    (0.0137)\phantom{**} &    (0.0138)\phantom{**}\smallskip \\
$y_{t-4}$    &                         &                         &                         &    \phantom{*}0.0912*** &    \phantom{*}0.0691*** \\
             &                         &                         &                         &    (0.0129)\phantom{**} &    (0.0137)\phantom{**}\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &    \phantom{*}0.0606*** \\
             &                         &                         &                         &                         &    (0.0129)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes \\
CD           &                 98.4131 &                 138.329 &                 143.378 &                 145.319 &                 145.898 \\
\medskip\\
Observations &                   6,021 &                   6,019 &                   6,016 &                   6,012 &                   6,007 \\
$R^2$        &                  0.5287 &                  0.5473 &                  0.5522 &                  0.5559 &                  0.5574 \bigskip \\ 


\hline \multicolumn{6}{c}{\parboxc{c}{0.6cm}{Panel B: $y_t = (\sqrt{MSE_{DBJM}}-\sqrt{MSE_{RF}})$}} \\\hline
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} &       \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &               -0.249*** &              -0.2609*** &              -0.2611*** &                    -0.2611*** &                    -0.2618*** \\
             &     (0.0125)\phantom{*} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &          (0.0129)\phantom{**} &          (0.0129)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &               -0.048*** &              -0.0486*** &                    -0.0481*** &                    -0.0481*** \\
             &                         &     (0.0129)\phantom{*} &    (0.0133)\phantom{**} &          (0.0134)\phantom{**} &          (0.0133)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &      -0.0022\phantom{*} &  \phantom{*}0.0003\phantom{*} &  \phantom{*}0.0031\phantom{*} \\
             &                         &                         &                (0.0129) &                      (0.0134) &                      (0.0134)\smallskip \\
$y_{t-4}$    &                         &                         &                         &             \phantom{*}0.0101 &            \phantom{*}0.0249* \\
             &                         &                         &                         &                       (0.013) &                      (0.0134)\smallskip \\
$y_{t-5}$    &                         &                         &                         &                               &          \phantom{*}0.0571*** \\
             &                         &                         &                         &                               &          (0.0129)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                           Yes &                           Yes \\
CD           &                 44.0862 &                 50.8611 &                 54.4218 &                       56.2808 &                       57.2613 \\
\medskip\\
Observations &                   6,021 &                   6,019 &                   6,016 &                         6,012 &                         6,007 \\
$R^2$        &                  0.0978 &                  0.0997 &                  0.0994 &                        0.0992 &                        0.1021 \\
\bottomrule
\end{tabular}


==> table/lag_reg_panel_30.tex <==
\begin{tabular}{lccccc}
\toprule \multicolumn{6}{c}{\parboxc{c}{0.7cm}{Panel A: $y_t = (\sqrt{MSE_{DBJM}}-\sqrt{MSE_{HM}})$}} \\\hline
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &    \phantom{*}0.5834*** &    \phantom{*}0.4879*** &    \phantom{*}0.4745*** &    \phantom{*}0.4701*** &          \phantom{*}0.4664*** \\
             &    (0.0105)\phantom{**} &    (0.0128)\phantom{**} &    (0.0129)\phantom{**} &    (0.013)\phantom{***} &          (0.013)\phantom{***}\smallskip \\
$y_{t-2}$    &                         &     \phantom{*}0.164*** &    \phantom{*}0.1249*** &    \phantom{*}0.1181*** &          \phantom{*}0.1145*** \\
             &                         &     (0.0128)\phantom{*} &    (0.0142)\phantom{**} &    (0.0143)\phantom{**} &          (0.0143)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.0806*** &    \phantom{*}0.0545*** &          \phantom{*}0.0466*** \\
             &                         &                         &    (0.0129)\phantom{**} &    (0.0143)\phantom{**} &          (0.0144)\phantom{**}\smallskip \\
$y_{t-4}$    &                         &                         &                         &    \phantom{*}0.0548*** &  \phantom{*}0.0232\phantom{*} \\
             &                         &                         &                         &    (0.013)\phantom{***} &                      (0.0143)\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &          \phantom{*}0.0674*** \\
             &                         &                         &                         &                         &          (0.013)\phantom{***} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                           Yes \\
CD           &                 80.5765 &                 124.747 &                 132.506 &                 135.711 &                       137.098 \\
\medskip\\
Observations &                   5,965 &                   5,963 &                   5,960 &                   5,956 &                         5,951 \\
$R^2$        &                  0.4199 &                  0.4354 &                  0.4389 &                  0.4404 &                        0.4428 \bigskip \\ 


\hline \multicolumn{6}{c}{\parboxc{c}{0.6cm}{Panel B: $y_t = (\sqrt{MSE_{DBJM}}-\sqrt{MSE_{RF}})$}} \\\hline
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &    \phantom{*}0.7538*** &    \phantom{*}0.6834*** &    \phantom{*}0.6799*** &     \phantom{*}0.682*** &    \phantom{*}0.6802*** \\
             &    (0.0085)\phantom{**} &    (0.0129)\phantom{**} &    (0.013)\phantom{***} &     (0.013)\phantom{**} &    (0.013)\phantom{***}\smallskip \\
$y_{t-2}$    &                         &    \phantom{*}0.0935*** &    \phantom{*}0.0682*** &    \phantom{*}0.0717*** &     \phantom{*}0.074*** \\
             &                         &    (0.0129)\phantom{**} &    (0.0157)\phantom{**} &    (0.0157)\phantom{**} &     (0.0157)\phantom{*}\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.0372*** &    \phantom{*}0.0734*** &    \phantom{*}0.0757*** \\
             &                         &                         &    (0.013)\phantom{***} &    (0.0157)\phantom{**} &    (0.0157)\phantom{**}\smallskip \\
$y_{t-4}$    &                         &                         &                         &              -0.0534*** &               -0.0321** \\
             &                         &                         &                         &    (0.013)\phantom{***} &     (0.0157)\phantom{*}\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &               -0.0314** \\
             &                         &                         &                         &                         &     (0.013)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes \\
CD           &                 8.21062 &                 16.5301 &                 18.5439 &                 19.3449 &                 19.9107 \\
\medskip\\
Observations &                   5,965 &                   5,963 &                   5,960 &                   5,956 &                   5,951 \\
$R^2$        &                  0.5685 &                  0.5722 &                  0.5727 &                  0.5739 &                  0.5742 \\
\bottomrule
\end{tabular}


==> table/lag_reg_panel_5.tex <==
\begin{tabular}{lccccc}
\toprule \multicolumn{6}{c}{\parboxc{c}{0.7cm}{Panel A: $y_t = (\sqrt{MSE_{DBJM}}-\sqrt{MSE_{HM}})$}} \\\hline
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &    \phantom{*}0.4688*** &    \phantom{*}0.4131*** &    \phantom{*}0.4045*** &    \phantom{*}0.3998*** &    \phantom{*}0.3937*** \\
             &    (0.0114)\phantom{**} &    (0.0128)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &    \phantom{*}0.1189*** &    \phantom{*}0.0894*** &    \phantom{*}0.0833*** &      \phantom{*}0.08*** \\
             &                         &    (0.0128)\phantom{**} &    (0.0139)\phantom{**} &    (0.0139)\phantom{**} &                (0.0139)\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.0715*** &    \phantom{*}0.0442*** &     \phantom{*}0.037*** \\
             &                         &                         &    (0.0129)\phantom{**} &    (0.0139)\phantom{**} &     (0.0139)\phantom{*}\smallskip \\
$y_{t-4}$    &                         &                         &                         &    \phantom{*}0.0676*** &     \phantom{*}0.0327** \\
             &                         &                         &                         &    (0.0129)\phantom{**} &     (0.0139)\phantom{*}\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &    \phantom{*}0.0876*** \\
             &                         &                         &                         &                         &    (0.0129)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes \\
CD           &                 93.5054 &                 128.144 &                 135.502 &                 138.945 &                 140.324 \\
\medskip\\
Observations &                   6,012 &                   6,010 &                   6,007 &                   6,003 &                   5,998 \\
$R^2$        &                  0.4053 &                  0.4135 &                  0.4164 &                   0.419 &                  0.4235 \bigskip \\ 


\hline \multicolumn{6}{c}{\parboxc{c}{0.6cm}{Panel B: $y_t = (\sqrt{MSE_{DBJM}}-\sqrt{MSE_{RF}})$}} \\\hline
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} \\
\midrule
$y_{t-1}$    &    \phantom{*}0.1679*** &    \phantom{*}0.1885*** &    \phantom{*}0.1704*** &    \phantom{*}0.1472*** &    \phantom{*}0.1573*** \\
             &    (0.0127)\phantom{**} &    (0.0128)\phantom{**} &    (0.0128)\phantom{**} &    (0.0128)\phantom{**} &    (0.0129)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &              -0.1233*** &              -0.0956*** &              -0.1107*** &              -0.1029*** \\
             &                         &    (0.0128)\phantom{**} &    (0.0129)\phantom{**} &    (0.0128)\phantom{**} &    (0.0129)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &               -0.147*** &                -0.12*** &              -0.1129*** \\
             &                         &                         &     (0.0128)\phantom{*} &                (0.0128) &    (0.0129)\phantom{**}\smallskip \\
$y_{t-4}$    &                         &                         &                         &              -0.1581*** &              -0.1676*** \\
             &                         &                         &                         &    (0.0128)\phantom{**} &    (0.0129)\phantom{**}\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &    \phantom{*}0.0647*** \\
             &                         &                         &                         &                         &    (0.0129)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes \\
CD           &                 16.3345 &                 17.9059 &                  19.353 &                  19.617 &                 20.0191 \\
\medskip\\
Observations &                   6,012 &                   6,010 &                   6,007 &                   6,003 &                   5,998 \\
$R^2$        &                  0.0287 &                  0.0433 &                  0.0638 &                  0.0871 &                  0.0908 \\
\bottomrule
\end{tabular}


==> table/oracle/lag_reg_hbL1.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
$y_{t-100}$  &                         &                         &                         &                         &                         &                         &            -0.0116\phantom{*} \\
             &                         &                         &                         &                         &                         &                         &                      (0.0127)\smallskip \\
$y_{t-1}$    &    \phantom{*}0.2056*** &    \phantom{*}0.1878*** &    \phantom{*}0.1809*** &    \phantom{*}0.1761*** &    \phantom{*}0.1741*** &    \phantom{*}0.1721*** &          \phantom{*}0.1731*** \\
             &    (0.0126)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &          (0.013)\phantom{***}\smallskip \\
$y_{t-2}$    &                         &     \phantom{*}0.086*** &    \phantom{*}0.0709*** &    \phantom{*}0.0666*** &    \phantom{*}0.0643*** &     \phantom{*}0.061*** &          \phantom{*}0.0622*** \\
             &                         &     (0.0129)\phantom{*} &    (0.0131)\phantom{**} &    (0.0131)\phantom{**} &    (0.0131)\phantom{**} &     (0.0131)\phantom{*} &          (0.0132)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.0799*** &    \phantom{*}0.0687*** &    \phantom{*}0.0664*** &    \phantom{*}0.0623*** &          \phantom{*}0.0607*** \\
             &                         &                         &    (0.013)\phantom{***} &    (0.0132)\phantom{**} &    (0.0132)\phantom{**} &    (0.0132)\phantom{**} &          (0.0133)\phantom{**}\smallskip \\
$y_{t-4}$    &                         &                         &                         &    \phantom{*}0.0609*** &    \phantom{*}0.0549*** &    \phantom{*}0.0509*** &          \phantom{*}0.0513*** \\
             &                         &                         &                         &    (0.013)\phantom{***} &    (0.0132)\phantom{**} &    (0.0132)\phantom{**} &          (0.0133)\phantom{**}\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &     \phantom{*}0.0334** &      \phantom{*}0.0225* &  \phantom{*}0.022*\phantom{*} \\
             &                         &                         &                         &                         &     (0.013)\phantom{**} &                (0.0132) &                      (0.0133)\smallskip \\
$y_{t-6}$    &                         &                         &                         &                         &                         &    \phantom{*}0.0617*** &          \phantom{*}0.0616*** \\
             &                         &                         &                         &                         &                         &    (0.013)\phantom{***} &          (0.0131)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes &                           Yes \\
\medskip\\
Observations &                   6,021 &                   6,019 &                   6,016 &                   6,012 &                   6,007 &                   6,001 &                         5,901 \\
$R^2$        &                  0.1893 &                  0.1952 &                  0.2001 &                  0.2029 &                  0.2035 &                  0.2063 &                        0.2104 \\
\bottomrule
\end{tabular}


==> table/oracle/lag_reg_hbL30.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} &       \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} &       \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
$y_{t-100}$  &                         &                         &                         &                               &                               &                               &            -0.011\phantom{**} \\
             &                         &                         &                         &                               &                               &                               &                      (0.0107)\smallskip \\
$y_{t-1}$    &    \phantom{*}0.5344*** &    \phantom{*}0.3966*** &    \phantom{*}0.3885*** &          \phantom{*}0.3877*** &          \phantom{*}0.3872*** &           \phantom{*}0.387*** &           \phantom{*}0.388*** \\
             &    (0.0109)\phantom{**} &    (0.0125)\phantom{**} &    (0.0129)\phantom{**} &          (0.013)\phantom{***} &          (0.013)\phantom{***} &           (0.013)\phantom{**} &           (0.0131)\phantom{*}\smallskip \\
$y_{t-2}$    &                         &    \phantom{*}0.2581*** &    \phantom{*}0.2457*** &          \phantom{*}0.2395*** &          \phantom{*}0.2392*** &           \phantom{*}0.239*** &          \phantom{*}0.2393*** \\
             &                         &    (0.0125)\phantom{**} &    (0.0135)\phantom{**} &          (0.0139)\phantom{**} &          (0.0139)\phantom{**} &           (0.0139)\phantom{*} &          (0.014)\phantom{***}\smallskip \\
$y_{t-3}$    &                         &                         &     \phantom{*}0.0315** &  \phantom{*}0.0218\phantom{*} &  \phantom{*}0.0176\phantom{*} &  \phantom{*}0.0174\phantom{*} &  \phantom{*}0.0165\phantom{*} \\
             &                         &                         &     (0.013)\phantom{**} &                      (0.0139) &                      (0.0142) &                      (0.0143) &                      (0.0144)\smallskip \\
$y_{t-4}$    &                         &                         &                         &            \phantom{*}0.0251* &  \phantom{*}0.0183\phantom{*} &  \phantom{*}0.0156\phantom{*} &  \phantom{*}0.0153\phantom{*} \\
             &                         &                         &                         &            (0.013)\phantom{*} &                      (0.0139) &                      (0.0143) &                      (0.0144)\smallskip \\
$y_{t-5}$    &                         &                         &                         &                               &             \phantom{*}0.0176 &  \phantom{*}0.0132\phantom{*} &   \phantom{*}0.014\phantom{*} \\
             &                         &                         &                         &                               &                       (0.013) &                      (0.0139) &                       (0.014)\smallskip \\
$y_{t-6}$    &                         &                         &                         &                               &                               &             \phantom{*}0.0113 &  \phantom{*}0.0113\phantom{*} \\
             &                         &                         &                         &                               &                               &                       (0.013) &                      (0.0131) \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                           Yes &                           Yes &                           Yes &                           Yes \\
\medskip\\
Observations &                   5,992 &                   5,990 &                   5,987 &                         5,983 &                         5,978 &                         5,972 &                         5,872 \\
$R^2$        &                  0.3423 &                   0.386 &                  0.3865 &                        0.3867 &                        0.3868 &                        0.3867 &                        0.3885 \\
\bottomrule
\end{tabular}


==> table/oracle/lag_reg_hbL5.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} &       \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
$y_{t-100}$  &                         &                         &                         &                         &                               &                               &            -0.0037\phantom{*} \\
             &                         &                         &                         &                         &                               &                               &                      (0.0119)\smallskip \\
$y_{t-1}$    &    \phantom{*}0.3934*** &    \phantom{*}0.3432*** &    \phantom{*}0.3351*** &    \phantom{*}0.3325*** &          \phantom{*}0.3285*** &          \phantom{*}0.3272*** &          \phantom{*}0.3285*** \\
             &    (0.0119)\phantom{**} &    (0.0128)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &          (0.0129)\phantom{**} &          (0.0129)\phantom{**} &          (0.0131)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &    \phantom{*}0.1275*** &    \phantom{*}0.1058*** &    \phantom{*}0.1015*** &          \phantom{*}0.0967*** &          \phantom{*}0.0966*** &          \phantom{*}0.0975*** \\
             &                         &    (0.0128)\phantom{**} &    (0.0135)\phantom{**} &    (0.0136)\phantom{**} &          (0.0136)\phantom{**} &          (0.0136)\phantom{**} &          (0.0137)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.0633*** &    \phantom{*}0.0493*** &          \phantom{*}0.0393*** &          \phantom{*}0.0388*** &          \phantom{*}0.0379*** \\
             &                         &                         &    (0.0129)\phantom{**} &    (0.0136)\phantom{**} &          (0.0137)\phantom{**} &          (0.0137)\phantom{**} &          (0.0138)\phantom{**}\smallskip \\
$y_{t-4}$    &                         &                         &                         &    \phantom{*}0.0416*** &  \phantom{*}0.009\phantom{**} &  \phantom{*}0.0077\phantom{*} &  \phantom{*}0.0078\phantom{*} \\
             &                         &                         &                         &    (0.013)\phantom{***} &                      (0.0136) &                      (0.0137) &                      (0.0138)\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &          \phantom{*}0.0976*** &          \phantom{*}0.0932*** &          \phantom{*}0.0931*** \\
             &                         &                         &                         &                         &          (0.0129)\phantom{**} &          (0.0136)\phantom{**} &          (0.0137)\phantom{**}\smallskip \\
$y_{t-6}$    &                         &                         &                         &                         &                               &             \phantom{*}0.0133 &  \phantom{*}0.0127\phantom{*} \\
             &                         &                         &                         &                         &                               &                       (0.013) &                      (0.0131) \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                           Yes &                           Yes &                           Yes \\
\medskip\\
Observations &                   6,017 &                   6,015 &                   6,012 &                   6,008 &                         6,003 &                         5,997 &                         5,897 \\
$R^2$        &                  0.2303 &                  0.2427 &                  0.2456 &                  0.2468 &                        0.2537 &                        0.2536 &                        0.2555 \\
\bottomrule
\end{tabular}


==> table/oracle/lag_reg_obL1.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} &       \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} &       \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
$y_{t-100}$  &                         &                         &                         &                               &                               &                               &            \phantom{*}0.0219* \\
             &                         &                         &                         &                               &                               &                               &            (0.013)\phantom{*}\smallskip \\
$y_{t-1}$    &    \phantom{*}0.1339*** &    \phantom{*}0.1286*** &    \phantom{*}0.1281*** &          \phantom{*}0.1283*** &          \phantom{*}0.1287*** &           \phantom{*}0.128*** &          \phantom{*}0.1299*** \\
             &    (0.0128)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &          (0.0129)\phantom{**} &          (0.0129)\phantom{**} &           (0.0129)\phantom{*} &          (0.013)\phantom{***}\smallskip \\
$y_{t-2}$    &                         &    \phantom{*}0.0394*** &    \phantom{*}0.0378*** &          \phantom{*}0.0384*** &          \phantom{*}0.0381*** &          \phantom{*}0.0389*** &           \phantom{*}0.036*** \\
             &                         &    (0.0129)\phantom{**} &    (0.013)\phantom{***} &          (0.013)\phantom{***} &          (0.013)\phantom{***} &          (0.013)\phantom{***} &           (0.0131)\phantom{*}\smallskip \\
$y_{t-3}$    &                         &                         &       \phantom{*}0.0121 &  \phantom{*}0.0141\phantom{*} &  \phantom{*}0.0128\phantom{*} &  \phantom{*}0.0129\phantom{*} &  \phantom{*}0.0149\phantom{*} \\
             &                         &                         &                 (0.013) &                      (0.0131) &                      (0.0131) &                      (0.0131) &                      (0.0132)\smallskip \\
$y_{t-4}$    &                         &                         &                         &                       -0.0154 &            -0.0199\phantom{*} &            -0.0209\phantom{*} &                      -0.0232* \\
             &                         &                         &                         &                       (0.013) &                      (0.0131) &                      (0.0131) &                      (0.0132)\smallskip \\
$y_{t-5}$    &                         &                         &                         &                               &          \phantom{*}0.0341*** &            \phantom{*}0.031** &           \phantom{*}0.0339** \\
             &                         &                         &                         &                               &          (0.013)\phantom{***} &                      (0.0131) &           (0.0132)\phantom{*}\smallskip \\
$y_{t-6}$    &                         &                         &                         &                               &                               &             \phantom{*}0.0195 &  \phantom{*}0.0207\phantom{*} \\
             &                         &                         &                         &                               &                               &                       (0.013) &                      (0.0131) \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                           Yes &                           Yes &                           Yes &                           Yes \\
\medskip\\
Observations &                   6,021 &                   6,019 &                   6,016 &                         6,012 &                         6,007 &                         6,001 &                         5,901 \\
$R^2$        &                  0.0728 &                  0.0741 &                   0.074 &                         0.074 &                        0.0749 &                        0.0752 &                         0.076 \\
\bottomrule
\end{tabular}


==> table/oracle/lag_reg_obL30.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} &       \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
$y_{t-100}$  &                         &                         &                         &                         &                               &                               &            -0.0066\phantom{*} \\
             &                         &                         &                         &                         &                               &                               &                      (0.0101)\smallskip \\
$y_{t-1}$    &    \phantom{*}0.6128*** &    \phantom{*}0.4947*** &    \phantom{*}0.4753*** &    \phantom{*}0.4718*** &          \phantom{*}0.4702*** &          \phantom{*}0.4683*** &          \phantom{*}0.4653*** \\
             &    (0.0102)\phantom{**} &    (0.0127)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &          (0.0129)\phantom{**} &          (0.013)\phantom{***} &          (0.0131)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &    \phantom{*}0.1922*** &    \phantom{*}0.1423*** &    \phantom{*}0.1375*** &          \phantom{*}0.1333*** &          \phantom{*}0.1331*** &          \phantom{*}0.1336*** \\
             &                         &    (0.0127)\phantom{**} &    (0.0142)\phantom{**} &    (0.0143)\phantom{**} &          (0.0143)\phantom{**} &          (0.0143)\phantom{**} &          (0.0144)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &    \phantom{*}0.1006*** &    \phantom{*}0.0844*** &          \phantom{*}0.0775*** &          \phantom{*}0.0748*** &           \phantom{*}0.076*** \\
             &                         &                         &    (0.0129)\phantom{**} &    (0.0143)\phantom{**} &          (0.0144)\phantom{**} &          (0.0144)\phantom{**} &           (0.0145)\phantom{*}\smallskip \\
$y_{t-4}$    &                         &                         &                         &    \phantom{*}0.0338*** &  \phantom{*}0.0106\phantom{*} &  \phantom{*}0.0056\phantom{*} &  \phantom{*}0.0051\phantom{*} \\
             &                         &                         &                         &    (0.0129)\phantom{**} &                      (0.0143) &                      (0.0144) &                      (0.0145)\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &          \phantom{*}0.0493*** &           \phantom{*}0.0319** &           \phantom{*}0.0335** \\
             &                         &                         &                         &                         &          (0.0129)\phantom{**} &           (0.0143)\phantom{*} &           (0.0144)\phantom{*}\smallskip \\
$y_{t-6}$    &                         &                         &                         &                         &                               &          \phantom{*}0.0363*** &          \phantom{*}0.0361*** \\
             &                         &                         &                         &                         &                               &          (0.013)\phantom{***} &          (0.0131)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                           Yes &                           Yes &                           Yes \\
\medskip\\
Observations &                   5,992 &                   5,990 &                   5,987 &                   5,983 &                         5,978 &                         5,972 &                         5,872 \\
$R^2$        &                  0.4159 &                  0.4374 &                  0.4429 &                  0.4432 &                        0.4443 &                        0.4449 &                        0.4427 \\
\bottomrule
\end{tabular}


==> table/oracle/lag_reg_obL5.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} &       \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
$y_{t-100}$  &                         &                         &                         &                         &                               &                               &  \phantom{*}0.0029\phantom{*} \\
             &                         &                         &                         &                         &                               &                               &                      (0.0121)\smallskip \\
$y_{t-1}$    &    \phantom{*}0.3707*** &    \phantom{*}0.3444*** &    \phantom{*}0.3454*** &    \phantom{*}0.3457*** &          \phantom{*}0.3452*** &          \phantom{*}0.3447*** &          \phantom{*}0.3452*** \\
             &    (0.012)\phantom{***} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &    (0.0129)\phantom{**} &          (0.0129)\phantom{**} &          (0.0129)\phantom{**} &          (0.0131)\phantom{**}\smallskip \\
$y_{t-2}$    &                         &     \phantom{*}0.071*** &     \phantom{*}0.076*** &    \phantom{*}0.0743*** &          \phantom{*}0.0747*** &          \phantom{*}0.0741*** &          \phantom{*}0.0743*** \\
             &                         &     (0.0129)\phantom{*} &     (0.0136)\phantom{*} &    (0.0137)\phantom{**} &          (0.0137)\phantom{**} &          (0.0137)\phantom{**} &          (0.0138)\phantom{**}\smallskip \\
$y_{t-3}$    &                         &                         &      -0.0146\phantom{*} &                -0.0228* &            -0.024*\phantom{*} &                      -0.0233* &                      -0.0244* \\
             &                         &                         &                (0.0129) &                (0.0137) &                      (0.0137) &                      (0.0137) &                      (0.0139)\smallskip \\
$y_{t-4}$    &                         &                         &                         &      \phantom{*}0.0239* &  \phantom{*}0.018\phantom{**} &  \phantom{*}0.0157\phantom{*} &  \phantom{*}0.0156\phantom{*} \\
             &                         &                         &                         &                (0.0129) &                      (0.0137) &                      (0.0137) &                      (0.0139)\smallskip \\
$y_{t-5}$    &                         &                         &                         &                         &             \phantom{*}0.0165 &  \phantom{*}0.0059\phantom{*} &  \phantom{*}0.0069\phantom{*} \\
             &                         &                         &                         &                         &                       (0.013) &                      (0.0137) &                      (0.0138)\smallskip \\
$y_{t-6}$    &                         &                         &                         &                         &                               &           \phantom{*}0.0302** &  \phantom{*}0.03**\phantom{*} \\
             &                         &                         &                         &                         &                               &           (0.013)\phantom{**} &                      (0.0131) \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                           Yes &                           Yes &                           Yes \\
\medskip\\
Observations &                   6,017 &                   6,015 &                   6,012 &                   6,008 &                         6,003 &                         5,997 &                         5,897 \\
$R^2$        &                  0.1696 &                  0.1737 &                  0.1737 &                   0.174 &                        0.1739 &                        0.1743 &                        0.1748 \\
\bottomrule
\end{tabular}


==> table/oracle/perf_reg_hbL1.tex <==
\begin{tabular}{lcccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} \\
\midrule
$(b-a)_0$    &                         &                         &              -0.0255*** &                         &                         &      -0.0017\phantom{*} \\
             &                         &                         &    (0.0021)\phantom{**} &                         &                         &                (0.0034)\smallskip \\
$JUMP_0$     &                         &    \phantom{*}0.0016*** &                         &                         &    \phantom{*}0.0016*** &                         \\
             &                         &    (0.0001)\phantom{**} &                         &                         &    (0.0002)\phantom{**} &                        \smallskip \\
$VIX_0$      &    \phantom{*}0.0001*** &                         &                         &    \phantom{*}0.0002*** &                         &                         \\
             &    (0.0)\phantom{*****} &                         &                         &    (0.0)\phantom{*****} &                         &                        \smallskip \\
one          &              -0.0059*** &              -0.0041*** &    \phantom{*}0.0008*** &                         &                         &                         \\
             &    (0.0002)\phantom{**} &    (0.0001)\phantom{**} &    (0.0003)\phantom{**} &                         &                         &                         \\
\medskip\\
year FE      &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes \\
CD           &                 57.3407 &                 3.26813 &                 29.3001 &                 406.048 &                 10.7335 &                 15.6806 \\
\medskip\\
Observations &                   6,002 &                   5,938 &                   6,002 &                   6,002 &                   5,938 &                   6,002 \\
$R^2$        &                  0.0451 &                  0.0193 &                  0.0244 &                  0.1906 &                  0.1621 &                  0.1536 \\
\bottomrule
\end{tabular}


==> table/oracle/perf_reg_hbL30.tex <==
\begin{tabular}{lcccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} &       \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} &       \parboxc{c}{0.6cm}{(6)} \\
\midrule
$(b-a)_0$    &                         &                         &                    -0.0171*** &                         &                         &  \phantom{*}0.0006\phantom{*} \\
             &                         &                         &          (0.0037)\phantom{**} &                         &                         &                      (0.0061)\smallskip \\
$JUMP_0$     &                         &     \phantom{*}0.005*** &                               &                         &    \phantom{*}0.0052*** &                               \\
             &                         &     (0.0003)\phantom{*} &                               &                         &    (0.0003)\phantom{**} &                              \smallskip \\
$VIX_0$      &    \phantom{*}0.0003*** &                         &                               &    \phantom{*}0.0004*** &                         &                               \\
             &    (0.0)\phantom{*****} &                         &                               &    (0.0)\phantom{*****} &                         &                              \smallskip \\
one          &              -0.0083*** &              -0.0053*** &  \phantom{*}0.0008\phantom{*} &                         &                         &                               \\
             &    (0.0003)\phantom{**} &    (0.0002)\phantom{**} &                      (0.0005) &                         &                         &                               \\
\medskip\\
year FE      &                      No &                      No &                            No &                     Yes &                     Yes &                           Yes \\
CD           &                 57.3495 &                 3.26697 &                        29.289 &                 409.473 &                 11.1234 &                       15.5327 \\
\medskip\\
Observations &                   5,963 &                   5,899 &                         5,963 &                   5,963 &                   5,899 &                         5,963 \\
$R^2$        &                  0.0748 &                  0.0612 &                        0.0035 &                  0.1205 &                  0.1141 &                        0.0794 \\
\bottomrule
\end{tabular}


==> table/oracle/perf_reg_hbL5.tex <==
\begin{tabular}{lcccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} \\
\midrule
$(b-a)_0$    &                         &                         &              -0.0263*** &                         &                         &      -0.0009\phantom{*} \\
             &                         &                         &    (0.0026)\phantom{**} &                         &                         &                (0.0044)\smallskip \\
$JUMP_0$     &                         &    \phantom{*}0.0025*** &                         &                         &    \phantom{*}0.0031*** &                         \\
             &                         &    (0.0002)\phantom{**} &                         &                         &    (0.0002)\phantom{**} &                        \smallskip \\
$VIX_0$      &    \phantom{*}0.0002*** &                         &                         &    \phantom{*}0.0003*** &                         &                         \\
             &    (0.0)\phantom{*****} &                         &                         &    (0.0)\phantom{*****} &                         &                        \smallskip \\
one          &              -0.0059*** &               -0.004*** &    \phantom{*}0.0016*** &                         &                         &                         \\
             &    (0.0002)\phantom{**} &     (0.0002)\phantom{*} &    (0.0004)\phantom{**} &                         &                         &                         \\
\medskip\\
year FE      &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes \\
CD           &                 57.3549 &                 3.26847 &                 29.2926 &                 405.974 &                 10.7666 &                 15.6638 \\
\medskip\\
Observations &                   5,998 &                   5,934 &                   5,998 &                   5,998 &                   5,934 &                   5,998 \\
$R^2$        &                  0.0434 &                  0.0288 &                  0.0162 &                  0.1283 &                  0.1116 &                  0.0889 \\
\bottomrule
\end{tabular}


==> table/oracle/perf_reg_obL1.tex <==
\begin{tabular}{lcccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} &       \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} \\
\midrule
$(b-a)_0$    &                         &                         &                    -0.0128*** &                         &                               &              -0.0177*** \\
             &                         &                         &          (0.0022)\phantom{**} &                         &                               &    (0.0038)\phantom{**}\smallskip \\
$JUMP_0$     &                         &              -0.0004*** &                               &                         &  \phantom{*}0.0003\phantom{*} &                         \\
             &                         &    (0.0002)\phantom{**} &                               &                         &                      (0.0002) &                        \smallskip \\
$VIX_0$      &                 -0.0*** &                         &                               &        \phantom{*}0.0** &                               &                         \\
             &       (0.0)\phantom{**} &                         &                               &        (0.0)\phantom{*} &                               &                        \smallskip \\
one          &              -0.0012*** &              -0.0014*** &  \phantom{*}0.0001\phantom{*} &                         &                               &                         \\
             &    (0.0002)\phantom{**} &    (0.0001)\phantom{**} &                      (0.0003) &                         &                               &                         \\
\medskip\\
year FE      &                      No &                      No &                            No &                     Yes &                           Yes &                     Yes \\
CD           &                 57.3407 &                 3.26813 &                       29.3001 &                 406.048 &                       10.7335 &                 15.6806 \\
\medskip\\
Observations &                   6,002 &                   5,938 &                         6,002 &                   6,002 &                         5,938 &                   6,002 \\
$R^2$        &                  0.0011 &                  0.0011 &                        0.0054 &                  0.0573 &                        0.0577 &                  0.0599 \\
\bottomrule
\end{tabular}


==> table/oracle/perf_reg_obL30.tex <==
\begin{tabular}{lcccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} \\
\midrule
$(b-a)_0$    &                         &                         &     \phantom{*}0.0106** &                         &                         &    \phantom{*}0.0246*** \\
             &                         &                         &     (0.0045)\phantom{*} &                         &                         &    (0.0075)\phantom{**}\smallskip \\
$JUMP_0$     &                         &    \phantom{*}0.0049*** &                         &                         &    \phantom{*}0.0066*** &                         \\
             &                         &    (0.0003)\phantom{**} &                         &                         &    (0.0004)\phantom{**} &                        \smallskip \\
$VIX_0$      &    \phantom{*}0.0003*** &                         &                         &    \phantom{*}0.0004*** &                         &                         \\
             &    (0.0)\phantom{*****} &                         &                         &    (0.0)\phantom{*****} &                         &                        \smallskip \\
one          &              -0.0084*** &              -0.0064*** &              -0.0044*** &                         &                         &                         \\
             &    (0.0004)\phantom{**} &    (0.0003)\phantom{**} &    (0.0007)\phantom{**} &                         &                         &                         \\
\medskip\\
year FE      &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes \\
CD           &                 57.3495 &                 3.26697 &                  29.289 &                 409.473 &                 11.1234 &                 15.5327 \\
\medskip\\
Observations &                   5,963 &                   5,899 &                   5,963 &                   5,963 &                   5,899 &                   5,963 \\
$R^2$        &                  0.0359 &                  0.0406 &                  0.0008 &                  0.0903 &                  0.0977 &                   0.063 \\
\bottomrule
\end{tabular}


==> table/oracle/perf_reg_obL5.tex <==
\begin{tabular}{lcccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} &    \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} \\
\midrule
$(b-a)_0$    &                         &                         &              -0.0124*** &                            &                               &              -0.0208*** \\
             &                         &                         &    (0.003)\phantom{***} &                            &                               &    (0.0051)\phantom{**}\smallskip \\
$JUMP_0$     &                         &               -0.0004** &                         &                            &  \phantom{*}0.0003\phantom{*} &                         \\
             &                         &     (0.0002)\phantom{*} &                         &                            &                      (0.0003) &                        \smallskip \\
$VIX_0$      &                 -0.0*** &                         &                         &  \phantom{*}0.0\phantom{*} &                               &                         \\
             &       (0.0)\phantom{**} &                         &                         &                      (0.0) &                               &                        \smallskip \\
one          &              -0.0019*** &              -0.0023*** &                -0.0008* &                            &                               &                         \\
             &    (0.0003)\phantom{**} &    (0.0002)\phantom{**} &                (0.0004) &                            &                               &                         \\
\medskip\\
year FE      &                      No &                      No &                      No &                        Yes &                           Yes &                     Yes \\
CD           &                 57.3549 &                 3.26847 &                 29.2926 &                    405.974 &                       10.7666 &                 15.6638 \\
\medskip\\
Observations &                   5,998 &                   5,934 &                   5,998 &                      5,998 &                         5,934 &                   5,998 \\
$R^2$        &                   0.001 &                  0.0006 &                  0.0027 &                     0.0372 &                        0.0381 &                  0.0399 \\
\bottomrule
\end{tabular}


==> table/oracle_oos_mean.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  HM. oracle &  BDJM. oracle &  RF. oracle \\
\midrule
1  &     0.01329 &       0.01538 &     0.01342 \\
2  &     0.01514 &       0.01900 &     0.01564 \\
3  &     0.01605 &       0.02079 &     0.01692 \\
4  &     0.01670 &       0.02189 &     0.01719 \\
5  &     0.01722 &       0.02256 &     0.01746 \\
6  &     0.01773 &       0.02350 &     0.01838 \\
7  &     0.01813 &       0.02439 &     0.01898 \\
8  &     0.01855 &       0.02494 &     0.01923 \\
9  &     0.01884 &       0.02540 &     0.01964 \\
10 &     0.01917 &       0.02577 &     0.02047 \\
11 &     0.01941 &       0.02675 &     0.02103 \\
12 &     0.01967 &       0.02751 &     0.02175 \\
13 &     0.01987 &       0.02808 &     0.02202 \\
14 &     0.01977 &       0.02805 &     0.02183 \\
15 &     0.01973 &       0.02808 &     0.02166 \\
16 &     0.01972 &       0.02836 &     0.02175 \\
17 &     0.01966 &       0.02792 &     0.02171 \\
18 &     0.01951 &       0.02733 &     0.02119 \\
19 &     0.01935 &       0.02626 &     0.02056 \\
20 &     0.01933 &       0.02587 &     0.02046 \\
21 &     0.01970 &       0.02683 &     0.02114 \\
22 &     0.02003 &       0.02770 &     0.02134 \\
23 &     0.02017 &       0.02837 &     0.02108 \\
24 &     0.02038 &       0.02796 &     0.02076 \\
25 &     0.02053 &       0.02871 &     0.02110 \\
26 &     0.02076 &       0.02927 &     0.02160 \\
27 &     0.02104 &       0.02976 &     0.02184 \\
28 &     0.02128 &       0.03009 &     0.02205 \\
29 &     0.02139 &       0.03033 &     0.02233 \\
30 &     0.02147 &       0.03120 &     0.02285 \\
\bottomrule
\end{tabular}


==> table/oracle_oos_q10.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  HM. oracle &  BDJM. oracle &  RF. oracle \\
\midrule
1  &     0.00584 &       0.00565 &     0.00375 \\
2  &     0.00628 &       0.00601 &     0.00480 \\
3  &     0.00651 &       0.00632 &     0.00520 \\
4  &     0.00671 &       0.00651 &     0.00538 \\
5  &     0.00683 &       0.00669 &     0.00549 \\
6  &     0.00704 &       0.00678 &     0.00589 \\
7  &     0.00718 &       0.00698 &     0.00634 \\
8  &     0.00730 &       0.00696 &     0.00651 \\
9  &     0.00739 &       0.00712 &     0.00661 \\
10 &     0.00738 &       0.00706 &     0.00677 \\
11 &     0.00738 &       0.00731 &     0.00702 \\
12 &     0.00750 &       0.00744 &     0.00743 \\
13 &     0.00743 &       0.00748 &     0.00740 \\
14 &     0.00741 &       0.00763 &     0.00724 \\
15 &     0.00755 &       0.00754 &     0.00722 \\
16 &     0.00750 &       0.00764 &     0.00734 \\
17 &     0.00752 &       0.00769 &     0.00738 \\
18 &     0.00748 &       0.00766 &     0.00732 \\
19 &     0.00750 &       0.00745 &     0.00708 \\
20 &     0.00757 &       0.00773 &     0.00720 \\
21 &     0.00768 &       0.00780 &     0.00740 \\
22 &     0.00783 &       0.00790 &     0.00765 \\
23 &     0.00784 &       0.00815 &     0.00756 \\
24 &     0.00787 &       0.00792 &     0.00755 \\
25 &     0.00772 &       0.00790 &     0.00747 \\
26 &     0.00787 &       0.00801 &     0.00783 \\
27 &     0.00802 &       0.00804 &     0.00792 \\
28 &     0.00802 &       0.00811 &     0.00790 \\
29 &     0.00805 &       0.00821 &     0.00781 \\
30 &     0.00803 &       0.00828 &     0.00817 \\
\bottomrule
\end{tabular}


==> table/oracle_oos_q50.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  HM. oracle &  BDJM. oracle &  RF. oracle \\
\midrule
1  &     0.01015 &       0.01086 &     0.00855 \\
2  &     0.01114 &       0.01251 &     0.01046 \\
3  &     0.01174 &       0.01343 &     0.01146 \\
4  &     0.01206 &       0.01362 &     0.01154 \\
5  &     0.01222 &       0.01422 &     0.01182 \\
6  &     0.01256 &       0.01467 &     0.01271 \\
7  &     0.01294 &       0.01510 &     0.01313 \\
8  &     0.01322 &       0.01515 &     0.01340 \\
9  &     0.01341 &       0.01542 &     0.01336 \\
10 &     0.01366 &       0.01575 &     0.01394 \\
11 &     0.01367 &       0.01633 &     0.01447 \\
12 &     0.01378 &       0.01668 &     0.01506 \\
13 &     0.01384 &       0.01695 &     0.01533 \\
14 &     0.01381 &       0.01671 &     0.01493 \\
15 &     0.01401 &       0.01676 &     0.01487 \\
16 &     0.01399 &       0.01696 &     0.01516 \\
17 &     0.01387 &       0.01702 &     0.01527 \\
18 &     0.01378 &       0.01685 &     0.01497 \\
19 &     0.01387 &       0.01653 &     0.01448 \\
20 &     0.01400 &       0.01670 &     0.01440 \\
21 &     0.01434 &       0.01723 &     0.01500 \\
22 &     0.01438 &       0.01778 &     0.01538 \\
23 &     0.01442 &       0.01784 &     0.01524 \\
24 &     0.01475 &       0.01792 &     0.01491 \\
25 &     0.01478 &       0.01805 &     0.01532 \\
26 &     0.01492 &       0.01831 &     0.01563 \\
27 &     0.01500 &       0.01832 &     0.01580 \\
28 &     0.01528 &       0.01841 &     0.01601 \\
29 &     0.01557 &       0.01878 &     0.01612 \\
30 &     0.01560 &       0.01931 &     0.01620 \\
\bottomrule
\end{tabular}


==> table/oracle_oos_q90.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  HM. oracle &  BDJM. oracle &  RF. oracle \\
\midrule
1  &     0.02336 &       0.02774 &     0.02696 \\
2  &     0.02833 &       0.03757 &     0.03089 \\
3  &     0.02962 &       0.04124 &     0.03221 \\
4  &     0.03106 &       0.04355 &     0.03304 \\
5  &     0.03167 &       0.04676 &     0.03376 \\
6  &     0.03263 &       0.04995 &     0.03522 \\
7  &     0.03312 &       0.05033 &     0.03629 \\
8  &     0.03373 &       0.05288 &     0.03641 \\
9  &     0.03409 &       0.05316 &     0.03672 \\
10 &     0.03457 &       0.05480 &     0.03823 \\
11 &     0.03536 &       0.05643 &     0.04017 \\
12 &     0.03689 &       0.05804 &     0.04072 \\
13 &     0.03657 &       0.05783 &     0.04169 \\
14 &     0.03651 &       0.05821 &     0.04074 \\
15 &     0.03655 &       0.05881 &     0.04053 \\
16 &     0.03679 &       0.06025 &     0.04143 \\
17 &     0.03578 &       0.05603 &     0.04067 \\
18 &     0.03505 &       0.05395 &     0.03912 \\
19 &     0.03414 &       0.05249 &     0.03799 \\
20 &     0.03551 &       0.05065 &     0.03814 \\
21 &     0.03649 &       0.05435 &     0.03858 \\
22 &     0.03740 &       0.05537 &     0.03865 \\
23 &     0.03748 &       0.05717 &     0.03843 \\
24 &     0.03651 &       0.05674 &     0.03826 \\
25 &     0.03697 &       0.05954 &     0.03903 \\
26 &     0.03804 &       0.06114 &     0.03927 \\
27 &     0.03994 &       0.06265 &     0.04000 \\
28 &     0.04026 &       0.06340 &     0.04052 \\
29 &     0.04082 &       0.06454 &     0.04103 \\
30 &     0.03956 &       0.06617 &     0.04209 \\
\bottomrule
\end{tabular}


==> table/oracle_oos_q95.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  HM. oracle &  BDJM. oracle &  RF. oracle \\
\midrule
1  &     0.05662 &       0.07485 &     0.07583 \\
2  &     0.06755 &       0.10071 &     0.08241 \\
3  &     0.07774 &       0.12377 &     0.09349 \\
4  &     0.08298 &       0.13732 &     0.09232 \\
5  &     0.08426 &       0.13633 &     0.10300 \\
6  &     0.09217 &       0.14314 &     0.10048 \\
7  &     0.09315 &       0.15002 &     0.10160 \\
8  &     0.08884 &       0.16161 &     0.10333 \\
9  &     0.10353 &       0.16097 &     0.10910 \\
10 &     0.10777 &       0.15634 &     0.11335 \\
11 &     0.10774 &       0.16799 &     0.11522 \\
12 &     0.10977 &       0.17608 &     0.12329 \\
13 &     0.11116 &       0.17613 &     0.11869 \\
14 &     0.11490 &       0.17398 &     0.12363 \\
15 &     0.10465 &       0.17636 &     0.12168 \\
16 &     0.10935 &       0.18003 &     0.11938 \\
17 &     0.10674 &       0.18852 &     0.11649 \\
18 &     0.10411 &       0.18850 &     0.11387 \\
19 &     0.10354 &       0.17341 &     0.11109 \\
20 &     0.09498 &       0.14752 &     0.10782 \\
21 &     0.10126 &       0.15733 &     0.10492 \\
22 &     0.10179 &       0.16034 &     0.10705 \\
23 &     0.10081 &       0.17895 &     0.10805 \\
24 &     0.10085 &       0.16472 &     0.10620 \\
25 &     0.10280 &       0.17706 &     0.10248 \\
26 &     0.10077 &       0.18018 &     0.10560 \\
27 &     0.10491 &       0.18767 &     0.10822 \\
28 &     0.10580 &       0.17693 &     0.11001 \\
29 &     0.10018 &       0.17567 &     0.11634 \\
30 &     0.10352 &       0.18129 &     0.11879 \\
\bottomrule
\end{tabular}


==> table/perf_reg_hbL1.tex <==
\begin{tabular}{lcccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} & \parboxc{c}{0.6cm}{(7)} & \parboxc{c}{0.6cm}{(8)} \\
\midrule
$(b-a)_t$       &                         &                         &    \phantom{*}0.0061*** &    \phantom{*}0.0025*** &                         &                         &    \phantom{*}0.0511*** &    \phantom{*}0.0226*** \\
                &                         &                         &    (0.0008)\phantom{**} &    (0.0009)\phantom{**} &                         &                         &    (0.0019)\phantom{**} &    (0.0019)\phantom{**}\smallskip \\
$JUMP_t$        &                         &              -0.0048*** &                         &              -0.0048*** &                         &              -0.0069*** &                         &              -0.0081*** \\
                &                         &    (0.0001)\phantom{**} &                         &    (0.0001)\phantom{**} &                         &    (0.0001)\phantom{**} &                         &    (0.0001)\phantom{**}\smallskip \\
$VIX_t$         &              -0.0006*** &                         &                         &                         &              -0.0008*** &                         &                         &                         \\
                &    (0.0)\phantom{*****} &                         &                         &                         &    (0.0)\phantom{*****} &                         &                         &                        \smallskip \\
$\tilde{VIX_t}$ &                         &                         &                         &               -0.001*** &                         &                         &                         &               -0.001*** \\
                &                         &                         &                         &     (0.0)\phantom{****} &                         &                         &                         &     (0.0)\phantom{****}\smallskip \\
constant        &              -0.0021*** &               -0.009*** &              -0.0123*** &              -0.0093*** &                         &                         &                         &                         \\
                &    (0.0001)\phantom{**} &     (0.0001)\phantom{*} &    (0.0001)\phantom{**} &    (0.0001)\phantom{**} &                         &                         &                         &                         \\
\medskip\\
year FE         &                      No &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes &                     Yes \\
CD              &                 50.6997 &                  3.8966 &                 28.8601 &                 109.365 &                 442.682 &                 14.2311 &                 35.1089 &                 304.418 \\
\medskip\\
Observations    &               5,517,409 &               5,508,146 &               5,517,409 &               5,508,146 &               5,517,409 &               5,508,146 &               5,517,409 &               5,508,146 \\
$R^2$           &                  0.0026 &                  0.0005 &                       0 &                  0.0035 &                  0.0064 &                  0.0043 &                   0.004 &                  0.0066 \\
\bottomrule
\end{tabular}


==> table/perf_reg_hbL30.tex <==
\begin{tabular}{lcccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} & \parboxc{c}{0.6cm}{(7)} & \parboxc{c}{0.6cm}{(8)} \\
\midrule
$(b-a)_t$       &                         &                         &              -0.0526*** &               -0.067*** &                         &                         &              -0.0694*** &              -0.1055*** \\
                &                         &                         &    (0.0018)\phantom{**} &     (0.0019)\phantom{*} &                         &                         &    (0.0041)\phantom{**} &    (0.0042)\phantom{**}\smallskip \\
$JUMP_t$        &                         &              -0.0051*** &                         &              -0.0036*** &                         &              -0.0026*** &                         &              -0.0054*** \\
                &                         &    (0.0002)\phantom{**} &                         &    (0.0002)\phantom{**} &                         &    (0.0003)\phantom{**} &                         &    (0.0003)\phantom{**}\smallskip \\
$VIX_t$         &              -0.0007*** &                         &                         &                         &              -0.0009*** &                         &                         &                         \\
                &    (0.0)\phantom{*****} &                         &                         &                         &    (0.0)\phantom{*****} &                         &                         &                        \smallskip \\
$\tilde{VIX_t}$ &                         &                         &                         &              -0.0016*** &                         &                         &                         &              -0.0016*** \\
                &                         &                         &                         &    (0.0)\phantom{*****} &                         &                         &                         &    (0.0)\phantom{*****}\smallskip \\
constant        &              -0.0009*** &              -0.0106*** &              -0.0065*** &              -0.0028*** &                         &                         &                         &                         \\
                &    (0.0002)\phantom{**} &    (0.0001)\phantom{**} &    (0.0002)\phantom{**} &    (0.0002)\phantom{**} &                         &                         &                         &                         \\
\medskip\\
year FE         &                      No &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes &                     Yes \\
CD              &                 50.7216 &                 3.96725 &                 28.9412 &                 108.885 &                 450.495 &                 14.8485 &                 35.9498 &                 305.763 \\
\medskip\\
Observations    &               5,340,055 &               5,332,648 &               5,340,055 &               5,332,648 &               5,340,055 &               5,332,648 &               5,340,055 &               5,332,648 \\
$R^2$           &                   0.001 &                  0.0001 &                  0.0002 &                  0.0018 &                  0.0044 &                  0.0037 &                  0.0037 &                  0.0049 \\
\bottomrule
\end{tabular}


==> table/perf_reg_hbL5.tex <==
\begin{tabular}{lcccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} & \parboxc{c}{0.6cm}{(7)} & \parboxc{c}{0.6cm}{(8)} \\
\midrule
$(b-a)_t$       &                         &                         &      \phantom{*}0.0022* &     \phantom{*}0.0029** &                         &                         &     \phantom{*}0.075*** &    \phantom{*}0.0516*** \\
                &                         &                         &                (0.0012) &     (0.0013)\phantom{*} &                         &                         &     (0.0028)\phantom{*} &    (0.0028)\phantom{**}\smallskip \\
$JUMP_t$        &                         &              -0.0049*** &                         &              -0.0049*** &                         &              -0.0078*** &                         &              -0.0083*** \\
                &                         &    (0.0001)\phantom{**} &                         &    (0.0001)\phantom{**} &                         &    (0.0002)\phantom{**} &                         &    (0.0002)\phantom{**}\smallskip \\
$VIX_t$         &              -0.0005*** &                         &                         &                         &              -0.0006*** &                         &                         &                         \\
                &    (0.0)\phantom{*****} &                         &                         &                         &    (0.0)\phantom{*****} &                         &                         &                        \smallskip \\
$\tilde{VIX_t}$ &                         &                         &                         &              -0.0007*** &                         &                         &                         &              -0.0007*** \\
                &                         &                         &                         &    (0.0)\phantom{*****} &                         &                         &                         &    (0.0)\phantom{*****}\smallskip \\
constant        &              -0.0045*** &              -0.0097*** &              -0.0126*** &                -0.01*** &                         &                         &                         &                         \\
                &    (0.0001)\phantom{**} &    (0.0001)\phantom{**} &    (0.0002)\phantom{**} &                (0.0002) &                         &                         &                         &                         \\
\medskip\\
year FE         &                      No &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes &                     Yes \\
CD              &                 50.7023 &                 3.90577 &                 28.8714 &                 109.299 &                 443.476 &                 14.2956 &                 35.2186 &                 304.578 \\
\medskip\\
Observations    &               5,493,397 &               5,484,390 &               5,493,397 &               5,484,390 &               5,493,397 &               5,484,390 &               5,493,397 &               5,484,390 \\
$R^2$           &                  0.0008 &                  0.0003 &                       0 &                   0.001 &                  0.0027 &                  0.0022 &                   0.002 &                  0.0027 \\
\bottomrule
\end{tabular}


==> table/perf_reg_obL1.tex <==
\begin{tabular}{lcccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} & \parboxc{c}{0.6cm}{(7)} & \parboxc{c}{0.6cm}{(8)} \\
\midrule
$(b-a)_t$       &                         &                         &               -0.4326** &              -1.1106*** &                         &                         &    \phantom{*}6.8411*** &      -0.0998\phantom{*} \\
                &                         &                         &     (0.2173)\phantom{*} &    (0.2245)\phantom{**} &                         &                         &    (0.4922)\phantom{**} &                (0.3103)\smallskip \\
$JUMP_t$        &                         &              -0.2537*** &                         &              -0.2288*** &                         &                 -0.0202 &                         &              -0.3194*** \\
                &                         &    (0.0228)\phantom{**} &                         &    (0.0233)\phantom{**} &                         &                 (0.034) &                         &    (0.0305)\phantom{**}\smallskip \\
$VIX_t$         &               -0.041*** &                         &                         &                         &              -0.0485*** &                         &                         &                         \\
                &     (0.0012)\phantom{*} &                         &                         &                         &    (0.0017)\phantom{**} &                         &                         &                        \smallskip \\
$\tilde{VIX_t}$ &                         &                         &                         &              -0.0871*** &                         &                         &                         &              -0.0941*** \\
                &                         &                         &                         &    (0.0021)\phantom{**} &                         &                         &                         &    (0.0023)\phantom{**}\smallskip \\
constant        &    \phantom{*}0.3713*** &              -0.1766*** &               -0.256*** &                 -0.0464 &                         &                         &                         &                         \\
                &    (0.0217)\phantom{**} &    (0.0144)\phantom{**} &     (0.0291)\phantom{*} &       (0.03)\phantom{*} &                         &                         &                         &                         \\
\medskip\\
year FE         &                      No &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes &                     Yes \\
CD              &                 50.6991 &                 3.89434 &                 28.8573 &                 109.381 &                  442.49 &                 14.2154 &                 35.0816 &                 174.618 \\
\medskip\\
Observations    &               5,523,411 &               5,514,084 &               5,523,411 &               5,514,084 &               5,523,411 &               5,514,084 &               5,523,411 &               5,514,084 \\
$R^2$           &                  0.0002 &                       0 &                       0 &                  0.0003 &                  0.0004 &                  0.0002 &                  0.0002 &                  0.0008 \\
\bottomrule
\end{tabular}


==> table/perf_reg_obL30.tex <==
\begin{tabular}{lcccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} &          \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} &          \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} &          \parboxc{c}{0.6cm}{(6)} &          \parboxc{c}{0.6cm}{(7)} &          \parboxc{c}{0.6cm}{(8)} \\
\midrule
$(b-a)_t$       &                         &                                  &              19.2497*** &                         60.76*** &                         &                                  &                      162.4937*** &                       96.8253*** \\
                &                         &                                  &    (0.9452)\phantom{**} &                         (0.9741) &                         &                                  &  \phantom{*}(2.1408)\phantom{**} &             (1.3451)\phantom{**}\smallskip \\
$JUMP_t$        &                         &                      -13.4754*** &                         &                      -14.8361*** &                         &                      -24.2848*** &                                  &                      -23.5819*** \\
                &                         &  \phantom{*}(0.099)\phantom{***} &                         &  \phantom{*}(0.1013)\phantom{**} &                         &  \phantom{*}(0.1473)\phantom{**} &                                  &  \phantom{*}(0.1324)\phantom{**}\smallskip \\
$VIX_t$         &              -0.3061*** &                                  &                         &                                  &              -0.2809*** &                                  &                                  &                                  \\
                &    (0.0053)\phantom{**} &                                  &                         &                                  &    (0.0074)\phantom{**} &                                  &                                  &                                 \smallskip \\
$\tilde{VIX_t}$ &                         &                                  &                         &             \phantom{*}0.8553*** &                         &                                  &                                  &              \phantom{*}1.029*** \\
                &                         &                                  &                         &             (0.009)\phantom{***} &                         &                                  &                                  &              (0.0099)\phantom{*}\smallskip \\
constant        &    \phantom{*}2.4645*** &             \phantom{*}4.5261*** &              -5.1236*** &                       -2.5984*** &                         &                                  &                                  &                                  \\
                &    (0.0945)\phantom{**} &             (0.0623)\phantom{**} &    (0.1265)\phantom{**} &             (0.1301)\phantom{**} &                         &                                  &                                  &                                  \\
\medskip\\
year FE         &                      No &                               No &                      No &                               No &                     Yes &                              Yes &                              Yes &                              Yes \\
CD              &                 50.6867 &                          3.89322 &                 28.8498 &                          109.392 &                 443.021 &                          14.2601 &                          35.0994 &                          174.646 \\
\medskip\\
Observations    &               5,519,005 &                        5,509,678 &               5,519,005 &                        5,509,678 &               5,519,005 &                        5,509,678 &                        5,519,005 &                        5,509,678 \\
$R^2$           &                  0.0006 &                           0.0034 &                  0.0001 &                           0.0054 &                  0.0009 &                           0.0055 &                           0.0017 &                           0.0092 \\
\bottomrule
\end{tabular}


==> table/perf_reg_obL5.tex <==
\begin{tabular}{lcccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} & \parboxc{c}{0.6cm}{(7)} & \parboxc{c}{0.6cm}{(8)} \\
\midrule
$(b-a)_t$       &                         &                         &              -1.3513*** &               -3.612*** &                         &                         &              15.8412*** &    \phantom{*}7.2956*** \\
                &                         &                         &    (0.5008)\phantom{**} &     (0.5173)\phantom{*} &                         &                         &    (1.1346)\phantom{**} &    (0.7151)\phantom{**}\smallskip \\
$JUMP_t$        &                         &              -0.7315*** &                         &              -0.6506*** &                         &              -0.7505*** &                         &              -1.1787*** \\
                &                         &    (0.0525)\phantom{**} &                         &    (0.0538)\phantom{**} &                         &    (0.0783)\phantom{**} &                         &    (0.0704)\phantom{**}\smallskip \\
$VIX_t$         &              -0.1244*** &                         &                         &                         &              -0.1907*** &                         &                         &                         \\
                &    (0.0028)\phantom{**} &                         &                         &                         &    (0.0039)\phantom{**} &                         &                         &                        \smallskip \\
$\tilde{VIX_t}$ &                         &                         &                         &              -0.2705*** &                         &                         &                         &              -0.3086*** \\
                &                         &                         &                         &    (0.0048)\phantom{**} &                         &                         &                         &    (0.0053)\phantom{**}\smallskip \\
constant        &    \phantom{*}1.1129*** &              -0.5713*** &              -0.7856*** &               -0.1478** &                         &                         &                         &                         \\
                &    (0.0501)\phantom{**} &    (0.0331)\phantom{**} &    (0.067)\phantom{***} &     (0.0691)\phantom{*} &                         &                         &                         &                         \\
\medskip\\
year FE         &                      No &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes &                     Yes \\
CD              &                 50.6991 &                 3.89434 &                 28.8573 &                 109.381 &                 442.491 &                 14.2156 &                 35.0815 &                 174.618 \\
\medskip\\
Observations    &               5,523,407 &               5,514,080 &               5,523,407 &               5,514,080 &               5,523,407 &               5,514,080 &               5,523,407 &               5,514,080 \\
$R^2$           &                  0.0004 &                       0 &                       0 &                  0.0006 &                  0.0006 &                  0.0002 &                  0.0002 &                  0.0013 \\
\bottomrule
\end{tabular}


==> table/perf_reg_panel_1.tex <==
\begin{tabular}{lcccccccc}
\toprule \multicolumn{6}{c}{\parboxc{c}{0.7cm}{Panel A: $y_{t,i,t} = 100(MSE_{DBJM,i,t}-MSE_{HM,i,t})$}} \\\hline
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} & \parboxc{c}{0.6cm}{(7)} & \parboxc{c}{0.6cm}{(8)} \\
\midrule
$(b-a)_t$       &                         &                         &    \phantom{*}0.0061*** &    \phantom{*}0.0025*** &                         &                         &    \phantom{*}0.0511*** &    \phantom{*}0.0226*** \\
                &                         &                         &    (0.0008)\phantom{**} &    (0.0009)\phantom{**} &                         &                         &    (0.0019)\phantom{**} &    (0.0019)\phantom{**}\smallskip \\
$JUMP_t$        &                         &              -0.0048*** &                         &              -0.0048*** &                         &              -0.0069*** &                         &              -0.0081*** \\
                &                         &    (0.0001)\phantom{**} &                         &    (0.0001)\phantom{**} &                         &    (0.0001)\phantom{**} &                         &    (0.0001)\phantom{**}\smallskip \\
$VIX_t$         &              -0.0006*** &                         &                         &                         &              -0.0008*** &                         &                         &                         \\
                &    (0.0)\phantom{*****} &                         &                         &                         &    (0.0)\phantom{*****} &                         &                         &                        \smallskip \\
$\tilde{VIX_t}$ &                         &                         &                         &               -0.001*** &                         &                         &                         &               -0.001*** \\
                &                         &                         &                         &     (0.0)\phantom{****} &                         &                         &                         &     (0.0)\phantom{****}\smallskip \\
constant        &              -0.0021*** &               -0.009*** &              -0.0123*** &              -0.0093*** &                         &                         &                         &                         \\
                &    (0.0001)\phantom{**} &     (0.0001)\phantom{*} &    (0.0001)\phantom{**} &    (0.0001)\phantom{**} &                         &                         &                         &                         \\
\medskip\\
year FE         &                      No &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes &                     Yes \\
\medskip\\
Observations    &               5,517,409 &               5,508,146 &               5,517,409 &               5,508,146 &               5,517,409 &               5,508,146 &               5,517,409 &               5,508,146 \\
$R^2$           &                  0.0026 &                  0.0005 &                       0 &                  0.0035 &                  0.0064 &                  0.0043 &                   0.004 &                  0.0066 \bigskip \\ 


\hline \multicolumn{6}{c}{\parboxc{c}{0.6cm}{Panel B: $y_{i,t} = 100(MSE_{DBJM,i,t}-MSE_{RF,i,t})$}} \\\hline
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} & \parboxc{c}{0.6cm}{(7)} & \parboxc{c}{0.6cm}{(8)} \\
\midrule
$(b-a)_t$       &                         &                         &               -0.4326** &              -1.1106*** &                         &                         &    \phantom{*}6.8411*** &      -0.0998\phantom{*} \\
                &                         &                         &     (0.2173)\phantom{*} &    (0.2245)\phantom{**} &                         &                         &    (0.4922)\phantom{**} &                (0.3103)\smallskip \\
$JUMP_t$        &                         &              -0.2537*** &                         &              -0.2288*** &                         &                 -0.0202 &                         &              -0.3194*** \\
                &                         &    (0.0228)\phantom{**} &                         &    (0.0233)\phantom{**} &                         &                 (0.034) &                         &    (0.0305)\phantom{**}\smallskip \\
$VIX_t$         &               -0.041*** &                         &                         &                         &              -0.0485*** &                         &                         &                         \\
                &     (0.0012)\phantom{*} &                         &                         &                         &    (0.0017)\phantom{**} &                         &                         &                        \smallskip \\
$\tilde{VIX_t}$ &                         &                         &                         &              -0.0871*** &                         &                         &                         &              -0.0941*** \\
                &                         &                         &                         &    (0.0021)\phantom{**} &                         &                         &                         &    (0.0023)\phantom{**}\smallskip \\
constant        &    \phantom{*}0.3713*** &              -0.1766*** &               -0.256*** &                 -0.0464 &                         &                         &                         &                         \\
                &    (0.0217)\phantom{**} &    (0.0144)\phantom{**} &     (0.0291)\phantom{*} &       (0.03)\phantom{*} &                         &                         &                         &                         \\
\medskip\\
year FE         &                      No &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes &                     Yes \\
\medskip\\
Observations    &               5,523,411 &               5,514,084 &               5,523,411 &               5,514,084 &               5,523,411 &               5,514,084 &               5,523,411 &               5,514,084 \\
$R^2$           &                  0.0002 &                       0 &                       0 &                  0.0003 &                  0.0004 &                  0.0002 &                  0.0002 &                  0.0008 \\
\bottomrule
\end{tabular}


==> table/perf_reg_panel_30.tex <==
\begin{tabular}{lcccccc}
\toprule \multicolumn{6}{c}{\parboxc{c}{0.7cm}{Panel A: $y_{t,i,t} = 100(MSE_{DBJM,i,t}-MSE_{HM,i,t})$}} \\\hline
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} \\
\midrule
$(b-a)_0$    &                         &                         &              -0.0526*** &                         &                         &              -0.0694*** \\
             &                         &                         &    (0.0018)\phantom{**} &                         &                         &    (0.0041)\phantom{**}\smallskip \\
$JUMP_0$     &                         &              -0.0051*** &                         &                         &              -0.0026*** &                         \\
             &                         &    (0.0002)\phantom{**} &                         &                         &    (0.0003)\phantom{**} &                        \smallskip \\
$VIX_0$      &              -0.0007*** &                         &                         &              -0.0009*** &                         &                         \\
             &    (0.0)\phantom{*****} &                         &                         &    (0.0)\phantom{*****} &                         &                        \smallskip \\
constant     &              -0.0009*** &              -0.0106*** &              -0.0065*** &                         &                         &                         \\
             &    (0.0002)\phantom{**} &    (0.0001)\phantom{**} &    (0.0002)\phantom{**} &                         &                         &                         \\
\medskip\\
year FE      &                      No &                      No &                      No &                     Yes &                     Yes &                     Yes \\
\medskip\\
Observations &               5,340,055 &               5,332,648 &               5,340,055 &               5,340,055 &               5,332,648 &               5,340,055 \\
$R^2$        &                   0.001 &                  0.0001 &                  0.0002 &                  0.0044 &                  0.0037 &                  0.0037 \bigskip \\ 


\hline \multicolumn{6}{c}{\parboxc{c}{0.6cm}{Panel B: $y_{i,t} = 100(MSE_{DBJM,i,t}-MSE_{RF,i,t})$}} \\\hline
{} & \parboxc{c}{0.6cm}{(1)} &          \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &          \parboxc{c}{0.6cm}{(5)} &          \parboxc{c}{0.6cm}{(6)} \\
\midrule
$(b-a)_0$    &                         &                                  &              19.2497*** &                         &                                  &                      162.4937*** \\
             &                         &                                  &    (0.9452)\phantom{**} &                         &                                  &  \phantom{*}(2.1408)\phantom{**}\smallskip \\
$JUMP_0$     &                         &                      -13.4754*** &                         &                         &                      -24.2848*** &                                  \\
             &                         &  \phantom{*}(0.099)\phantom{***} &                         &                         &  \phantom{*}(0.1473)\phantom{**} &                                 \smallskip \\
$VIX_0$      &              -0.3061*** &                                  &                         &              -0.2809*** &                                  &                                  \\
             &    (0.0053)\phantom{**} &                                  &                         &    (0.0074)\phantom{**} &                                  &                                 \smallskip \\
constant     &    \phantom{*}2.4645*** &             \phantom{*}4.5261*** &              -5.1236*** &                         &                                  &                                  \\
             &    (0.0945)\phantom{**} &             (0.0623)\phantom{**} &    (0.1265)\phantom{**} &                         &                                  &                                  \\
\medskip\\
year FE      &                      No &                               No &                      No &                     Yes &                              Yes &                              Yes \\
\medskip\\
Observations &               5,519,005 &                        5,509,678 &               5,519,005 &               5,519,005 &                        5,509,678 &                        5,519,005 \\
$R^2$        &                  0.0006 &                           0.0034 &                  0.0001 &                  0.0009 &                           0.0055 &                           0.0017 \\
\bottomrule
\end{tabular}


==> tex/lag_reg.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
dMAE-1 days   &    \phantom{*}0.1548*** &                         &                         &                         &                               &                                &                               \\
              &    (9.9065)\phantom{**} &                         &                         &                         &                               &                                &                              \smallskip \\
dMAE-2 days   &                         &    \phantom{*}0.0879*** &                         &                         &                               &                                &                               \\
              &                         &    (4.1082)\phantom{**} &                         &                         &                               &                                &                              \smallskip \\
dMAE-3 days   &                         &                         &    \phantom{*}0.1137*** &                         &                               &                                &                               \\
              &                         &                         &    (4.3957)\phantom{**} &                         &                               &                                &                              \smallskip \\
dMAE-4 days   &                         &                         &                         &    \phantom{*}0.0817*** &                               &                                &                               \\
              &                         &                         &                         &    (2.812)\phantom{***} &                               &                                &                              \smallskip \\
dMAE-5 days   &                         &                         &                         &                         &  \phantom{*}0.0308\phantom{*} &                                &                               \\
              &                         &                         &                         &                         &                      (0.9684) &                                &                              \smallskip \\
dMAE-30 days  &                         &                         &                         &                         &                               &  \phantom{*}-0.0469\phantom{*} &                               \\
              &                         &                         &                         &                         &                               &                      (-0.6927) &                              \smallskip \\
dMAE-252 days &                         &                         &                         &                         &                               &                                &  \phantom{*}0.201\phantom{**} \\
              &                         &                         &                         &                         &                               &                                &                      (0.7338) \\
\medskip\\
year FE       &                     Yes &                     Yes &                     Yes &                     Yes &                           Yes &                            Yes &                           Yes \\
\medskip\\
Observations  &                   4,028 &                   4,028 &                   4,028 &                   4,028 &                         4,028 &                          4,028 &                         4,028 \\
$R^2$         &                   0.033 &                  0.0135 &                  0.0141 &                  0.0113 &                        0.0096 &                         0.0094 &                        0.0095 \\
\bottomrule
\end{tabular}


==> tex/lag_reg_hbL1.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &        \parboxc{c}{0.6cm}{(7)} \\
\midrule
$y_{-1}$                                 &   \phantom{**}0.2759*** &                         &                         &                         &                         &                                &                                \\
                                         &   (16.5461)\phantom{**} &                         &                         &                         &                         &                                &                               \smallskip \\
$\frac{1}{2}  \sum_{t=-1}^{-2}  y_t$     &                         &     \phantom{*}0.064*** &                         &                         &                         &                                &                                \\
                                         &                         &     (2.9473)\phantom{*} &                         &                         &                         &                                &                               \smallskip \\
$\frac{1}{3}  \sum_{t=-1}^{-3}  y_t$     &                         &                         &    \phantom{*}0.1027*** &                         &                         &                                &                                \\
                                         &                         &                         &    (4.0356)\phantom{**} &                         &                         &                                &                               \smallskip \\
$\frac{1}{4}  \sum_{t=-1}^{-4}  y_t$     &                         &                         &                         &    \phantom{*}0.0892*** &                         &                                &                                \\
                                         &                         &                         &                         &    (3.1053)\phantom{**} &                         &                                &                               \smallskip \\
$\frac{1}{5}  \sum_{t=-1}^{-5}  y_t$     &                         &                         &                         &                         &     \phantom{*}0.0725** &                                &                                \\
                                         &                         &                         &                         &                         &     (2.3025)\phantom{*} &                                &                               \smallskip \\
$\frac{1}{30}  \sum_{t=-1}^{-30}  y_t$   &                         &                         &                         &                         &                         &  \phantom{*}-0.0854\phantom{*} &                                \\
                                         &                         &                         &                         &                         &                         &                      (-1.4963) &                               \smallskip \\
$\frac{1}{252}  \sum_{t=-1}^{-252}  y_t$ &                         &                         &                         &                         &                         &                                &  \phantom{*}-0.3074\phantom{*} \\
                                         &                         &                         &                         &                         &                         &                                &                      (-1.3489) \\
\medskip\\
year FE                                  &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes &                            Yes &                            Yes \\
\medskip\\
Observations                             &                   3,345 &                   3,345 &                   3,345 &                   3,345 &                   3,345 &                          3,345 &                          3,345 \\
$R^2$                                    &                  0.1587 &                  0.0918 &                  0.0939 &                  0.0921 &                  0.0909 &                           0.09 &                         0.0899 \\
\bottomrule
\end{tabular}


==> tex/lag_reg_hbL10.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
$y_{-1}$                                 &   \phantom{**}0.4034*** &                         &                         &                         &                               &                         &                               \\
                                         &   (25.4527)\phantom{**} &                         &                         &                         &                               &                         &                              \smallskip \\
$\frac{1}{2}  \sum_{t=-1}^{-2}  y_t$     &                         &   \phantom{**}0.2746*** &                         &                         &                               &                         &                               \\
                                         &                         &   (13.6805)\phantom{**} &                         &                         &                               &                         &                              \smallskip \\
$\frac{1}{3}  \sum_{t=-1}^{-3}  y_t$     &                         &                         &    \phantom{*}0.1932*** &                         &                               &                         &                               \\
                                         &                         &                         &    (8.4991)\phantom{**} &                         &                               &                         &                              \smallskip \\
$\frac{1}{4}  \sum_{t=-1}^{-4}  y_t$     &                         &                         &                         &    \phantom{*}0.1109*** &                               &                         &                               \\
                                         &                         &                         &                         &    (4.4497)\phantom{**} &                               &                         &                              \smallskip \\
$\frac{1}{5}  \sum_{t=-1}^{-5}  y_t$     &                         &                         &                         &                         &  \phantom{*}0.0199\phantom{*} &                         &                               \\
                                         &                         &                         &                         &                         &                      (0.7404) &                         &                              \smallskip \\
$\frac{1}{30}  \sum_{t=-1}^{-30}  y_t$   &                         &                         &                         &                         &                               &    \phantom{*}-0.206*** &                               \\
                                         &                         &                         &                         &                         &                               &    (-3.4483)\phantom{*} &                              \smallskip \\
$\frac{1}{252}  \sum_{t=-1}^{-252}  y_t$ &                         &                         &                         &                         &                               &                         &  \phantom{*}0.1609\phantom{*} \\
                                         &                         &                         &                         &                         &                               &                         &                      (0.6718) \\
\medskip\\
year FE                                  &                     Yes &                     Yes &                     Yes &                     Yes &                           Yes &                     Yes &                           Yes \\
\medskip\\
Observations                             &                   3,345 &                   3,345 &                   3,345 &                   3,345 &                         3,345 &                   3,345 &                         3,345 \\
$R^2$                                    &                  0.1946 &                  0.0891 &                  0.0583 &                  0.0435 &                         0.038 &                  0.0412 &                        0.0379 \\
\bottomrule
\end{tabular}


==> tex/lag_reg_hbL2.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
dMAE-1 days   &    \phantom{*}0.1548*** &                         &                         &                         &                               &                                &                               \\
              &    (9.9065)\phantom{**} &                         &                         &                         &                               &                                &                              \smallskip \\
dMAE-2 days   &                         &    \phantom{*}0.0879*** &                         &                         &                               &                                &                               \\
              &                         &    (4.1082)\phantom{**} &                         &                         &                               &                                &                              \smallskip \\
dMAE-3 days   &                         &                         &    \phantom{*}0.1137*** &                         &                               &                                &                               \\
              &                         &                         &    (4.3957)\phantom{**} &                         &                               &                                &                              \smallskip \\
dMAE-4 days   &                         &                         &                         &    \phantom{*}0.0817*** &                               &                                &                               \\
              &                         &                         &                         &    (2.812)\phantom{***} &                               &                                &                              \smallskip \\
dMAE-5 days   &                         &                         &                         &                         &  \phantom{*}0.0308\phantom{*} &                                &                               \\
              &                         &                         &                         &                         &                      (0.9684) &                                &                              \smallskip \\
dMAE-30 days  &                         &                         &                         &                         &                               &  \phantom{*}-0.0469\phantom{*} &                               \\
              &                         &                         &                         &                         &                               &                      (-0.6927) &                              \smallskip \\
dMAE-252 days &                         &                         &                         &                         &                               &                                &  \phantom{*}0.201\phantom{**} \\
              &                         &                         &                         &                         &                               &                                &                      (0.7338) \\
\medskip\\
year FE       &                     Yes &                     Yes &                     Yes &                     Yes &                           Yes &                            Yes &                           Yes \\
\medskip\\
Observations  &                   4,028 &                   4,028 &                   4,028 &                   4,028 &                         4,028 &                          4,028 &                         4,028 \\
$R^2$         &                   0.033 &                  0.0135 &                  0.0141 &                  0.0113 &                        0.0096 &                         0.0094 &                        0.0095 \\
\bottomrule
\end{tabular}


==> tex/lag_reg_obL1.tex <==
\begin{tabular}{lccccccc}
\toprule
{} &        \parboxc{c}{0.6cm}{(1)} &        \parboxc{c}{0.6cm}{(2)} &        \parboxc{c}{0.6cm}{(3)} &       \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
$y_{-1}$                                 &  \phantom{*}-0.0006\phantom{*} &                                &                                &                               &                               &                         &                               \\
                                         &                      (-0.0342) &                                &                                &                               &                               &                         &                              \smallskip \\
$\frac{1}{2}  \sum_{t=-1}^{-2}  y_t$     &                                &  \phantom{*}-0.0169\phantom{*} &                                &                               &                               &                         &                               \\
                                         &                                &                      (-0.6903) &                                &                               &                               &                         &                              \smallskip \\
$\frac{1}{3}  \sum_{t=-1}^{-3}  y_t$     &                                &                                &  \phantom{*}-0.0206\phantom{*} &                               &                               &                         &                               \\
                                         &                                &                                &                      (-0.6889) &                               &                               &                         &                              \smallskip \\
$\frac{1}{4}  \sum_{t=-1}^{-4}  y_t$     &                                &                                &                                &  \phantom{*}0.0243\phantom{*} &                               &                         &                               \\
                                         &                                &                                &                                &                      (0.7004) &                               &                         &                              \smallskip \\
$\frac{1}{5}  \sum_{t=-1}^{-5}  y_t$     &                                &                                &                                &                               &  \phantom{*}0.0302\phantom{*} &                         &                               \\
                                         &                                &                                &                                &                               &                      (0.7756) &                         &                              \smallskip \\
$\frac{1}{30}  \sum_{t=-1}^{-30}  y_t$   &                                &                                &                                &                               &                               &    \phantom{*}-0.1865** &                               \\
                                         &                                &                                &                                &                               &                               &    (-2.045)\phantom{**} &                              \smallskip \\
$\frac{1}{252}  \sum_{t=-1}^{-252}  y_t$ &                                &                                &                                &                               &                               &                         &  \phantom{*}0.1431\phantom{*} \\
                                         &                                &                                &                                &                               &                               &                         &                      (0.3456) \\
\medskip\\
year FE                                  &                            Yes &                            Yes &                            Yes &                           Yes &                           Yes &                     Yes &                           Yes \\
\medskip\\
Observations                             &                          3,345 &                          3,345 &                          3,345 &                         3,345 &                         3,345 &                   3,345 &                         3,345 \\
$R^2$                                    &                         0.0246 &                         0.0247 &                         0.0247 &                        0.0247 &                        0.0247 &                  0.0258 &                        0.0246 \\
\bottomrule
\end{tabular}


==> tex/lag_reg_obL10.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} &       \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
$y_{-1}$                                 &    \phantom{*}0.1309*** &                         &                               &                         &                         &                         &                               \\
                                         &    (7.6441)\phantom{**} &                         &                               &                         &                         &                         &                              \smallskip \\
$\frac{1}{2}  \sum_{t=-1}^{-2}  y_t$     &                         &    \phantom{*}0.0626*** &                               &                         &                         &                         &                               \\
                                         &                         &    (2.7297)\phantom{**} &                               &                         &                         &                         &                              \smallskip \\
$\frac{1}{3}  \sum_{t=-1}^{-3}  y_t$     &                         &                         &  \phantom{*}0.0396\phantom{*} &                         &                         &                         &                               \\
                                         &                         &                         &                      (1.4653) &                         &                         &                         &                              \smallskip \\
$\frac{1}{4}  \sum_{t=-1}^{-4}  y_t$     &                         &                         &                               &     \phantom{*}0.0782** &                         &                         &                               \\
                                         &                         &                         &                               &     (2.5552)\phantom{*} &                         &                         &                              \smallskip \\
$\frac{1}{5}  \sum_{t=-1}^{-5}  y_t$     &                         &                         &                               &                         &     \phantom{*}0.0697** &                         &                               \\
                                         &                         &                         &                               &                         &     (2.0668)\phantom{*} &                         &                              \smallskip \\
$\frac{1}{30}  \sum_{t=-1}^{-30}  y_t$   &                         &                         &                               &                         &                         &     \phantom{*}0.1471** &                               \\
                                         &                         &                         &                               &                         &                         &     (1.9642)\phantom{*} &                              \smallskip \\
$\frac{1}{252}  \sum_{t=-1}^{-252}  y_t$ &                         &                         &                               &                         &                         &                         &  \phantom{*}0.0077\phantom{*} \\
                                         &                         &                         &                               &                         &                         &                         &                      (0.0225) \\
\medskip\\
year FE                                  &                     Yes &                     Yes &                           Yes &                     Yes &                     Yes &                     Yes &                           Yes \\
\medskip\\
Observations                             &                   3,366 &                   3,366 &                         3,366 &                   3,366 &                   3,366 &                   3,366 &                         3,366 \\
$R^2$                                    &                  0.0462 &                  0.0317 &                        0.0302 &                  0.0314 &                  0.0308 &                  0.0307 &                        0.0295 \\
\bottomrule
\end{tabular}


==> tex/lag_reg_obL2.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} &        \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} &       \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} & \parboxc{c}{0.6cm}{(7)} \\
\midrule
dMAE-1 days   &       \phantom{*}0.0084 &                                &                         &                               &                         &                                &                         \\
              &                 (0.528) &                                &                         &                               &                         &                                &                        \smallskip \\
dMAE-2 days   &                         &  \phantom{*}-0.0252\phantom{*} &                         &                               &                         &                                &                         \\
              &                         &                      (-1.1247) &                         &                               &                         &                                &                        \smallskip \\
dMAE-3 days   &                         &                                &    \phantom{*}-0.0676** &                               &                         &                                &                         \\
              &                         &                                &    (-2.4564)\phantom{*} &                               &                         &                                &                        \smallskip \\
dMAE-4 days   &                         &                                &                         &  \phantom{*}0.016\phantom{**} &                         &                                &                         \\
              &                         &                                &                         &                      (0.4974) &                         &                                &                        \smallskip \\
dMAE-5 days   &                         &                                &                         &                               &      \phantom{*}-0.0259 &                                &                         \\
              &                         &                                &                         &                               &                (-0.719) &                                &                        \smallskip \\
dMAE-30 days  &                         &                                &                         &                               &                         &  \phantom{*}-0.1204\phantom{*} &                         \\
              &                         &                                &                         &                               &                         &                      (-1.6043) &                        \smallskip \\
dMAE-252 days &                         &                                &                         &                               &                         &                                &      \phantom{*}0.5416* \\
              &                         &                                &                         &                               &                         &                                &                (1.9115) \\
\medskip\\
year FE       &                     Yes &                            Yes &                     Yes &                           Yes &                     Yes &                            Yes &                     Yes \\
\medskip\\
Observations  &                   4,028 &                          4,028 &                   4,028 &                         4,028 &                   4,028 &                          4,028 &                   4,028 \\
$R^2$         &                  0.0141 &                         0.0144 &                  0.0155 &                        0.0141 &                  0.0142 &                         0.0147 &                   0.015 \\
\bottomrule
\end{tabular}


==> tex/lag_reghbL2.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &       \parboxc{c}{0.6cm}{(7)} \\
\midrule
os_r1(2)     &    \phantom{*}0.1548*** &                         &                         &                         &                               &                                &                               \\
             &    (9.9065)\phantom{**} &                         &                         &                         &                               &                                &                              \smallskip \\
os_r2(2)     &                         &    \phantom{*}0.0879*** &                         &                         &                               &                                &                               \\
             &                         &    (4.1082)\phantom{**} &                         &                         &                               &                                &                              \smallskip \\
os_r3(2)     &                         &                         &    \phantom{*}0.1137*** &                         &                               &                                &                               \\
             &                         &                         &    (4.3957)\phantom{**} &                         &                               &                                &                              \smallskip \\
os_r4(2)     &                         &                         &                         &    \phantom{*}0.0817*** &                               &                                &                               \\
             &                         &                         &                         &    (2.812)\phantom{***} &                               &                                &                              \smallskip \\
os_r5(2)     &                         &                         &                         &                         &  \phantom{*}0.0308\phantom{*} &                                &                               \\
             &                         &                         &                         &                         &                      (0.9684) &                                &                              \smallskip \\
os_r30(2)    &                         &                         &                         &                         &                               &  \phantom{*}-0.0469\phantom{*} &                               \\
             &                         &                         &                         &                         &                               &                      (-0.6927) &                              \smallskip \\
os_r252(2)   &                         &                         &                         &                         &                               &                                &  \phantom{*}0.201\phantom{**} \\
             &                         &                         &                         &                         &                               &                                &                      (0.7338) \\
\medskip\\
year FE      &                     Yes &                     Yes &                     Yes &                     Yes &                           Yes &                            Yes &                           Yes \\
\medskip\\
Observations &                   4,028 &                   4,028 &                   4,028 &                   4,028 &                         4,028 &                          4,028 &                         4,028 \\
$R^2$        &                   0.033 &                  0.0135 &                  0.0141 &                  0.0113 &                        0.0096 &                         0.0094 &                        0.0095 \\
\bottomrule
\end{tabular}


==> tex/mae_L1.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} &  Bates mae is &  Bates mae os &  Hest. mae is &  Hest. mae os &  OLS mae is &  OLS mae os \\
\midrule
mean &        0.0086 &        0.0119 &        0.0084 &        0.0118 &      0.0075 &      0.0128 \\
std  &        0.0082 &        0.0111 &        0.0069 &        0.0106 &      0.0089 &      0.0121 \\
min  &        0.0014 &        0.0017 &        0.0020 &        0.0025 &      0.0017 &      0.0023 \\
5\%   &        0.0030 &        0.0038 &        0.0034 &        0.0041 &      0.0030 &      0.0042 \\
10\%  &        0.0036 &        0.0044 &        0.0039 &        0.0048 &      0.0033 &      0.0049 \\
15\%  &        0.0039 &        0.0050 &        0.0043 &        0.0053 &      0.0035 &      0.0054 \\
20\%  &        0.0043 &        0.0055 &        0.0046 &        0.0058 &      0.0038 &      0.0059 \\
25\%  &        0.0047 &        0.0060 &        0.0050 &        0.0063 &      0.0040 &      0.0063 \\
30\%  &        0.0050 &        0.0065 &        0.0053 &        0.0068 &      0.0042 &      0.0068 \\
35\%  &        0.0053 &        0.0070 &        0.0057 &        0.0073 &      0.0045 &      0.0073 \\
40\%  &        0.0057 &        0.0076 &        0.0060 &        0.0078 &      0.0047 &      0.0078 \\
45\%  &        0.0061 &        0.0082 &        0.0063 &        0.0082 &      0.0050 &      0.0084 \\
50\%  &        0.0065 &        0.0088 &        0.0067 &        0.0088 &      0.0052 &      0.0091 \\
55\%  &        0.0070 &        0.0095 &        0.0071 &        0.0095 &      0.0056 &      0.0098 \\
60\%  &        0.0075 &        0.0103 &        0.0076 &        0.0101 &      0.0059 &      0.0108 \\
65\%  &        0.0082 &        0.0113 &        0.0081 &        0.0110 &      0.0064 &      0.0119 \\
70\%  &        0.0089 &        0.0123 &        0.0088 &        0.0121 &      0.0069 &      0.0131 \\
75\%  &        0.0097 &        0.0137 &        0.0095 &        0.0135 &      0.0077 &      0.0147 \\
80\%  &        0.0107 &        0.0156 &        0.0104 &        0.0154 &      0.0088 &      0.0169 \\
85\%  &        0.0122 &        0.0183 &        0.0119 &        0.0177 &      0.0103 &      0.0198 \\
90\%  &        0.0149 &        0.0221 &        0.0141 &        0.0213 &      0.0130 &      0.0240 \\
95\%  &        0.0207 &        0.0296 &        0.0188 &        0.0284 &      0.0189 &      0.0333 \\
max  &        0.1824 &        0.2571 &        0.1663 &        0.2595 &      0.2486 &      0.2612 \\
\bottomrule
\end{tabular}


==> tex/mae_L30.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} &  Bates mae is &  Bates mae os &  Hest. mae is &  Hest. mae os &  OLS mae is &  OLS mae os \\
\midrule
mean &        0.0086 &        0.0200 &        0.0084 &        0.0211 &      0.0075 &      0.0335 \\
std  &        0.0082 &        0.0193 &        0.0069 &        0.0245 &      0.0089 &      0.0351 \\
min  &        0.0014 &        0.0025 &        0.0020 &        0.0027 &      0.0017 &      0.0036 \\
5\%   &        0.0030 &        0.0054 &        0.0034 &        0.0053 &      0.0030 &      0.0069 \\
10\%  &        0.0036 &        0.0066 &        0.0039 &        0.0062 &      0.0033 &      0.0086 \\
15\%  &        0.0039 &        0.0076 &        0.0043 &        0.0071 &      0.0035 &      0.0102 \\
20\%  &        0.0043 &        0.0085 &        0.0046 &        0.0079 &      0.0038 &      0.0117 \\
25\%  &        0.0047 &        0.0093 &        0.0050 &        0.0087 &      0.0040 &      0.0133 \\
30\%  &        0.0050 &        0.0102 &        0.0053 &        0.0095 &      0.0042 &      0.0148 \\
35\%  &        0.0053 &        0.0112 &        0.0057 &        0.0103 &      0.0044 &      0.0165 \\
40\%  &        0.0057 &        0.0122 &        0.0060 &        0.0113 &      0.0047 &      0.0183 \\
45\%  &        0.0061 &        0.0133 &        0.0063 &        0.0123 &      0.0049 &      0.0203 \\
50\%  &        0.0065 &        0.0144 &        0.0067 &        0.0134 &      0.0052 &      0.0226 \\
55\%  &        0.0070 &        0.0158 &        0.0071 &        0.0149 &      0.0055 &      0.0251 \\
60\%  &        0.0075 &        0.0172 &        0.0076 &        0.0165 &      0.0059 &      0.0281 \\
65\%  &        0.0082 &        0.0189 &        0.0081 &        0.0183 &      0.0063 &      0.0314 \\
70\%  &        0.0089 &        0.0208 &        0.0088 &        0.0204 &      0.0069 &      0.0355 \\
75\%  &        0.0097 &        0.0233 &        0.0095 &        0.0232 &      0.0077 &      0.0405 \\
80\%  &        0.0107 &        0.0266 &        0.0104 &        0.0269 &      0.0088 &      0.0474 \\
85\%  &        0.0123 &        0.0310 &        0.0119 &        0.0325 &      0.0103 &      0.0560 \\
90\%  &        0.0150 &        0.0385 &        0.0141 &        0.0415 &      0.0130 &      0.0702 \\
95\%  &        0.0209 &        0.0543 &        0.0190 &        0.0626 &      0.0189 &      0.0971 \\
max  &        0.1824 &        0.3158 &        0.1663 &        0.3646 &      0.2486 &      0.4522 \\
\bottomrule
\end{tabular}


==> tex/mae_yy_L1.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} &  Bates mae is &  Bates mae os &  Hest. mae is &  Hest. mae os &  OLS mae is &  OLS mae os \\
year &               &               &               &               &             &             \\
\midrule
2001 &      0.013645 &      0.017190 &      0.012679 &      0.016218 &    0.010788 &    0.020395 \\
2002 &      0.014265 &      0.018462 &      0.013327 &      0.017524 &    0.012788 &    0.021684 \\
2003 &      0.008967 &      0.011593 &      0.008525 &      0.010991 &    0.008544 &    0.014614 \\
2004 &      0.008065 &      0.010219 &      0.007951 &      0.010027 &    0.007331 &    0.012356 \\
2005 &      0.006900 &      0.008562 &      0.006707 &      0.008375 &    0.005440 &    0.009950 \\
2006 &      0.008079 &      0.010216 &      0.007855 &      0.010077 &    0.006540 &    0.011343 \\
2007 &      0.008852 &      0.012422 &      0.008619 &      0.012326 &    0.007013 &    0.013074 \\
2008 &      0.016128 &      0.022512 &      0.014288 &      0.021550 &    0.012428 &    0.020676 \\
2009 &      0.008764 &      0.013139 &      0.008832 &      0.013240 &    0.009929 &    0.016554 \\
2010 &      0.006297 &      0.010888 &      0.006573 &      0.011116 &    0.006339 &    0.011019 \\
2011 &      0.009408 &      0.014956 &      0.008915 &      0.014791 &    0.009820 &    0.015577 \\
2012 &      0.006010 &      0.008872 &      0.006455 &      0.009211 &    0.005849 &    0.009643 \\
2013 &      0.005795 &      0.008075 &      0.006150 &      0.008358 &    0.005583 &    0.008798 \\
2014 &      0.005462 &      0.007764 &      0.005718 &      0.008093 &    0.004937 &    0.007697 \\
2015 &      0.005879 &      0.009570 &      0.006010 &      0.009728 &    0.004939 &    0.009543 \\
2016 &      0.007255 &      0.010110 &      0.007791 &      0.010679 &    0.006380 &    0.010473 \\
2017 &      0.009005 &      0.010067 &      0.008192 &      0.009321 &    0.005653 &    0.007941 \\
2018 &      0.009016 &      0.012563 &      0.008840 &      0.012420 &    0.006380 &    0.010381 \\
2019 &      0.006206 &      0.009005 &      0.006596 &      0.009445 &    0.006146 &    0.010930 \\
\bottomrule
\end{tabular}


==> tex/mae_yy_L30.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} &  Bates mae is &  Bates mae os &  Hest. mae is &  Hest. mae os &  OLS mae is &  OLS mae os \\
year &               &               &               &               &             &             \\
\midrule
2001 &      0.013645 &      0.030796 &      0.012679 &      0.031595 &    0.010788 &    0.046929 \\
2002 &      0.014265 &      0.033881 &      0.013327 &      0.032725 &    0.012788 &    0.046727 \\
2003 &      0.008967 &      0.024761 &      0.008525 &      0.023490 &    0.008544 &    0.029889 \\
2004 &      0.008065 &      0.018050 &      0.007951 &      0.018056 &    0.007331 &    0.020741 \\
2005 &      0.006900 &      0.015024 &      0.006707 &      0.014661 &    0.005440 &    0.018593 \\
2006 &      0.008079 &      0.015199 &      0.007855 &      0.016835 &    0.006540 &    0.019929 \\
2007 &      0.008852 &      0.021212 &      0.008619 &      0.021762 &    0.007013 &    0.035266 \\
2008 &      0.016128 &      0.041417 &      0.014288 &      0.050875 &    0.012428 &    0.072625 \\
2009 &      0.008764 &      0.030953 &      0.008832 &      0.028686 &    0.009929 &    0.045484 \\
2010 &      0.006297 &      0.017537 &      0.006573 &      0.016970 &    0.006339 &    0.036976 \\
2011 &      0.009408 &      0.019632 &      0.008915 &      0.024436 &    0.009820 &    0.042953 \\
2012 &      0.006010 &      0.015036 &      0.006455 &      0.014912 &    0.005849 &    0.030592 \\
2013 &      0.005795 &      0.011479 &      0.006150 &      0.013024 &    0.005583 &    0.021286 \\
2014 &      0.005462 &      0.010647 &      0.005718 &      0.011838 &    0.004937 &    0.021538 \\
2015 &      0.005879 &      0.013070 &      0.006010 &      0.014417 &    0.004939 &    0.033694 \\
2016 &      0.007255 &      0.014292 &      0.007791 &      0.017192 &    0.006380 &    0.031363 \\
2017 &      0.008947 &      0.013394 &      0.008159 &      0.012756 &    0.005636 &    0.015217 \\
2018 &      0.009354 &      0.016776 &      0.009008 &      0.018562 &    0.005862 &    0.035385 \\
2019 &      0.006205 &      0.013395 &      0.006642 &      0.014612 &    0.006317 &    0.030081 \\
\bottomrule
\end{tabular}


==> tex/perc_hbL1.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  in sample &     os(1) &     os(2) &     os(3) &     os(4) &     os(5) &    os(10) &    os(30) \\
\midrule
mean &  -0.006552 & -0.004731 & -0.003810 & -0.003254 & -0.003182 & -0.002792 & -0.002372 & -0.001633 \\
std  &   0.007041 &  0.009680 &  0.009862 &  0.009773 &  0.009747 &  0.009792 &  0.009979 &  0.009296 \\
5\%   &  -0.021601 & -0.021668 & -0.020736 & -0.019664 & -0.019781 & -0.019623 & -0.019247 & -0.015896 \\
10\%  &  -0.015928 & -0.016415 & -0.015434 & -0.014411 & -0.014478 & -0.014266 & -0.014004 & -0.011493 \\
15\%  &  -0.012083 & -0.013338 & -0.012548 & -0.011797 & -0.011530 & -0.011278 & -0.010742 & -0.009148 \\
20\%  &  -0.010065 & -0.010959 & -0.010302 & -0.009635 & -0.009743 & -0.009403 & -0.008744 & -0.007545 \\
25\%  &  -0.008464 & -0.009202 & -0.008655 & -0.008246 & -0.008081 & -0.007873 & -0.007170 & -0.006241 \\
30\%  &  -0.007374 & -0.007949 & -0.007280 & -0.007076 & -0.006975 & -0.006712 & -0.006010 & -0.005330 \\
35\%  &  -0.006436 & -0.006856 & -0.006286 & -0.006032 & -0.005746 & -0.005415 & -0.004970 & -0.004294 \\
40\%  &  -0.005696 & -0.005799 & -0.005127 & -0.004845 & -0.004693 & -0.004427 & -0.003998 & -0.003510 \\
45\%  &  -0.004930 & -0.004927 & -0.004160 & -0.003805 & -0.003689 & -0.003386 & -0.003075 & -0.002751 \\
50\%  &  -0.004310 & -0.004147 & -0.003411 & -0.002934 & -0.002724 & -0.002395 & -0.002240 & -0.001926 \\
55\%  &  -0.003787 & -0.003093 & -0.002511 & -0.002007 & -0.001810 & -0.001258 & -0.001437 & -0.001084 \\
60\%  &  -0.003245 & -0.002226 & -0.001446 & -0.000894 & -0.000875 & -0.000359 & -0.000479 & -0.000244 \\
65\%  &  -0.002810 & -0.001326 & -0.000523 &  0.000305 &  0.000200 &  0.000691 &  0.000537 &  0.000715 \\
70\%  &  -0.002377 & -0.000322 &  0.000558 &  0.001419 &  0.001283 &  0.001779 &  0.001808 &  0.001720 \\
75\%  &  -0.001950 &  0.000957 &  0.001807 &  0.002613 &  0.002498 &  0.003018 &  0.002873 &  0.003042 \\
80\%  &  -0.001498 &  0.002345 &  0.003310 &  0.003809 &  0.003828 &  0.004283 &  0.004480 &  0.004408 \\
85\%  &  -0.001083 &  0.004088 &  0.005116 &  0.005647 &  0.005329 &  0.005917 &  0.006360 &  0.006281 \\
90\%  &  -0.000630 &  0.006132 &  0.007383 &  0.007732 &  0.007730 &  0.008123 &  0.008857 &  0.008848 \\
95\%  &  -0.000149 &  0.009299 &  0.010928 &  0.011255 &  0.011597 &  0.011765 &  0.013454 &  0.013665 \\
\bottomrule
\end{tabular}


==> tex/perc_hbL10.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  in sample &     os(1) &     os(2) &     os(3) &     os(4) &     os(5) &    os(10) &    os(30) \\
\midrule
mean &  -0.006552 & -0.004731 & -0.003810 & -0.003254 & -0.003182 & -0.002792 & -0.002372 & -0.001633 \\
std  &   0.007041 &  0.009680 &  0.009862 &  0.009773 &  0.009747 &  0.009792 &  0.009979 &  0.009296 \\
5\%   &  -0.021601 & -0.021668 & -0.020736 & -0.019664 & -0.019781 & -0.019623 & -0.019247 & -0.015896 \\
10\%  &  -0.015928 & -0.016415 & -0.015434 & -0.014411 & -0.014478 & -0.014266 & -0.014004 & -0.011493 \\
15\%  &  -0.012083 & -0.013338 & -0.012548 & -0.011797 & -0.011530 & -0.011278 & -0.010742 & -0.009148 \\
20\%  &  -0.010065 & -0.010959 & -0.010302 & -0.009635 & -0.009743 & -0.009403 & -0.008744 & -0.007545 \\
25\%  &  -0.008464 & -0.009202 & -0.008655 & -0.008246 & -0.008081 & -0.007873 & -0.007170 & -0.006241 \\
30\%  &  -0.007374 & -0.007949 & -0.007280 & -0.007076 & -0.006975 & -0.006712 & -0.006010 & -0.005330 \\
35\%  &  -0.006436 & -0.006856 & -0.006286 & -0.006032 & -0.005746 & -0.005415 & -0.004970 & -0.004294 \\
40\%  &  -0.005696 & -0.005799 & -0.005127 & -0.004845 & -0.004693 & -0.004427 & -0.003998 & -0.003510 \\
45\%  &  -0.004930 & -0.004927 & -0.004160 & -0.003805 & -0.003689 & -0.003386 & -0.003075 & -0.002751 \\
50\%  &  -0.004310 & -0.004147 & -0.003411 & -0.002934 & -0.002724 & -0.002395 & -0.002240 & -0.001926 \\
55\%  &  -0.003787 & -0.003093 & -0.002511 & -0.002007 & -0.001810 & -0.001258 & -0.001437 & -0.001084 \\
60\%  &  -0.003245 & -0.002226 & -0.001446 & -0.000894 & -0.000875 & -0.000359 & -0.000479 & -0.000244 \\
65\%  &  -0.002810 & -0.001326 & -0.000523 &  0.000305 &  0.000200 &  0.000691 &  0.000537 &  0.000715 \\
70\%  &  -0.002377 & -0.000322 &  0.000558 &  0.001419 &  0.001283 &  0.001779 &  0.001808 &  0.001720 \\
75\%  &  -0.001950 &  0.000957 &  0.001807 &  0.002613 &  0.002498 &  0.003018 &  0.002873 &  0.003042 \\
80\%  &  -0.001498 &  0.002345 &  0.003310 &  0.003809 &  0.003828 &  0.004283 &  0.004480 &  0.004408 \\
85\%  &  -0.001083 &  0.004088 &  0.005116 &  0.005647 &  0.005329 &  0.005917 &  0.006360 &  0.006281 \\
90\%  &  -0.000630 &  0.006132 &  0.007383 &  0.007732 &  0.007730 &  0.008123 &  0.008857 &  0.008848 \\
95\%  &  -0.000149 &  0.009299 &  0.010928 &  0.011255 &  0.011597 &  0.011765 &  0.013454 &  0.013665 \\
\bottomrule
\end{tabular}


==> tex/perc_obL1.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  in sample &     os(1) &     os(2) &     os(3) &     os(4) &     os(5) &    os(10) &    os(30) \\
\midrule
mean &   0.062263 &  0.005296 &  0.000224 & -0.001552 & -0.001997 & -0.001300 & -0.007317 & -0.006961 \\
std  &   0.029569 &  0.022789 &  0.021331 &  0.020014 &  0.020161 &  0.019804 &  0.026467 &  0.019985 \\
5\%   &   0.031555 & -0.031395 & -0.033730 & -0.032257 & -0.032876 & -0.032670 & -0.046960 & -0.035819 \\
10\%  &   0.035879 & -0.021649 & -0.023673 & -0.024396 & -0.024106 & -0.022921 & -0.030316 & -0.026364 \\
15\%  &   0.039527 & -0.015734 & -0.018030 & -0.018930 & -0.019263 & -0.017924 & -0.023014 & -0.021076 \\
20\%  &   0.042435 & -0.011141 & -0.014112 & -0.015387 & -0.015415 & -0.013981 & -0.019006 & -0.017731 \\
25\%  &   0.045002 & -0.007470 & -0.011158 & -0.012536 & -0.012469 & -0.011394 & -0.015341 & -0.014626 \\
30\%  &   0.047346 & -0.004470 & -0.008554 & -0.009943 & -0.009840 & -0.009107 & -0.012750 & -0.012421 \\
35\%  &   0.049430 & -0.001682 & -0.005833 & -0.007260 & -0.007678 & -0.006718 & -0.010446 & -0.010494 \\
40\%  &   0.051850 &  0.001172 & -0.003845 & -0.005272 & -0.005844 & -0.004798 & -0.008075 & -0.008642 \\
45\%  &   0.054220 &  0.003381 & -0.001529 & -0.003239 & -0.003880 & -0.002807 & -0.006011 & -0.006857 \\
50\%  &   0.056556 &  0.005631 &  0.000373 & -0.001398 & -0.001886 & -0.000876 & -0.004159 & -0.005394 \\
55\%  &   0.058830 &  0.007939 &  0.002412 &  0.000330 &  0.000037 &  0.000851 & -0.002224 & -0.003754 \\
60\%  &   0.061466 &  0.010086 &  0.004553 &  0.002300 &  0.002079 &  0.002646 & -0.000482 & -0.002206 \\
65\%  &   0.064877 &  0.012777 &  0.006761 &  0.004593 &  0.004108 &  0.004607 &  0.001135 & -0.000619 \\
70\%  &   0.068101 &  0.015648 &  0.009180 &  0.006539 &  0.006180 &  0.006615 &  0.003255 &  0.001187 \\
75\%  &   0.072166 &  0.018624 &  0.011676 &  0.009157 &  0.008454 &  0.008746 &  0.005558 &  0.002915 \\
80\%  &   0.076429 &  0.021834 &  0.015055 &  0.012004 &  0.010973 &  0.011689 &  0.007806 &  0.004944 \\
85\%  &   0.082483 &  0.025891 &  0.018340 &  0.015551 &  0.014635 &  0.015294 &  0.010781 &  0.007667 \\
90\%  &   0.091562 &  0.031075 &  0.023537 &  0.020573 &  0.019001 &  0.019775 &  0.014712 &  0.011086 \\
95\%  &   0.110916 &  0.039726 &  0.031007 &  0.029383 &  0.026713 &  0.027646 &  0.022314 &  0.017183 \\
\bottomrule
\end{tabular}


==> tex/perc_obL10.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  in sample &     os(1) &     os(2) &     os(3) &     os(4) &     os(5) &    os(10) &    os(30) \\
\midrule
mean &   0.059155 &  0.003480 & -0.000935 & -0.002584 & -0.002946 & -0.002376 & -0.007715 & -0.007355 \\
std  &   0.029188 &  0.022626 &  0.021249 &  0.020320 &  0.020351 &  0.019915 &  0.026730 &  0.020406 \\
5\%   &   0.028550 & -0.033175 & -0.035056 & -0.034401 & -0.034380 & -0.034563 & -0.048241 & -0.037074 \\
10\%  &   0.033021 & -0.023294 & -0.025192 & -0.025597 & -0.025769 & -0.024420 & -0.030483 & -0.027083 \\
15\%  &   0.036722 & -0.016857 & -0.018988 & -0.019946 & -0.020082 & -0.018959 & -0.023307 & -0.021490 \\
20\%  &   0.039633 & -0.012420 & -0.014817 & -0.016225 & -0.016495 & -0.015045 & -0.019236 & -0.018054 \\
25\%  &   0.042243 & -0.008825 & -0.012059 & -0.013531 & -0.013474 & -0.012302 & -0.015837 & -0.014882 \\
30\%  &   0.044522 & -0.005640 & -0.009426 & -0.010677 & -0.010814 & -0.009772 & -0.012995 & -0.012769 \\
35\%  &   0.046933 & -0.003083 & -0.006762 & -0.007977 & -0.008428 & -0.007639 & -0.010639 & -0.010726 \\
40\%  &   0.049242 & -0.000438 & -0.004332 & -0.005829 & -0.006481 & -0.005461 & -0.008411 & -0.008827 \\
45\%  &   0.051418 &  0.001828 & -0.002203 & -0.003886 & -0.004414 & -0.003689 & -0.006169 & -0.007124 \\
50\%  &   0.053641 &  0.004009 & -0.000284 & -0.001995 & -0.002547 & -0.001762 & -0.004348 & -0.005677 \\
55\%  &   0.056021 &  0.006117 &  0.001621 & -0.000045 & -0.000513 &  0.000234 & -0.002428 & -0.004030 \\
60\%  &   0.058705 &  0.008639 &  0.003601 &  0.001846 &  0.001370 &  0.002036 & -0.000646 & -0.002362 \\
65\%  &   0.061763 &  0.011282 &  0.005727 &  0.003973 &  0.003310 &  0.003827 &  0.000907 & -0.000769 \\
70\%  &   0.065050 &  0.013793 &  0.008036 &  0.006167 &  0.005478 &  0.005770 &  0.002897 &  0.000875 \\
75\%  &   0.068625 &  0.016519 &  0.010444 &  0.008312 &  0.007667 &  0.007862 &  0.004946 &  0.002795 \\
80\%  &   0.073123 &  0.019867 &  0.013414 &  0.011196 &  0.010167 &  0.010625 &  0.007528 &  0.004817 \\
85\%  &   0.078928 &  0.023788 &  0.017017 &  0.014844 &  0.013668 &  0.013910 &  0.010427 &  0.007331 \\
90\%  &   0.087559 &  0.028960 &  0.021833 &  0.019546 &  0.018232 &  0.019044 &  0.013923 &  0.010765 \\
95\%  &   0.105917 &  0.037038 &  0.028680 &  0.027103 &  0.025682 &  0.026585 &  0.021487 &  0.017284 \\
\bottomrule
\end{tabular}


==> tex/perf_reg_1.tex <==
\begin{tabular}{lcccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} &       \parboxc{c}{0.6cm}{(3)} &        \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} \\
\midrule
ba           &                         &                         &  \phantom{*}0.0001\phantom{*} &                                &                         &   \phantom{*}0.0006\phantom{*} \\
             &                         &                         &                      (0.0447) &                                &                         &                       (0.2769)\smallskip \\
ba(2)        &                         &                         &                               &  \phantom{*}-0.0009\phantom{*} &                         &  \phantom{*}-0.0004\phantom{*} \\
             &                         &                         &                               &                      (-0.5033) &                         &                      (-0.1917)\smallskip \\
dVatm        &                         &    \phantom{*}-0.0055** &                               &                                &                         &           \phantom{*}-0.0055** \\
             &                         &    (-2.4205)\phantom{*} &                               &                                &                         &           (-2.3632)\phantom{*}\smallskip \\
dba          &       \phantom{*}0.0007 &                         &                               &                                &                         &   \phantom{*}0.0018\phantom{*} \\
             &                 (0.361) &                         &                               &                                &                         &                       (0.8534)\smallskip \\
dMAE-1 days  &                         &                         &                               &                                &    \phantom{*}0.1548*** &           \phantom{*}0.1542*** \\
             &                         &                         &                               &                                &    (9.9065)\phantom{**} &           (9.8652)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                           Yes &                            Yes &                     Yes &                            Yes \\
\medskip\\
Observations &                   4,028 &                   4,028 &                         4,028 &                          4,028 &                   4,028 &                          4,028 \\
$R^2$        &                  0.0094 &                  0.0108 &                        0.0093 &                         0.0094 &                   0.033 &                         0.0335 \\
\bottomrule
\end{tabular}


==> tex/perf_reg_hbL1.tex <==
\begin{tabular}{lcccccccccc}
\toprule
{} &       \parboxc{c}{0.6cm}{(1)} &        \parboxc{c}{0.6cm}{(2)} &        \parboxc{c}{0.6cm}{(3)} &       \parboxc{c}{0.6cm}{(4)} &        \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &        \parboxc{c}{0.6cm}{(7)} &        \parboxc{c}{0.6cm}{(8)} &       \parboxc{c}{0.6cm}{(9)} &       \parboxc{c}{0.6cm}{(10)} \\
\midrule
one              &         \phantom{**}-0.002*** &         \phantom{**}-0.0014*** &         \phantom{**}-0.0012*** &        \phantom{**}-0.0012*** &         \phantom{**}-0.0022*** &                                &                                &                                &                               &                                \\
                 &         (-13.6817)\phantom{*} &         (-13.436)\phantom{***} &         (-16.8439)\phantom{**} &        (-20.6757)\phantom{**} &         (-13.2975)\phantom{**} &                                &                                &                                &                               &                               \smallskip \\
$d(b-a)$         &  \phantom{*}0.0001\phantom{*} &                                &                                &                               &   \phantom{*}0.0001\phantom{*} &  \phantom{*}-0.0\phantom{****} &                                &                                &                               &  \phantom{*}-0.0\phantom{****} \\
                 &                      (0.7948) &                                &                                &                               &                       (0.6395) &                      (-0.0015) &                                &                                &                               &                      (-0.1824)\smallskip \\
$(b-a)_{t=0}$    &            \phantom{*}0.0047* &                                &                                &                               &   \phantom{*}0.0038\phantom{*} &  \phantom{*}-0.001\phantom{**} &                                &                                &                               &  \phantom{*}-0.0019\phantom{*} \\
                 &                      (1.7952) &                                &                                &                               &                       (1.4465) &                      (-0.3517) &                                &                                &                               &                      (-0.6677)\smallskip \\
$(b-a)_{t=\tau}$ &          \phantom{*}0.0078*** &                                &                                &                               &           \phantom{*}0.0073*** &   \phantom{*}0.0036\phantom{*} &                                &                                &                               &   \phantom{*}0.003\phantom{**} \\
                 &          (3.0819)\phantom{**} &                                &                                &                               &           (2.9034)\phantom{**} &                       (1.3853) &                                &                                &                               &                       (1.1258)\smallskip \\
$VIX_0$          &                               &  \phantom{*}-0.0013\phantom{*} &                                &                               &   \phantom{*}0.0003\phantom{*} &                                &  \phantom{*}-0.0015\phantom{*} &                                &                               &              \phantom{*}0.0003 \\
                 &                               &                      (-0.5349) &                                &                               &                       (0.1055) &                                &                      (-0.6095) &                                &                               &                        (0.138)\smallskip \\
$VIX_{\tau}$     &                               &              \phantom{*}0.0029 &                                &                               &   \phantom{*}0.0031\phantom{*} &                                &   \phantom{*}0.0023\phantom{*} &                                &                               &   \phantom{*}0.0034\phantom{*} \\
                 &                               &                        (1.212) &                                &                               &                       (1.2431) &                                &                       (0.9638) &                                &                               &                       (1.3571)\smallskip \\
$dVIX$           &                               &  \phantom{*}-0.0008\phantom{*} &                                &                               &  \phantom{*}-0.0011\phantom{*} &                                &   \phantom{*}0.0002\phantom{*} &                                &                               &  \phantom{*}-0.0002\phantom{*} \\
                 &                               &                      (-0.9071) &                                &                               &                      (-1.2177) &                                &                       (0.1961) &                                &                               &                      (-0.1979)\smallskip \\
$JUMP_0$         &                               &                                &  \phantom{*}-0.0143\phantom{*} &                               &   \phantom{*}0.0952\phantom{*} &                                &                                &  \phantom{*}-0.0293\phantom{*} &                               &   \phantom{*}0.0918\phantom{*} \\
                 &                               &                                &                      (-0.1301) &                               &                       (0.8259) &                                &                                &                      (-0.2712) &                               &                       (0.7843)\smallskip \\
$JUMP_{\tau}$    &                               &                                &   \phantom{*}0.0239\phantom{*} &                               &  \phantom{*}-0.138\phantom{**} &                                &                                &   \phantom{*}0.0162\phantom{*} &                               &  \phantom{*}-0.1421\phantom{*} \\
                 &                               &                                &                       (0.2175) &                               &                      (-1.1662) &                                &                                &                       (0.1504) &                               &                      (-1.1686)\smallskip \\
$dJUMP$          &                               &                                &                                &  \phantom{*}0.0017\phantom{*} &  \phantom{*}-0.0001\phantom{*} &                                &                                &                                &  \phantom{*}0.0004\phantom{*} &  \phantom{*}-0.0006\phantom{*} \\
                 &                               &                                &                                &                      (1.0492) &                      (-0.0704) &                                &                                &                                &                      (0.2623) &                      (-0.3685) \\
\medskip\\
year FE          &                            No &                             No &                             No &                            No &                             No &                            Yes &                            Yes &                            Yes &                           Yes &                            Yes \\
\medskip\\
Observations     &                         3,909 &                          3,909 &                          3,909 &                         3,909 &                          3,909 &                          3,909 &                          3,909 &                          3,909 &                         3,909 &                          3,909 \\
$R^2$            &                        0.0094 &                         0.0026 &                        -0.0001 &                             0 &                         0.0116 &                         0.0395 &                         0.0395 &                         0.0396 &                        0.0395 &                         0.0405 \\
\bottomrule
\end{tabular}


==> tex/perf_reg_hbL10.tex <==
\begin{tabular}{lcccccccccc}
\toprule
{} &       \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} &        \parboxc{c}{0.6cm}{(3)} &        \parboxc{c}{0.6cm}{(4)} &        \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} & \parboxc{c}{0.6cm}{(7)} &        \parboxc{c}{0.6cm}{(8)} &        \parboxc{c}{0.6cm}{(9)} &       \parboxc{c}{0.6cm}{(10)} \\
\midrule
one              &         \phantom{*}-0.0053*** &    \phantom{*}-0.002*** &          \phantom{*}-0.0025*** &          \phantom{*}-0.0022*** &          \phantom{*}-0.0047*** &                                &                         &                                &                                &                                \\
                 &         (-8.3102)\phantom{**} &    (-4.6583)\phantom{*} &          (-8.6273)\phantom{**} &          (-8.8896)\phantom{**} &          (-6.3477)\phantom{**} &                                &                         &                                &                                &                               \smallskip \\
$d(b-a)$         &  \phantom{*}0.0005\phantom{*} &                         &                                &                                &   \phantom{*}0.0006\phantom{*} &   \phantom{*}0.0001\phantom{*} &                         &                                &                                &   \phantom{*}0.0002\phantom{*} \\
                 &                      (1.2526) &                         &                                &                                &                       (1.5365) &                       (0.1406) &                         &                                &                                &                       (0.5705)\smallskip \\
$(b-a)_{t=0}$    &           \phantom{*}0.0181** &                         &                                &                                &             \phantom{*}0.0156* &  \phantom{*}-0.006\phantom{**} &                         &                                &                                &  \phantom{*}-0.0033\phantom{*} \\
                 &           (1.9924)\phantom{*} &                         &                                &                                &                       (1.6709) &                      (-0.5856) &                         &                                &                                &                      (-0.3106)\smallskip \\
$(b-a)_{t=\tau}$ &          \phantom{*}0.0243*** &                         &                                &                                &           \phantom{*}0.0288*** &   \phantom{*}0.0057\phantom{*} &                         &                                &                                &   \phantom{*}0.0126\phantom{*} \\
                 &          (2.6953)\phantom{**} &                         &                                &                                &           (3.1685)\phantom{**} &                       (0.5792) &                         &                                &                                &                       (1.2683)\smallskip \\
$VIX_0$          &                               &     \phantom{*}0.0114** &                                &                                &            \phantom{*}0.0117** &                                &     \phantom{*}0.0095** &                                &                                &   \phantom{*}0.0082\phantom{*} \\
                 &                               &     (2.5155)\phantom{*} &                                &                                &            (2.1318)\phantom{*} &                                &     (2.0376)\phantom{*} &                                &                                &                       (1.3524)\smallskip \\
$VIX_{\tau}$     &                               &     \phantom{*}-0.0082* &                                &                                &          \phantom{*}-0.0129*** &                                &    \phantom{*}-0.0109** &                                &                                &           \phantom{*}-0.0126** \\
                 &                               &               (-1.8102) &                                &                                &          (-2.6357)\phantom{**} &                                &    (-2.2654)\phantom{*} &                                &                                &           (-2.3182)\phantom{*}\smallskip \\
$dVIX$           &                               &   \phantom{*}-0.0068*** &                                &                                &          \phantom{*}-0.0066*** &                                &   \phantom{*}-0.0054*** &                                &                                &          \phantom{*}-0.0058*** \\
                 &                               &   (-4.1281)\phantom{**} &                                &                                &          (-3.9302)\phantom{**} &                                &   (-3.207)\phantom{***} &                                &                                &          (-3.3498)\phantom{**}\smallskip \\
$JUMP_0$         &                               &                         &   \phantom{*}0.1015\phantom{*} &                                &   \phantom{*}0.0189\phantom{*} &                                &                         &   \phantom{*}0.1061\phantom{*} &                                &   \phantom{*}0.0113\phantom{*} \\
                 &                               &                         &                       (1.2048) &                                &                       (0.2023) &                                &                         &                       (1.2504) &                                &                       (0.1192)\smallskip \\
$JUMP_{\tau}$    &                               &                         &  \phantom{*}-0.0583\phantom{*} &                                &   \phantom{*}0.0097\phantom{*} &                                &                         &  \phantom{*}-0.0961\phantom{*} &                                &   \phantom{*}0.0422\phantom{*} \\
                 &                               &                         &                      (-0.6904) &                                &                       (0.0904) &                                &                         &                      (-1.1083) &                                &                       (0.3523)\smallskip \\
$dJUMP$          &                               &                         &                                &  \phantom{*}-0.0\phantom{****} &  \phantom{*}-0.0001\phantom{*} &                                &                         &                                &  \phantom{*}-0.0001\phantom{*} &   \phantom{*}0.0002\phantom{*} \\
                 &                               &                         &                                &                      (-0.0115) &                      (-0.0653) &                                &                         &                                &                      (-0.1185) &                       (0.1851) \\
\medskip\\
year FE          &                            No &                      No &                             No &                             No &                             No &                            Yes &                     Yes &                            Yes &                            Yes &                            Yes \\
\medskip\\
Observations     &                         3,345 &                   3,345 &                          3,345 &                          3,345 &                          3,345 &                          3,345 &                   3,345 &                          3,345 &                          3,345 &                          3,345 \\
$R^2$            &                         0.007 &                   0.006 &                         0.0002 &                        -0.0003 &                         0.0127 &                         0.0375 &                  0.0422 &                          0.038 &                         0.0378 &                         0.0413 \\
\bottomrule
\end{tabular}


==> tex/perf_reg_hbL2.tex <==
\begin{tabular}{lcccccc}
\toprule
{} & \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} &       \parboxc{c}{0.6cm}{(3)} &        \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} \\
\midrule
b-a          &                         &                         &  \phantom{*}0.0001\phantom{*} &                                &                         &   \phantom{*}0.0006\phantom{*} \\
             &                         &                         &                      (0.0447) &                                &                         &                       (0.2769)\smallskip \\
b-a(2)       &                         &                         &                               &  \phantom{*}-0.0009\phantom{*} &                         &  \phantom{*}-0.0004\phantom{*} \\
             &                         &                         &                               &                      (-0.5033) &                         &                      (-0.1917)\smallskip \\
dVatm        &                         &    \phantom{*}-0.0055** &                               &                                &                         &           \phantom{*}-0.0055** \\
             &                         &    (-2.4205)\phantom{*} &                               &                                &                         &           (-2.3632)\phantom{*}\smallskip \\
dba          &       \phantom{*}0.0007 &                         &                               &                                &                         &   \phantom{*}0.0018\phantom{*} \\
             &                 (0.361) &                         &                               &                                &                         &                       (0.8534)\smallskip \\
dMAE-1 days  &                         &                         &                               &                                &    \phantom{*}0.1548*** &           \phantom{*}0.1542*** \\
             &                         &                         &                               &                                &    (9.9065)\phantom{**} &           (9.8652)\phantom{**} \\
\medskip\\
year FE      &                     Yes &                     Yes &                           Yes &                            Yes &                     Yes &                            Yes \\
\medskip\\
Observations &                   4,028 &                   4,028 &                         4,028 &                          4,028 &                   4,028 &                          4,028 \\
$R^2$        &                  0.0094 &                  0.0108 &                        0.0093 &                         0.0094 &                   0.033 &                         0.0335 \\
\bottomrule
\end{tabular}


==> tex/perf_reg_obL1.tex <==
\begin{tabular}{lcccccccccc}
\toprule
{} &        \parboxc{c}{0.6cm}{(1)} &        \parboxc{c}{0.6cm}{(2)} &       \parboxc{c}{0.6cm}{(3)} &       \parboxc{c}{0.6cm}{(4)} &        \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &        \parboxc{c}{0.6cm}{(7)} &        \parboxc{c}{0.6cm}{(8)} &        \parboxc{c}{0.6cm}{(9)} &       \parboxc{c}{0.6cm}{(10)} \\
\midrule
one              &            \phantom{*}0.006*** &           \phantom{*}0.0034*** &           \phantom{*}0.004*** &         \phantom{**}0.0061*** &            \phantom{*}0.005*** &                                &                                &                                &                                &                                \\
                 &            (4.4491)\phantom{*} &           (3.7131)\phantom{**} &           (6.3201)\phantom{*} &         (12.0054)\phantom{**} &            (3.3484)\phantom{*} &                                &                                &                                &                                &                               \smallskip \\
$d(b-a)$         &  \phantom{*}-0.0003\phantom{*} &                                &                               &                               &  \phantom{*}-0.0002\phantom{*} &   \phantom{*}0.0003\phantom{*} &                                &                                &                                &   \phantom{*}0.0003\phantom{*} \\
                 &                      (-0.3415) &                                &                               &                               &                      (-0.2449) &                       (0.3171) &                                &                                &                                &                       (0.2849)\smallskip \\
$(b-a)_{t=0}$    &  \phantom{*}-0.0109\phantom{*} &                                &                               &                               &  \phantom{*}-0.0134\phantom{*} &  \phantom{*}-0.0106\phantom{*} &                                &                                &                                &  \phantom{*}-0.0116\phantom{*} \\
                 &                      (-0.4622) &                                &                               &                               &                      (-0.5643) &                      (-0.4211) &                                &                                &                                &                      (-0.4563)\smallskip \\
$(b-a)_{t=\tau}$ &              \phantom{*}0.0142 &                                &                               &                               &   \phantom{*}0.0071\phantom{*} &   \phantom{*}0.0028\phantom{*} &                                &                                &                                &   \phantom{*}0.0015\phantom{*} \\
                 &                        (0.615) &                                &                               &                               &                       (0.3075) &                       (0.1153) &                                &                                &                                &                       (0.0621)\smallskip \\
$VIX_0$          &                                &   \phantom{*}0.0287\phantom{*} &                               &                               &   \phantom{*}0.0085\phantom{*} &                                &   \phantom{*}0.0281\phantom{*} &                                &                                &   \phantom{*}0.0181\phantom{*} \\
                 &                                &                       (1.3229) &                               &                               &                       (0.3751) &                                &                       (1.2957) &                                &                                &                       (0.7936)\smallskip \\
$VIX_{\tau}$     &                                &  \phantom{*}-0.0181\phantom{*} &                               &                               &  \phantom{*}-0.0209\phantom{*} &                                &  \phantom{*}-0.0166\phantom{*} &                                &                                &  \phantom{*}-0.0151\phantom{*} \\
                 &                                &                      (-0.8316) &                               &                               &                      (-0.9256) &                                &                      (-0.7602) &                                &                                &                      (-0.6573)\smallskip \\
$dVIX$           &                                &             \phantom{*}0.0141* &                               &                               &            \phantom{*}0.0175** &                                &   \phantom{*}0.0051\phantom{*} &                                &                                &   \phantom{*}0.0078\phantom{*} \\
                 &                                &                       (1.7033) &                               &                               &            (2.0604)\phantom{*} &                                &                       (0.5986) &                                &                                &                       (0.8937)\smallskip \\
$JUMP_0$         &                                &                                &  \phantom{*}0.2902\phantom{*} &                               &   \phantom{*}0.1931\phantom{*} &                                &                                &   \phantom{*}0.5554\phantom{*} &                                &   \phantom{*}0.6812\phantom{*} \\
                 &                                &                                &                      (0.2842) &                               &                       (0.1783) &                                &                                &                       (0.5484) &                                &                       (0.6135)\smallskip \\
$JUMP_{\tau}$    &                                &                                &  \phantom{*}0.0113\phantom{*} &                               &   \phantom{*}0.2814\phantom{*} &                                &                                &  \phantom{*}-0.3117\phantom{*} &                                &  \phantom{*}-0.4768\phantom{*} \\
                 &                                &                                &                      (0.0111) &                               &                       (0.2525) &                                &                                &                      (-0.3071) &                                &                      (-0.4122)\smallskip \\
$dJUMP$          &                                &                                &                               &  \phantom{*}0.0026\phantom{*} &  \phantom{*}-0.0077\phantom{*} &                                &                                &                                &  \phantom{*}-0.0014\phantom{*} &             \phantom{*}-0.0054 \\
                 &                                &                                &                               &                      (0.1722) &                      (-0.4778) &                                &                                &                                &                      (-0.0875) &                       (-0.329) \\
\medskip\\
year FE          &                             No &                             No &                            No &                            No &                             No &                            Yes &                            Yes &                            Yes &                            Yes &                            Yes \\
\medskip\\
Observations     &                          3,345 &                          3,345 &                         3,345 &                         3,345 &                          3,345 &                          3,345 &                          3,345 &                          3,345 &                          3,345 &                          3,345 \\
$R^2$            &                        -0.0008 &                         0.0027 &                        0.0048 &                       -0.0003 &                         0.0048 &                         0.0241 &                         0.0252 &                         0.0258 &                         0.0246 &                         0.0244 \\
\bottomrule
\end{tabular}


==> tex/perf_reg_obL10.tex <==
\begin{tabular}{lcccccccccc}
\toprule
{} &       \parboxc{c}{0.6cm}{(1)} &        \parboxc{c}{0.6cm}{(2)} &        \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &        \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &        \parboxc{c}{0.6cm}{(7)} &        \parboxc{c}{0.6cm}{(8)} &        \parboxc{c}{0.6cm}{(9)} &       \parboxc{c}{0.6cm}{(10)} \\
\midrule
one              &         \phantom{*}-0.0046*** &          \phantom{*}-0.0071*** &          \phantom{*}-0.0065*** &   \phantom{*}-0.0056*** &          \phantom{*}-0.0049*** &                                &                                &                                &                                &                                \\
                 &         (-3.049)\phantom{***} &          (-6.9094)\phantom{**} &          (-9.38)\phantom{****} &   (-9.562)\phantom{***} &          (-2.8345)\phantom{**} &                                &                                &                                &                                &                               \smallskip \\
$d(b-a)$         &           \phantom{*}-0.0017* &                                &                                &                         &           \phantom{*}-0.0019** &  \phantom{*}-0.0008\phantom{*} &                                &                                &                                &  \phantom{*}-0.0007\phantom{*} \\
                 &                     (-1.9311) &                                &                                &                         &           (-2.0944)\phantom{*} &                      (-0.8276) &                                &                                &                                &                      (-0.7394)\smallskip \\
$(b-a)_{t=0}$    &           \phantom{*}-0.0418* &                                &                                &                         &           \phantom{*}-0.0456** &  \phantom{*}-0.0184\phantom{*} &                                &                                &                                &  \phantom{*}-0.0194\phantom{*} \\
                 &                     (-1.9397) &                                &                                &                         &           (-2.0521)\phantom{*} &                      (-0.7582) &                                &                                &                                &                      (-0.7758)\smallskip \\
$(b-a)_{t=\tau}$ &  \phantom{*}0.0215\phantom{*} &                                &                                &                         &   \phantom{*}0.0183\phantom{*} &              \phantom{*}0.0294 &                                &                                &                                &   \phantom{*}0.0314\phantom{*} \\
                 &                      (1.0045) &                                &                                &                         &                       (0.8497) &                        (1.258) &                                &                                &                                &                       (1.3264)\smallskip \\
$VIX_0$          &                               &  \phantom{*}-0.0042\phantom{*} &                                &                         &             \phantom{*}-0.0008 &                                &  \phantom{*}-0.0116\phantom{*} &                                &                                &   \phantom{*}0.0168\phantom{*} \\
                 &                               &                      (-0.3971) &                                &                         &                       (-0.059) &                                &                      (-1.0474) &                                &                                &                       (1.1649)\smallskip \\
$VIX_{\tau}$     &                               &   \phantom{*}0.0066\phantom{*} &                                &                         &   \phantom{*}0.0121\phantom{*} &                                &  \phantom{*}-0.0059\phantom{*} &                                &                                &  \phantom{*}-0.0004\phantom{*} \\
                 &                               &                       (0.6168) &                                &                         &                       (1.0408) &                                &                      (-0.5218) &                                &                                &                      (-0.0299)\smallskip \\
$dVIX$           &                               &   \phantom{*}0.0021\phantom{*} &                                &                         &   \phantom{*}0.0016\phantom{*} &                                &             \phantom{*}-0.0031 &                                &                                &  \phantom{*}-0.0044\phantom{*} \\
                 &                               &                       (0.5403) &                                &                         &                       (0.3903) &                                &                       (-0.781) &                                &                                &                      (-1.0858)\smallskip \\
$JUMP_0$         &                               &                                &  \phantom{*}-0.1635\phantom{*} &                         &  \phantom{*}-0.0569\phantom{*} &                                &                                &  \phantom{*}-0.28\phantom{***} &                                &  \phantom{*}-0.3087\phantom{*} \\
                 &                               &                                &                      (-0.8207) &                         &                      (-0.2556) &                                &                                &                      (-1.3909) &                                &                      (-1.3688)\smallskip \\
$JUMP_{\tau}$    &                               &                                &   \phantom{*}0.1781\phantom{*} &                         &  \phantom{*}-0.0479\phantom{*} &                                &                                &             \phantom{*}-0.1552 &                                &  \phantom{*}-0.3024\phantom{*} \\
                 &                               &                                &                       (0.8911) &                         &                      (-0.1877) &                                &                                &                       (-0.755) &                                &                      (-1.0616)\smallskip \\
$dJUMP$          &                               &                                &                                &     \phantom{*}-0.0046* &            \phantom{*}-0.0046* &                                &                                &                                &  \phantom{*}-0.0023\phantom{*} &  \phantom{*}-0.0015\phantom{*} \\
                 &                               &                                &                                &               (-1.8151) &                      (-1.6828) &                                &                                &                                &                      (-0.8916) &                      (-0.5415) \\
\medskip\\
year FE          &                            No &                             No &                             No &                      No &                             No &                            Yes &                            Yes &                            Yes &                            Yes &                            Yes \\
\medskip\\
Observations     &                         3,366 &                          3,366 &                          3,366 &                   3,366 &                          3,366 &                          3,366 &                          3,366 &                          3,366 &                          3,366 &                          3,366 \\
$R^2$            &                        0.0008 &                        -0.0006 &                        -0.0004 &                  0.0007 &                         0.0007 &                         0.0295 &                         0.0306 &                         0.0329 &                         0.0298 &                         0.0321 \\
\bottomrule
\end{tabular}


==> tex/perf_reg_obL2.tex <==
\begin{tabular}{lcccccc}
\toprule
{} &        \parboxc{c}{0.6cm}{(1)} & \parboxc{c}{0.6cm}{(2)} & \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} & \parboxc{c}{0.6cm}{(5)} & \parboxc{c}{0.6cm}{(6)} \\
\midrule
b-a          &                                &                         &     \phantom{*}-0.0104* &                         &                         &     \phantom{*}-0.0122* \\
             &                                &                         &               (-1.8238) &                         &                         &               (-1.9537)\smallskip \\
b-a(2)       &                                &                         &                         &    \phantom{*}-0.0129** &                         &   \phantom{*}-0.0195*** \\
             &                                &                         &                         &    (-2.28)\phantom{***} &                         &   (-3.0693)\phantom{**}\smallskip \\
dVatm        &                                &   \phantom{**}0.0806*** &                         &                         &                         &   \phantom{**}0.0942*** \\
             &                                &   (11.6369)\phantom{**} &                         &                         &                         &   (13.0697)\phantom{**}\smallskip \\
dba          &  \phantom{*}-0.012*\phantom{*} &                         &                         &                         &                         &   \phantom{*}-0.0186*** \\
             &                      (-1.9202) &                         &                         &                         &                         &   (-2.8715)\phantom{**}\smallskip \\
dMAE-1 days  &                                &                         &                         &                         &       \phantom{*}0.0084 &      \phantom{*}0.0285* \\
             &                                &                         &                         &                         &                 (0.528) &                (1.8194) \\
\medskip\\
year FE      &                            Yes &                     Yes &                     Yes &                     Yes &                     Yes &                     Yes \\
\medskip\\
Observations &                          4,028 &                   4,028 &                   4,028 &                   4,028 &                   4,028 &                   4,028 \\
$R^2$        &                          0.015 &                  0.0463 &                  0.0149 &                  0.0153 &                  0.0141 &                  0.0553 \\
\bottomrule
\end{tabular}


==> tex/perf_reghbL1.tex <==
\begin{tabular}{lcccccccccc}
\toprule
{} &       \parboxc{c}{0.6cm}{(1)} &        \parboxc{c}{0.6cm}{(2)} &        \parboxc{c}{0.6cm}{(3)} & \parboxc{c}{0.6cm}{(4)} &        \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &        \parboxc{c}{0.6cm}{(7)} &        \parboxc{c}{0.6cm}{(8)} &       \parboxc{c}{0.6cm}{(9)} &       \parboxc{c}{0.6cm}{(10)} \\
\midrule
$(b-a)_{t=0}$    &           \phantom{*}0.0242** &                                &                                &                         &             \phantom{*}0.0192* &  \phantom{*}-0.0061\phantom{*} &                                &                                &                               &  \phantom{*}-0.0091\phantom{*} \\
                 &           (2.2711)\phantom{*} &                                &                                &                         &                       (1.7821) &                      (-0.5452) &                                &                                &                               &                      (-0.8068)\smallskip \\
$(b-a)_{t=\tau}$ &          \phantom{*}0.0381*** &                                &                                &                         &           \phantom{*}0.0353*** &             \phantom{*}0.0183* &                                &                                &                               &   \phantom{*}0.0161\phantom{*} \\
                 &          (3.6485)\phantom{**} &                                &                                &                         &           (3.3619)\phantom{**} &                       (1.7274) &                                &                                &                               &                       (1.5188)\smallskip \\
dJump            &                               &                                &                                &     \phantom{*}0.0146** &   \phantom{*}0.0046\phantom{*} &                                &                                &                                &  \phantom{*}0.005\phantom{**} &   \phantom{*}0.0004\phantom{*} \\
                 &                               &                                &                                &     (2.0897)\phantom{*} &                       (0.6339) &                                &                                &                                &                      (0.7369) &                       (0.0578)\smallskip \\
dVix             &                               &  \phantom{*}-0.0035\phantom{*} &                                &                         &  \phantom{*}-0.0046\phantom{*} &                                &   \phantom{*}0.0029\phantom{*} &                                &                               &   \phantom{*}0.002\phantom{**} \\
                 &                               &                      (-0.9264) &                                &                         &                      (-1.1927) &                                &                       (0.7708) &                                &                               &                       (0.5218)\smallskip \\
d(b-a)           &  \phantom{*}0.0003\phantom{*} &                                &                                &                         &   \phantom{*}0.0002\phantom{*} &             \phantom{*}-0.0003 &                                &                                &                               &  \phantom{*}-0.0003\phantom{*} \\
                 &                      (0.7237) &                                &                                &                         &                       (0.5299) &                       (-0.628) &                                &                                &                               &                      (-0.8483)\smallskip \\
jump             &                               &                                &  \phantom{*}-0.211\phantom{**} &                         &   \phantom{*}0.2052\phantom{*} &                                &                                &  \phantom{*}-0.2314\phantom{*} &                               &   \phantom{*}0.1816\phantom{*} \\
                 &                               &                                &                      (-0.4516) &                         &                       (0.4176) &                                &                                &                      (-0.5167) &                               &                       (0.3702)\smallskip \\
jump 1           &                               &                                &              \phantom{*}0.3117 &                         &  \phantom{*}-0.313\phantom{**} &                                &                                &   \phantom{*}0.2449\phantom{*} &                               &  \phantom{*}-0.2656\phantom{*} \\
                 &                               &                                &                        (0.667) &                         &                      (-0.6188) &                                &                                &                       (0.5458) &                               &                      (-0.5198)\smallskip \\
one              &        \phantom{**}-0.0092*** &         \phantom{**}-0.0065*** &         \phantom{**}-0.0055*** &  \phantom{**}-0.0051*** &           \phantom{**}-0.01*** &                                &                                &                                &                               &                                \\
                 &        (-15.1502)\phantom{**} &         (-15.3753)\phantom{**} &         (-18.9992)\phantom{**} &  (-21.9822)\phantom{**} &                     (-14.8802) &                                &                                &                                &                               &                               \smallskip \\
vix              &                               &             \phantom{*}-0.0059 &                                &                         &  \phantom{*}-0.0013\phantom{*} &                                &  \phantom{*}-0.0066\phantom{*} &                                &                               &  \phantom{*}-0.0036\phantom{*} \\
                 &                               &             (-0.6)\phantom{**} &                                &                         &                      (-0.1217) &                                &                      (-0.6948) &                                &                               &                      (-0.3571)\smallskip \\
vix 1            &                               &   \phantom{*}0.0155\phantom{*} &                                &                         &   \phantom{*}0.0129\phantom{*} &                                &   \phantom{*}0.0117\phantom{*} &                                &                               &   \phantom{*}0.0132\phantom{*} \\
                 &                               &                       (1.5592) &                                &                         &                       (1.2604) &                                &                       (1.2138) &                                &                               &                       (1.2956) \\
\medskip\\
year FE          &                            No &                             No &                             No &                      No &                             No &                            Yes &                            Yes &                            Yes &                           Yes &                            Yes \\
\medskip\\
Observations     &                         3,345 &                          3,345 &                          3,345 &                   3,345 &                          3,345 &                          3,345 &                          3,345 &                          3,345 &                         3,345 &                          3,345 \\
$R^2$            &                        0.0166 &                         0.0067 &                         0.0024 &                   0.001 &                         0.0191 &                         0.0898 &                         0.0902 &                         0.0893 &                        0.0896 &                         0.0896 \\
\bottomrule
\end{tabular}


==> tex/slope_reghbL1.tex <==
\begin{tabular}{lcccccccc}
\toprule
{} &       \parboxc{c}{0.6cm}{(1)} &        \parboxc{c}{0.6cm}{(2)} &       \parboxc{c}{0.6cm}{(3)} &        \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &        \parboxc{c}{0.6cm}{(7)} &        \parboxc{c}{0.6cm}{(8)} \\
\midrule
one                     &          \phantom{*}-0.0004** &            \phantom{*}-0.0004* &         \phantom{*}-0.0007*** &           \phantom{*}-0.0007** &                               &                                &                                &                                \\
                        &          (-2.174)\phantom{**} &                      (-1.7404) &         (-2.6648)\phantom{**} &           (-2.4386)\phantom{*} &                               &                                &                                &                               \smallskip \\
$d \beta_K^{Put}$       &           \phantom{*}0.0014** &                                &                               &   \phantom{*}0.0007\phantom{*} &            \phantom{*}0.0011* &                                &                                &   \phantom{*}0.0005\phantom{*} \\
                        &           (2.348)\phantom{**} &                                &                               &                       (0.4991) &                      (1.6522) &                                &                                &                       (0.3504)\smallskip \\
$d \beta_K^{Call}$      &         \phantom{*}-0.0023*** &                                &                               &          \phantom{*}-0.0013*** &         \phantom{*}-0.0018*** &                                &                                &          \phantom{*}-0.0013*** \\
                        &         (-3.6041)\phantom{**} &                                &                               &          (-2.7379)\phantom{**} &         (-2.6231)\phantom{**} &                                &                                &          (-2.6452)\phantom{**}\smallskip \\
$d \beta_0^{Put}$       &  \phantom{*}0.0029\phantom{*} &                                &                               &   \phantom{*}0.0025\phantom{*} &  \phantom{*}0.0045\phantom{*} &                                &                                &   \phantom{*}0.0039\phantom{*} \\
                        &                      (1.0365) &                                &                               &                       (0.8581) &                      (1.6378) &                                &                                &                       (1.3431)\smallskip \\
$d \beta_0^{Call}$      &            \phantom{*}0.0044* &                                &                               &   \phantom{*}0.0037\phantom{*} &             \phantom{*}0.0034 &                                &                                &   \phantom{*}0.0032\phantom{*} \\
                        &                      (1.7327) &                                &                               &                       (1.4523) &             (1.37)\phantom{*} &                                &                                &                       (1.2764)\smallskip \\
$d \beta_T^{Call}$      &           \phantom{*}0.6674** &                                &                               &   \phantom{*}0.961\phantom{**} &          \phantom{*}0.7093*** &                                &                                &   \phantom{*}0.3694\phantom{*} \\
                        &           (2.5395)\phantom{*} &                                &                               &                       (1.1577) &          (2.6149)\phantom{**} &                                &                                &                       (0.4468)\smallskip \\
$d \beta_T^{Put}$       &          \phantom{*}-0.5969** &                                &                               &  \phantom{*}-0.3157\phantom{*} &          \phantom{*}-0.7125** &                                &                                &  \phantom{*}-1.2591\phantom{*} \\
                        &          (-1.9735)\phantom{*} &                                &                               &                      (-0.3146) &          (-2.3441)\phantom{*} &                                &                                &                      (-1.2569)\smallskip \\
$|\beta_K^{Put,0}|$     &                               &             \phantom{*}0.0015* &                               &   \phantom{*}0.0008\phantom{*} &                               &   \phantom{*}0.0013\phantom{*} &                                &   \phantom{*}0.0011\phantom{*} \\
                        &                               &             (1.753)\phantom{*} &                               &                       (0.4485) &                               &                       (1.4116) &                                &                       (0.6357)\smallskip \\
$|\beta_K^{Call,0}|$    &                               &          \phantom{*}-0.0035*** &                               &            \phantom{*}-0.0017* &                               &          \phantom{*}-0.0027*** &                                &  \phantom{*}-0.0015\phantom{*} \\
                        &                               &          (-3.6018)\phantom{**} &                               &                      (-1.7131) &                               &          (-2.6218)\phantom{**} &                                &                      (-1.5895)\smallskip \\
$|\beta_0^{Put,0}|$     &                               &  \phantom{*}-0.0035\phantom{*} &                               &  \phantom{*}-0.0037\phantom{*} &                               &  \phantom{*}-0.0013\phantom{*} &                                &   \phantom{*}0.0004\phantom{*} \\
                        &                               &                      (-1.6253) &                               &                      (-1.0892) &                               &                      (-0.4742) &                                &                       (0.1091)\smallskip \\
$|\beta_0^{Call,0}|$    &                               &             \phantom{*}0.0041* &                               &  \phantom{*}-0.0017\phantom{*} &                               &   \phantom{*}0.0025\phantom{*} &                                &   \phantom{*}0.0003\phantom{*} \\
                        &                               &                       (1.8527) &                               &                      (-0.4632) &                               &                       (0.8225) &                                &                       (0.0794)\smallskip \\
$|\beta_T^{Put,0}|$     &                               &  \phantom{*}-0.1163\phantom{*} &                               &  \phantom{*}-0.0622\phantom{*} &                               &  \phantom{*}-0.535\phantom{**} &                                &   \phantom{*}0.1308\phantom{*} \\
                        &                               &                      (-0.2892) &                               &                      (-0.0656) &                               &                      (-1.2062) &                                &                       (0.1393)\smallskip \\
$|\beta_T^{Call,0}|$    &                               &              \phantom{*}0.5581 &                               &   \phantom{*}0.1082\phantom{*} &                               &   \phantom{*}0.5769\phantom{*} &                                &   \phantom{*}0.3182\phantom{*} \\
                        &                               &                        (1.358) &                               &                       (0.1357) &                               &                       (1.2666) &                                &                       (0.4024)\smallskip \\
$|\beta_K^{Put,\tau}|$  &                               &                                &  \phantom{*}0.0007\phantom{*} &   \phantom{*}0.0003\phantom{*} &                               &                                &   \phantom{*}0.0007\phantom{*} &   \phantom{*}0.0001\phantom{*} \\
                        &                               &                                &                      (0.9545) &                       (0.2926) &                               &                                &                       (0.8447) &                       (0.0824)\smallskip \\
$|\beta_K^{Call,\tau}|$ &                               &                                &  \phantom{*}0.001\phantom{**} &             \phantom{*}-0.0004 &                               &                                &   \phantom{*}0.001\phantom{**} &  \phantom{*}-0.0003\phantom{*} \\
                        &                               &                                &                      (1.2063) &                       (-0.385) &                               &                                &                       (1.1618) &                      (-0.2622)\smallskip \\
$|\beta_0^{Put,\tau}|$  &                               &                                &         \phantom{*}-0.0125*** &  \phantom{*}-0.0051\phantom{*} &                               &                                &             \phantom{*}-0.01** &  \phantom{*}-0.0071\phantom{*} \\
                        &                               &                                &         (-3.1003)\phantom{**} &                      (-1.0014) &                               &                                &                       (-2.156) &                      (-1.2663)\smallskip \\
$|\beta_0^{Call,\tau}|$ &                               &                                &          \phantom{*}0.0144*** &            \phantom{*}0.0121** &                               &                                &            \phantom{*}0.0108** &   \phantom{*}0.0069\phantom{*} \\
                        &                               &                                &          (3.4568)\phantom{**} &            (2.2379)\phantom{*} &                               &                                &            (2.0624)\phantom{*} &                       (1.1257)\smallskip \\
$|\beta_T^{Put,\tau}|$  &                               &                                &          \phantom{*}-1.5116** &  \phantom{*}-0.865\phantom{**} &                               &                                &  \phantom{*}-1.2358\phantom{*} &  \phantom{*}-2.0103\phantom{*} \\
                        &                               &                                &          (-2.1465)\phantom{*} &                      (-0.6912) &                               &                                &                      (-1.6211) &                      (-1.5269)\smallskip \\
$|\beta_T^{Call,\tau}|$ &                               &                                &           \phantom{*}1.6051** &            \phantom{*}2.3131** &                               &                                &   \phantom{*}0.822\phantom{**} &   \phantom{*}0.766\phantom{**} \\
                        &                               &                                &           (2.2686)\phantom{*} &            (2.0414)\phantom{*} &                               &                                &                       (0.9946) &                       (0.6225) \\
\medskip\\
year FE                 &                            No &                             No &                            No &                             No &                           Yes &                            Yes &                            Yes &                            Yes \\
\medskip\\
Observations            &                         3,909 &                          3,909 &                         3,909 &                          3,909 &                         3,909 &                          3,909 &                          3,909 &                          3,909 \\
$R^2$                   &                        0.0103 &                         0.0099 &                         0.009 &                         0.0114 &                        0.0427 &                         0.0414 &                         0.0411 &                         0.0421 \\
\bottomrule
\end{tabular}


==> tex/slope_reghbL10.tex <==
\begin{tabular}{lcccccccc}
\toprule
{} &       \parboxc{c}{0.6cm}{(1)} &        \parboxc{c}{0.6cm}{(2)} &        \parboxc{c}{0.6cm}{(3)} &        \parboxc{c}{0.6cm}{(4)} &        \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &        \parboxc{c}{0.6cm}{(7)} &        \parboxc{c}{0.6cm}{(8)} \\
\midrule
one                     &  \phantom{*}0.0013\phantom{*} &   \phantom{*}0.0001\phantom{*} &  \phantom{*}-0.0003\phantom{*} &  \phantom{*}-0.0006\phantom{*} &                                &                                &                                &                                \\
                        &                      (1.6298) &                       (0.1335) &                      (-0.2822) &                      (-0.5192) &                                &                                &                                &                               \smallskip \\
$d \beta_K^{Put}$       &           \phantom{*}-0.0049* &                                &                                &  \phantom{*}-0.0029\phantom{*} &  \phantom{*}-0.002\phantom{**} &                                &                                &  \phantom{*}-0.0012\phantom{*} \\
                        &                     (-1.8899) &                                &                                &                      (-0.4264) &                      (-0.7023) &                                &                                &                      (-0.1729)\smallskip \\
$d \beta_K^{Call}$      &  \phantom{*}0.0015\phantom{*} &                                &                                &   \phantom{*}0.0012\phantom{*} &   \phantom{*}0.0028\phantom{*} &                                &                                &   \phantom{*}0.0017\phantom{*} \\
                        &                      (0.5335) &                                &                                &                       (0.5924) &                       (0.9566) &                                &                                &                       (0.7888)\smallskip \\
$d \beta_0^{Put}$       &          \phantom{*}-0.0211** &                                &                                &           \phantom{*}-0.0231** &           \phantom{*}-0.0217** &                                &                                &          \phantom{*}-0.0255*** \\
                        &          (-2.3773)\phantom{*} &                                &                                &           (-2.5015)\phantom{*} &           (-2.4706)\phantom{*} &                                &                                &          (-2.7879)\phantom{**}\smallskip \\
$d \beta_0^{Call}$      &  \phantom{*}0.0001\phantom{*} &                                &                                &   \phantom{*}0.0036\phantom{*} &  \phantom{*}-0.0011\phantom{*} &                                &                                &   \phantom{*}0.0006\phantom{*} \\
                        &                      (0.0079) &                                &                                &                       (0.3983) &                      (-0.1211) &                                &                                &                       (0.0659)\smallskip \\
$d \beta_T^{Call}$      &  \phantom{*}0.5661\phantom{*} &                                &                                &  \phantom{*}-2.4689\phantom{*} &             \phantom{*}-0.3015 &                                &                                &  \phantom{*}-3.1525\phantom{*} \\
                        &                      (0.3995) &                                &                                &                      (-0.8432) &                       (-0.207) &                                &                                &                      (-1.0767)\smallskip \\
$d \beta_T^{Put}$       &  \phantom{*}0.6874\phantom{*} &                                &                                &             \phantom{*}5.8628* &   \phantom{*}0.6585\phantom{*} &                                &                                &   \phantom{*}4.9203\phantom{*} \\
                        &                      (0.4492) &                                &                                &                       (1.9077) &                       (0.4293) &                                &                                &                       (1.6079)\smallskip \\
$|\beta_K^{Put,0}|$     &                               &  \phantom{*}-0.0042\phantom{*} &                                &   \phantom{*}0.0036\phantom{*} &                                &   \phantom{*}0.0018\phantom{*} &                                &   \phantom{*}0.0043\phantom{*} \\
                        &                               &                      (-1.0679) &                                &                       (0.4373) &                                &                       (0.4385) &                                &                       (0.5249)\smallskip \\
$|\beta_K^{Call,0}|$    &                               &  \phantom{*}-0.0022\phantom{*} &                                &              \phantom{*}0.0022 &                                &   \phantom{*}0.0026\phantom{*} &                                &   \phantom{*}0.0031\phantom{*} \\
                        &                               &                      (-0.5133) &                                &                        (0.598) &                                &                       (0.5827) &                                &                       (0.8675)\smallskip \\
$|\beta_0^{Put,0}|$     &                               &           \phantom{*}-0.0221** &                                &             \phantom{*}-0.0009 &                                &   \phantom{*}0.0037\phantom{*} &                                &              \phantom{*}0.0133 \\
                        &                               &           (-2.324)\phantom{**} &                                &                       (-0.074) &                                &                       (0.3208) &                                &                        (1.058)\smallskip \\
$|\beta_0^{Call,0}|$    &                               &           \phantom{*}0.0256*** &                                &  \phantom{*}-0.0029\phantom{*} &                                &  \phantom{*}-0.005\phantom{**} &                                &  \phantom{*}-0.0094\phantom{*} \\
                        &                               &           (2.6218)\phantom{**} &                                &                      (-0.2194) &                                &                      (-0.3887) &                                &                      (-0.6643)\smallskip \\
$|\beta_T^{Put,0}|$     &                               &            \phantom{*}4.7186** &                                &  \phantom{*}-1.5209\phantom{*} &                                &   \phantom{*}0.2461\phantom{*} &                                &             \phantom{*}-3.4932 \\
                        &                               &            (2.3454)\phantom{*} &                                &                      (-0.5003) &                                &                       (0.1143) &                                &                       (-1.149)\smallskip \\
$|\beta_T^{Call,0}|$    &                               &           \phantom{*}-4.6811** &                                &  \phantom{*}-0.4233\phantom{*} &                                &  \phantom{*}-1.0877\phantom{*} &                                &              \phantom{*}1.3494 \\
                        &                               &           (-2.4476)\phantom{*} &                                &                      (-0.1487) &                                &                      (-0.5311) &                                &                        (0.476)\smallskip \\
$|\beta_K^{Put,\tau}|$  &                               &                                &            \phantom{*}0.0077** &   \phantom{*}0.0076\phantom{*} &                                &                                &   \phantom{*}0.0048\phantom{*} &   \phantom{*}0.0059\phantom{*} \\
                        &                               &                                &            (2.3777)\phantom{*} &                       (1.4937) &                                &                                &                       (1.3722) &                       (1.1691)\smallskip \\
$|\beta_K^{Call,\tau}|$ &                               &                                &  \phantom{*}-0.0006\phantom{*} &   \phantom{*}0.001\phantom{**} &                                &                                &  \phantom{*}-0.0014\phantom{*} &   \phantom{*}0.0015\phantom{*} \\
                        &                               &                                &                      (-0.1655) &                       (0.2596) &                                &                                &                      (-0.3496) &                       (0.4009)\smallskip \\
$|\beta_0^{Put,\tau}|$  &                               &                                &             \phantom{*}0.0349* &   \phantom{*}0.0278\phantom{*} &                                &                                &             \phantom{*}0.0445* &              \phantom{*}0.0364 \\
                        &                               &                                &                       (1.7262) &                       (1.2522) &                                &                                &                       (1.9213) &                        (1.484)\smallskip \\
$|\beta_0^{Call,\tau}|$ &                               &                                &  \phantom{*}-0.0289\phantom{*} &  \phantom{*}-0.0174\phantom{*} &                                &                                &  \phantom{*}-0.049*\phantom{*} &            \phantom{*}-0.0482* \\
                        &                               &                                &                      (-1.3788) &                      (-0.7459) &                                &                                &                      (-1.9015) &            (-1.785)\phantom{*}\smallskip \\
$|\beta_T^{Put,\tau}|$  &                               &                                &                     13.2479*** &                     15.7816*** &                                &                                &                     13.0691*** &                     14.2939*** \\
                        &                               &                                &           (3.552)\phantom{***} &           (3.3832)\phantom{**} &                                &                                &           (3.1639)\phantom{**} &           (2.8089)\phantom{**}\smallskip \\
$|\beta_T^{Call,\tau}|$ &                               &                                &          \phantom{*}-9.8872*** &                     -10.6169** &                                &                                &                    -11.9752*** &                    -15.5827*** \\
                        &                               &                                &          (-2.6491)\phantom{**} &           (-2.2746)\phantom{*} &                                &                                &          (-2.7499)\phantom{**} &          (-2.9631)\phantom{**} \\
\medskip\\
year FE                 &                            No &                             No &                             No &                             No &                            Yes &                            Yes &                            Yes &                            Yes \\
\medskip\\
Observations            &                         3,345 &                          3,345 &                          3,345 &                          3,345 &                          3,345 &                          3,345 &                          3,345 &                          3,345 \\
$R^2$                   &                        0.0089 &                         0.0055 &                         0.0138 &                         0.0147 &                         0.0409 &                         0.0374 &                         0.0412 &                         0.0439 \\
\bottomrule
\end{tabular}


==> tex/slope_regobL1.tex <==
\begin{tabular}{lcccccccccccccc}
\toprule
{} &       \parboxc{c}{0.6cm}{(1)} &        \parboxc{c}{0.6cm}{(2)} &       \parboxc{c}{0.6cm}{(3)} &        \parboxc{c}{0.6cm}{(4)} &       \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &        \parboxc{c}{0.6cm}{(7)} &        \parboxc{c}{0.6cm}{(8)} &       \parboxc{c}{0.6cm}{(9)} &       \parboxc{c}{0.6cm}{(10)} &      \parboxc{c}{0.6cm}{(11)} &      \parboxc{c}{0.6cm}{(12)} &       \parboxc{c}{0.6cm}{(13)} &       \parboxc{c}{0.6cm}{(14)} \\
\midrule
one                     &          \phantom{*}-0.0004** &            \phantom{*}-0.0004* &         \phantom{*}-0.0007*** &           \phantom{*}-0.0007** &                               &                                &                                &                                &          \phantom{*}-0.0004** &            \phantom{*}-0.0004* &         \phantom{*}-0.0007*** &                               &                                &                                \\
                        &          (-2.262)\phantom{**} &            (-1.792)\phantom{*} &         (-2.7825)\phantom{**} &           (-2.5178)\phantom{*} &                               &                                &                                &                                &          (-2.262)\phantom{**} &            (-1.792)\phantom{*} &         (-2.7825)\phantom{**} &                               &                                &                               \smallskip \\
$d \beta_K^{Put}$       &           \phantom{*}0.0014** &                                &                               &   \phantom{*}0.0007\phantom{*} &  \phantom{*}0.001\phantom{**} &                                &                                &   \phantom{*}0.0005\phantom{*} &           \phantom{*}0.0014** &                                &                               &  \phantom{*}0.001\phantom{**} &                                &                                \\
                        &           (2.277)\phantom{**} &                                &                               &                       (0.5075) &                      (1.6102) &                                &                                &                       (0.3794) &           (2.277)\phantom{**} &                                &                               &                      (1.6102) &                                &                               \smallskip \\
$d \beta_K^{Call}$      &         \phantom{*}-0.0023*** &                                &                               &          \phantom{*}-0.0013*** &          \phantom{*}-0.0017** &                                &                                &           \phantom{*}-0.0012** &         \phantom{*}-0.0023*** &                                &                               &          \phantom{*}-0.0017** &                                &                                \\
                        &         (-3.5125)\phantom{**} &                                &                               &          (-2.6809)\phantom{**} &          (-2.5374)\phantom{*} &                                &                                &           (-2.5543)\phantom{*} &         (-3.5125)\phantom{**} &                                &                               &          (-2.5374)\phantom{*} &                                &                               \smallskip \\
$d \beta_0^{Put}$       &  \phantom{*}0.0028\phantom{*} &                                &                               &   \phantom{*}0.0025\phantom{*} &             \phantom{*}0.0044 &                                &                                &   \phantom{*}0.0039\phantom{*} &  \phantom{*}0.0028\phantom{*} &                                &                               &             \phantom{*}0.0044 &                                &                                \\
                        &                      (1.0099) &                                &                               &                       (0.8786) &                       (1.604) &                                &                                &                       (1.3518) &                      (1.0099) &                                &                               &                       (1.604) &                                &                               \smallskip \\
$d \beta_0^{Call}$      &            \phantom{*}0.0044* &                                &                               &   \phantom{*}0.0038\phantom{*} &  \phantom{*}0.0034\phantom{*} &                                &                                &   \phantom{*}0.0033\phantom{*} &            \phantom{*}0.0044* &                                &                               &  \phantom{*}0.0034\phantom{*} &                                &                                \\
                        &                      (1.7354) &                                &                               &                       (1.4757) &                      (1.3722) &                                &                                &                       (1.2941) &                      (1.7354) &                                &                               &                      (1.3722) &                                &                               \smallskip \\
$d \beta_T^{Call}$      &           \phantom{*}0.6194** &                                &                               &   \phantom{*}0.9393\phantom{*} &           \phantom{*}0.6571** &                                &                                &   \phantom{*}0.3552\phantom{*} &           \phantom{*}0.6194** &                                &                               &           \phantom{*}0.6571** &                                &                                \\
                        &           (2.3621)\phantom{*} &                                &                               &                       (1.1309) &           (2.4298)\phantom{*} &                                &                                &                       (0.4294) &           (2.3621)\phantom{*} &                                &                               &           (2.4298)\phantom{*} &                                &                               \smallskip \\
$d \beta_T^{Put}$       &           \phantom{*}-0.5633* &                                &                               &  \phantom{*}-0.3482\phantom{*} &          \phantom{*}-0.6783** &                                &                                &  \phantom{*}-1.3061\phantom{*} &           \phantom{*}-0.5633* &                                &                               &          \phantom{*}-0.6783** &                                &                                \\
                        &                     (-1.8645) &                                &                               &                      (-0.3468) &          (-2.2344)\phantom{*} &                                &                                &                      (-1.3034) &                     (-1.8645) &                                &                               &          (-2.2344)\phantom{*} &                                &                               \smallskip \\
$|\beta_K^{Put,0}|$     &                               &             \phantom{*}0.0015* &                               &   \phantom{*}0.0007\phantom{*} &                               &   \phantom{*}0.0013\phantom{*} &                                &   \phantom{*}0.001\phantom{**} &                               &             \phantom{*}0.0015* &                               &                               &   \phantom{*}0.0013\phantom{*} &                                \\
                        &                               &                       (1.6909) &                               &                       (0.3765) &                               &                       (1.3943) &                                &                       (0.5751) &                               &                       (1.6909) &                               &                               &                       (1.3943) &                               \smallskip \\
$|\beta_K^{Call,0}|$    &                               &          \phantom{*}-0.0034*** &                               &            \phantom{*}-0.0018* &                               &           \phantom{*}-0.0026** &                                &            \phantom{*}-0.0016* &                               &          \phantom{*}-0.0034*** &                               &                               &           \phantom{*}-0.0026** &                                \\
                        &                               &          (-3.508)\phantom{***} &                               &                      (-1.8164) &                               &           (-2.513)\phantom{**} &                                &                      (-1.6657) &                               &          (-3.508)\phantom{***} &                               &                               &           (-2.513)\phantom{**} &                               \smallskip \\
$|\beta_0^{Put,0}|$     &                               &  \phantom{*}-0.0032\phantom{*} &                               &  \phantom{*}-0.0038\phantom{*} &                               &  \phantom{*}-0.0009\phantom{*} &                                &   \phantom{*}0.0005\phantom{*} &                               &  \phantom{*}-0.0032\phantom{*} &                               &                               &  \phantom{*}-0.0009\phantom{*} &                                \\
                        &                               &                      (-1.4892) &                               &                      (-1.1211) &                               &                      (-0.3377) &                                &                       (0.1451) &                               &                      (-1.4892) &                               &                               &                      (-0.3377) &                               \smallskip \\
$|\beta_0^{Call,0}|$    &                               &             \phantom{*}0.0038* &                               &  \phantom{*}-0.0013\phantom{*} &                               &    \phantom{*}0.002\phantom{*} &                                &   \phantom{*}0.0004\phantom{*} &                               &             \phantom{*}0.0038* &                               &                               &    \phantom{*}0.002\phantom{*} &                                \\
                        &                               &                       (1.7016) &                               &                      (-0.3539) &                               &                        (0.654) &                                &                       (0.1148) &                               &                       (1.7016) &                               &                               &                        (0.654) &                               \smallskip \\
$|\beta_T^{Put,0}|$     &                               &  \phantom{*}-0.1409\phantom{*} &                               &  \phantom{*}-0.0099\phantom{*} &                               &  \phantom{*}-0.5684\phantom{*} &                                &   \phantom{*}0.1711\phantom{*} &                               &  \phantom{*}-0.1409\phantom{*} &                               &                               &  \phantom{*}-0.5684\phantom{*} &                                \\
                        &                               &                      (-0.3504) &                               &                      (-0.0104) &                               &                      (-1.2819) &                                &                       (0.1822) &                               &                      (-0.3504) &                               &                               &                      (-1.2819) &                               \smallskip \\
$|\beta_T^{Call,0}|$    &                               &   \phantom{*}0.5677\phantom{*} &                               &   \phantom{*}0.0999\phantom{*} &                               &   \phantom{*}0.6053\phantom{*} &                                &   \phantom{*}0.3279\phantom{*} &                               &   \phantom{*}0.5677\phantom{*} &                               &                               &   \phantom{*}0.6053\phantom{*} &                                \\
                        &                               &                       (1.3813) &                               &                       (0.1252) &                               &                       (1.3293) &                                &                       (0.4143) &                               &                       (1.3813) &                               &                               &                       (1.3293) &                               \smallskip \\
$|\beta_K^{Put,\tau}|$  &                               &                                &  \phantom{*}0.0007\phantom{*} &   \phantom{*}0.0003\phantom{*} &                               &                                &   \phantom{*}0.0006\phantom{*} &    \phantom{*}0.0\phantom{***} &                               &                                &  \phantom{*}0.0007\phantom{*} &                               &                                &   \phantom{*}0.0006\phantom{*} \\
                        &                               &                                &                      (0.9428) &                       (0.2205) &                               &                                &                       (0.7304) &                        (0.004) &                               &                                &                      (0.9428) &                               &                                &                       (0.7304)\smallskip \\
$|\beta_K^{Call,\tau}|$ &                               &                                &  \phantom{*}0.0009\phantom{*} &  \phantom{*}-0.0005\phantom{*} &                               &                                &   \phantom{*}0.0009\phantom{*} &  \phantom{*}-0.0004\phantom{*} &                               &                                &  \phantom{*}0.0009\phantom{*} &                               &                                &   \phantom{*}0.0009\phantom{*} \\
                        &                               &                                &                      (1.1342) &                      (-0.5164) &                               &                                &                       (1.0114) &                      (-0.3855) &                               &                                &                      (1.1342) &                               &                                &                       (1.0114)\smallskip \\
$|\beta_0^{Put,\tau}|$  &                               &                                &         \phantom{*}-0.0116*** &  \phantom{*}-0.004\phantom{**} &                               &                                &            \phantom{*}-0.0088* &  \phantom{*}-0.006\phantom{**} &                               &                                &         \phantom{*}-0.0116*** &                               &                                &            \phantom{*}-0.0088* \\
                        &                               &                                &         (-2.8726)\phantom{**} &                      (-0.7743) &                               &                                &                      (-1.9076) &                      (-1.0624) &                               &                                &         (-2.8726)\phantom{**} &                               &                                &                      (-1.9076)\smallskip \\
$|\beta_0^{Call,\tau}|$ &                               &                                &          \phantom{*}0.0135*** &            \phantom{*}0.0106** &                               &                                &             \phantom{*}0.0093* &   \phantom{*}0.0051\phantom{*} &                               &                                &          \phantom{*}0.0135*** &                               &                                &             \phantom{*}0.0093* \\
                        &                               &                                &          (3.2302)\phantom{**} &            (1.9642)\phantom{*} &                               &                                &                       (1.7852) &                       (0.8417) &                               &                                &          (3.2302)\phantom{**} &                               &                                &                       (1.7852)\smallskip \\
$|\beta_T^{Put,\tau}|$  &                               &                                &          \phantom{*}-1.3994** &             \phantom{*}-0.7813 &                               &                                &  \phantom{*}-1.1297\phantom{*} &  \phantom{*}-1.9528\phantom{*} &                               &                                &          \phantom{*}-1.3994** &                               &                                &  \phantom{*}-1.1297\phantom{*} \\
                        &                               &                                &          (-1.9889)\phantom{*} &                       (-0.624) &                               &                                &                      (-1.4831) &                      (-1.4826) &                               &                                &          (-1.9889)\phantom{*} &                               &                                &                      (-1.4831)\smallskip \\
$|\beta_T^{Call,\tau}|$ &                               &                                &            \phantom{*}1.522** &             \phantom{*}2.1924* &                               &                                &   \phantom{*}0.7055\phantom{*} &              \phantom{*}0.6187 &                               &                                &            \phantom{*}1.522** &                               &                                &   \phantom{*}0.7055\phantom{*} \\
                        &                               &                                &                      (2.1515) &                       (1.9348) &                               &                                &                       (0.8543) &                        (0.503) &                               &                                &                      (2.1515) &                               &                                &                       (0.8543) \\
\medskip\\
year FE                 &                            No &                             No &                            No &                             No &                           Yes &                            Yes &                            Yes &                            Yes &                            No &                             No &                            No &                           Yes &                            Yes &                            Yes \\
\medskip\\
Observations            &                         3,911 &                          3,911 &                         3,911 &                          3,911 &                         3,911 &                          3,911 &                          3,911 &                          3,911 &                         3,911 &                          3,911 &                         3,911 &                         3,911 &                          3,911 &                          3,911 \\
$R^2$                   &                        0.0097 &                         0.0094 &                        0.0081 &                         0.0105 &                        0.0423 &                         0.0412 &                         0.0405 &                         0.0416 &                        0.0097 &                         0.0094 &                        0.0081 &                        0.0423 &                         0.0412 &                         0.0405 \\
\bottomrule
\end{tabular}


==> tex/slope_regobL10.tex <==
\begin{tabular}{lcccccccc}
\toprule
{} &        \parboxc{c}{0.6cm}{(1)} &       \parboxc{c}{0.6cm}{(2)} &        \parboxc{c}{0.6cm}{(3)} &        \parboxc{c}{0.6cm}{(4)} &        \parboxc{c}{0.6cm}{(5)} &        \parboxc{c}{0.6cm}{(6)} &        \parboxc{c}{0.6cm}{(7)} &        \parboxc{c}{0.6cm}{(8)} \\
\midrule
one                     &          \phantom{*}-0.0147*** &         \phantom{*}-0.0148*** &          \phantom{*}-0.0226*** &          \phantom{*}-0.0226*** &                                &                                &                                &                                \\
                        &          (-8.0212)\phantom{**} &         (-7.2444)\phantom{**} &          (-8.9693)\phantom{**} &          (-8.1235)\phantom{**} &                                &                                &                                &                               \smallskip \\
$d \beta_K^{Put}$       &            \phantom{*}0.0151** &                               &                                &   \phantom{*}0.0258\phantom{*} &             \phantom{*}-0.0084 &                                &                                &   \phantom{*}0.0138\phantom{*} \\
                        &            (2.4667)\phantom{*} &                               &                                &                       (1.6074) &                       (-1.219) &                                &                                &                       (0.8572)\smallskip \\
$d \beta_K^{Call}$      &  \phantom{*}-0.0057\phantom{*} &                               &                                &              \phantom{*}0.0021 &              \phantom{*}0.0015 &                                &                                &  \phantom{*}-0.0003\phantom{*} \\
                        &                      (-0.8733) &                               &                                &                        (0.427) &                        (0.213) &                                &                                &                      (-0.0677)\smallskip \\
$d \beta_0^{Put}$       &   \phantom{*}0.0093\phantom{*} &                               &                                &   \phantom{*}0.0021\phantom{*} &   \phantom{*}0.003\phantom{**} &                                &                                &   \phantom{*}0.0034\phantom{*} \\
                        &                       (0.4439) &                               &                                &                       (0.0963) &                       (0.1441) &                                &                                &                       (0.1576)\smallskip \\
$d \beta_0^{Call}$      &  \phantom{*}-0.0122\phantom{*} &                               &                                &  \phantom{*}-0.0042\phantom{*} &  \phantom{*}-0.0152\phantom{*} &                                &                                &  \phantom{*}-0.0096\phantom{*} \\
                        &                      (-0.5861) &                               &                                &                      (-0.2007) &                      (-0.7313) &                                &                                &                      (-0.4575)\smallskip \\
$d \beta_T^{Call}$      &           \phantom{*}-6.9025** &                               &                                &   \phantom{*}1.1374\phantom{*} &  \phantom{*}-3.6594\phantom{*} &                                &                                &  \phantom{*}-5.7713\phantom{*} \\
                        &           (-2.0626)\phantom{*} &                               &                                &                       (0.1647) &                      (-1.0581) &                                &                                &                      (-0.8305)\smallskip \\
$d \beta_T^{Put}$       &             \phantom{*}6.9282* &                               &                                &              \phantom{*}5.5885 &   \phantom{*}3.6363\phantom{*} &                                &                                &   \phantom{*}9.371\phantom{**} \\
                        &                       (1.9165) &                               &                                &                        (0.773) &                       (0.9981) &                                &                                &                       (1.2942)\smallskip \\
$|\beta_K^{Put,0}|$     &                                &           \phantom{*}0.0183** &                                &  \phantom{*}-0.0198\phantom{*} &                                &  \phantom{*}-0.0092\phantom{*} &                                &  \phantom{*}-0.0237\phantom{*} \\
                        &                                &           (1.9896)\phantom{*} &                                &                      (-1.0136) &                                &                      (-0.9402) &                                &                      (-1.2153)\smallskip \\
$|\beta_K^{Call,0}|$    &                                &  \phantom{*}0.0002\phantom{*} &                                &  \phantom{*}-0.0073\phantom{*} &                                &  \phantom{*}-0.0104\phantom{*} &                                &  \phantom{*}-0.0099\phantom{*} \\
                        &                                &                      (0.0242) &                                &                      (-0.8509) &                                &                      (-0.9691) &                                &                      (-1.1636)\smallskip \\
$|\beta_0^{Put,0}|$     &                                &          \phantom{*}0.0877*** &                                &   \phantom{*}0.0246\phantom{*} &                                &  \phantom{*}-0.0245\phantom{*} &                                &  \phantom{*}-0.0406\phantom{*} \\
                        &                                &          (3.9215)\phantom{**} &                                &                       (0.8867) &                                &                      (-0.9027) &                                &                      (-1.3601)\smallskip \\
$|\beta_0^{Call,0}|$    &                                &         \phantom{*}-0.0895*** &                                &            \phantom{*}-0.0595* &                                &   \phantom{*}0.0146\phantom{*} &                                &   \phantom{*}0.0227\phantom{*} \\
                        &                                &         (-3.8866)\phantom{**} &                                &                      (-1.9345) &                                &                       (0.4756) &                                &                       (0.6741)\smallskip \\
$|\beta_T^{Put,0}|$     &                                &            \phantom{*}-1.2649 &                                &  \phantom{*}-1.9998\phantom{*} &                                &                      12.0082** &                                &   \phantom{*}5.0897\phantom{*} \\
                        &                                &                      (-0.267) &                                &                      (-0.2796) &                                &            (2.3601)\phantom{*} &                                &                       (0.7078)\smallskip \\
$|\beta_T^{Call,0}|$    &                                &             \phantom{*}1.9825 &                                &              \phantom{*}0.0133 &                                &            \phantom{*}-8.6985* &                                &             \phantom{*}-3.5462 \\
                        &                                &             (0.44)\phantom{*} &                                &                        (0.002) &                                &                      (-1.7954) &                                &                       (-0.527)\smallskip \\
$|\beta_K^{Put,\tau}|$  &                                &                               &  \phantom{*}-0.0009\phantom{*} &   \phantom{*}0.0139\phantom{*} &                                &                                &            \phantom{*}0.0187** &             \phantom{*}0.0218* \\
                        &                                &                               &                      (-0.1126) &                       (1.1526) &                                &                                &            (2.24)\phantom{***} &                       (1.8064)\smallskip \\
$|\beta_K^{Call,\tau}|$ &                                &                               &          \phantom{*}-0.0248*** &  \phantom{*}-0.0093\phantom{*} &                                &                                &  \phantom{*}-0.0136\phantom{*} &  \phantom{*}-0.0096\phantom{*} \\
                        &                                &                               &          (-2.905)\phantom{***} &                      (-1.0706) &                                &                                &                      (-1.4792) &                      (-1.1098)\smallskip \\
$|\beta_0^{Put,\tau}|$  &                                &                               &            \phantom{*}0.0948** &            \phantom{*}0.1109** &                                &                                &   \phantom{*}0.0286\phantom{*} &              \phantom{*}0.0556 \\
                        &                                &                               &            (1.9926)\phantom{*} &            (2.1223)\phantom{*} &                                &                                &                       (0.5208) &                        (0.955)\smallskip \\
$|\beta_0^{Call,\tau}|$ &                                &                               &  \phantom{*}-0.0751\phantom{*} &  \phantom{*}-0.0564\phantom{*} &                                &                                &  \phantom{*}-0.0367\phantom{*} &  \phantom{*}-0.0401\phantom{*} \\
                        &                                &                               &                      (-1.5189) &                      (-1.0275) &                                &                                &                      (-0.6004) &                      (-0.6267)\smallskip \\
$|\beta_T^{Put,\tau}|$  &                                &                               &   \phantom{*}9.7082\phantom{*} &                       20.1168* &                                &                                &             10.0962\phantom{*} &                       21.8326* \\
                        &                                &                               &                       (1.1037) &                       (1.8303) &                                &                                &                       (1.0299) &                       (1.8087)\smallskip \\
$|\beta_T^{Call,\tau}|$ &                                &                               &   \phantom{*}0.1102\phantom{*} &   \phantom{*}0.3527\phantom{*} &                                &                                &  \phantom{*}-7.4128\phantom{*} &            -12.7288\phantom{*} \\
                        &                                &                               &                       (0.0125) &                       (0.0321) &                                &                                &                      (-0.7175) &                      (-1.0205) \\
\medskip\\
year FE                 &                             No &                            No &                             No &                             No &                            Yes &                            Yes &                            Yes &                            Yes \\
\medskip\\
Observations            &                          3,366 &                         3,366 &                          3,366 &                          3,366 &                          3,366 &                          3,366 &                          3,366 &                          3,366 \\
$R^2$                   &                         0.0104 &                        0.0104 &                         0.0135 &                         0.0154 &                         0.0317 &                         0.0338 &                         0.0308 &                         0.0333 \\
\bottomrule
\end{tabular}


==> tex/yy_hbL1.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  in sample &     os(1) &     os(2) &     os(3) &     os(4) &     os(5) &    os(10) &    os(30) \\
year &            &           &           &           &           &           &           &           \\
\midrule
2001 &  -0.004783 & -0.004602 & -0.004446 & -0.003874 & -0.003825 & -0.003634 & -0.004037 & -0.003105 \\
2002 &  -0.004917 & -0.003890 & -0.003916 & -0.002863 & -0.002658 & -0.002522 & -0.002327 & -0.001855 \\
2003 &  -0.005175 & -0.004626 & -0.004907 & -0.003892 & -0.004847 & -0.004239 & -0.003547 & -0.003060 \\
2004 &  -0.004160 & -0.004437 & -0.004094 & -0.003673 & -0.003342 & -0.002547 & -0.002176 & -0.002608 \\
2005 &  -0.004217 & -0.002334 & -0.001395 & -0.001041 & -0.001323 & -0.000472 &  0.000997 &  0.001417 \\
2006 &  -0.006331 & -0.003818 & -0.002527 & -0.002413 & -0.002934 & -0.002482 & -0.000817 & -0.001261 \\
2007 &  -0.006604 & -0.004279 & -0.003184 & -0.002480 & -0.001897 & -0.001073 & -0.001645 &  0.000424 \\
2008 &  -0.005244 & -0.003172 & -0.002078 & -0.001110 & -0.001387 & -0.001208 & -0.001858 & -0.001910 \\
2009 &  -0.007972 & -0.006153 & -0.004609 & -0.003350 & -0.002953 & -0.002411 & -0.002991 & -0.002018 \\
2010 &  -0.004435 & -0.001681 & -0.001169 & -0.001374 & -0.001322 & -0.001225 & -0.001689 & -0.002570 \\
2011 &  -0.006006 & -0.003811 & -0.002780 & -0.002010 & -0.002029 & -0.001550 & -0.000889 & -0.000831 \\
2012 &  -0.005755 & -0.003348 & -0.002491 & -0.002408 & -0.001451 & -0.001880 & -0.001343 & -0.003082 \\
2013 &  -0.005917 & -0.003788 & -0.001947 & -0.001446 & -0.001660 & -0.001738 & -0.000273 &  0.001966 \\
2014 &  -0.006165 & -0.005133 & -0.004044 & -0.002659 & -0.002519 & -0.002278 & -0.001874 & -0.000618 \\
2015 &  -0.003574 & -0.002593 & -0.001740 & -0.002169 & -0.002449 & -0.001930 & -0.001960 & -0.001460 \\
2016 &  -0.008974 & -0.006204 & -0.005630 & -0.005378 & -0.005935 & -0.005153 & -0.006074 & -0.004224 \\
2017 &  -0.019786 & -0.015370 & -0.013399 & -0.012142 & -0.010441 & -0.009996 & -0.007884 & -0.002671 \\
2018 &  -0.009127 & -0.006039 & -0.004558 & -0.004432 & -0.004268 & -0.003971 & -0.002050 & -0.000746 \\
2019 &  -0.005665 & -0.004890 & -0.003559 & -0.003265 & -0.003460 & -0.002924 & -0.002779 & -0.003363 \\
\bottomrule
\end{tabular}


==> tex/yy_hbL10.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  in sample &     os(1) &     os(2) &     os(3) &     os(4) &     os(5) &    os(10) &    os(30) \\
year &            &           &           &           &           &           &           &           \\
\midrule
2001 &  -0.004783 & -0.004602 & -0.004446 & -0.003874 & -0.003825 & -0.003634 & -0.004037 & -0.003105 \\
2002 &  -0.004917 & -0.003890 & -0.003916 & -0.002863 & -0.002658 & -0.002522 & -0.002327 & -0.001855 \\
2003 &  -0.005175 & -0.004626 & -0.004907 & -0.003892 & -0.004847 & -0.004239 & -0.003547 & -0.003060 \\
2004 &  -0.004160 & -0.004437 & -0.004094 & -0.003673 & -0.003342 & -0.002547 & -0.002176 & -0.002608 \\
2005 &  -0.004217 & -0.002334 & -0.001395 & -0.001041 & -0.001323 & -0.000472 &  0.000997 &  0.001417 \\
2006 &  -0.006331 & -0.003818 & -0.002527 & -0.002413 & -0.002934 & -0.002482 & -0.000817 & -0.001261 \\
2007 &  -0.006604 & -0.004279 & -0.003184 & -0.002480 & -0.001897 & -0.001073 & -0.001645 &  0.000424 \\
2008 &  -0.005244 & -0.003172 & -0.002078 & -0.001110 & -0.001387 & -0.001208 & -0.001858 & -0.001910 \\
2009 &  -0.007972 & -0.006153 & -0.004609 & -0.003350 & -0.002953 & -0.002411 & -0.002991 & -0.002018 \\
2010 &  -0.004435 & -0.001681 & -0.001169 & -0.001374 & -0.001322 & -0.001225 & -0.001689 & -0.002570 \\
2011 &  -0.006006 & -0.003811 & -0.002780 & -0.002010 & -0.002029 & -0.001550 & -0.000889 & -0.000831 \\
2012 &  -0.005755 & -0.003348 & -0.002491 & -0.002408 & -0.001451 & -0.001880 & -0.001343 & -0.003082 \\
2013 &  -0.005917 & -0.003788 & -0.001947 & -0.001446 & -0.001660 & -0.001738 & -0.000273 &  0.001966 \\
2014 &  -0.006165 & -0.005133 & -0.004044 & -0.002659 & -0.002519 & -0.002278 & -0.001874 & -0.000618 \\
2015 &  -0.003574 & -0.002593 & -0.001740 & -0.002169 & -0.002449 & -0.001930 & -0.001960 & -0.001460 \\
2016 &  -0.008974 & -0.006204 & -0.005630 & -0.005378 & -0.005935 & -0.005153 & -0.006074 & -0.004224 \\
2017 &  -0.019786 & -0.015370 & -0.013399 & -0.012142 & -0.010441 & -0.009996 & -0.007884 & -0.002671 \\
2018 &  -0.009127 & -0.006039 & -0.004558 & -0.004432 & -0.004268 & -0.003971 & -0.002050 & -0.000746 \\
2019 &  -0.005665 & -0.004890 & -0.003559 & -0.003265 & -0.003460 & -0.002924 & -0.002779 & -0.003363 \\
\bottomrule
\end{tabular}


==> tex/yy_obL1.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  in sample &     os(1) &     os(2) &     os(3) &     os(4) &     os(5) &    os(10) &    os(30) \\
year &            &           &           &           &           &           &           &           \\
\midrule
2001 &   0.071162 & -0.004265 & -0.000556 & -0.005337 & -0.003823 & -0.005868 & -0.016019 & -0.011827 \\
2002 &   0.072826 &  0.000716 & -0.001431 & -0.003651 & -0.003973 & -0.003245 & -0.015469 & -0.008309 \\
2003 &   0.055175 & -0.000855 & -0.001630 & -0.002696 & -0.004203 & -0.003485 & -0.017729 & -0.010275 \\
2004 &   0.058692 &  0.001210 &  0.001102 &  0.000028 & -0.000805 & -0.000015 & -0.011189 & -0.005328 \\
2005 &   0.053131 &  0.002849 &  0.000159 & -0.002370 & -0.002197 & -0.001403 & -0.010007 & -0.008187 \\
2006 &   0.054298 &  0.002231 & -0.001392 & -0.003907 & -0.001497 &  0.001053 & -0.011035 & -0.009993 \\
2007 &   0.061071 &  0.001399 & -0.006743 & -0.003937 & -0.004626 & -0.004335 & -0.011875 & -0.009710 \\
2008 &   0.082940 &  0.010590 &  0.003192 & -0.000956 & -0.004017 & -0.000571 & -0.008149 & -0.008228 \\
2009 &   0.060977 &  0.009341 &  0.002277 &  0.000925 & -0.000138 &  0.001430 & -0.005909 & -0.005567 \\
2010 &   0.053150 &  0.009187 &  0.002491 &  0.001649 &  0.001097 & -0.000489 & -0.003240 & -0.005756 \\
2011 &   0.065878 &  0.004990 & -0.004515 & -0.002897 & -0.002754 & -0.003526 & -0.006932 & -0.005597 \\
2012 &   0.057473 &  0.007212 &  0.000867 & -0.002183 & -0.000753 & -0.000211 & -0.002961 & -0.005162 \\
2013 &   0.057796 &  0.010112 &  0.004285 & -0.001162 & -0.001491 &  0.000672 & -0.000667 & -0.004380 \\
2014 &   0.054635 &  0.008001 &  0.003957 &  0.000624 & -0.001570 & -0.000732 & -0.002376 & -0.005933 \\
2015 &   0.062128 &  0.010434 &  0.002461 & -0.000217 &  0.000335 &  0.000500 & -0.001180 & -0.004381 \\
2016 &   0.066631 &  0.009406 &  0.001558 & -0.000466 & -0.001176 & -0.000930 & -0.003150 & -0.004626 \\
2017 &   0.057418 &  0.008205 &  0.001517 &  0.000780 &  0.000009 &  0.000658 & -0.003479 & -0.007543 \\
2018 &   0.072796 &  0.003594 & -0.001685 & -0.002398 & -0.004873 & -0.002935 & -0.003104 & -0.005273 \\
2019 &   0.065878 &  0.006836 & -0.002050 & -0.001194 & -0.001230 & -0.001120 & -0.002725 & -0.005574 \\
\bottomrule
\end{tabular}


==> tex/yy_obL10.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  in sample &     os(1) &     os(2) &     os(3) &     os(4) &     os(5) &    os(10) &    os(30) \\
year &            &           &           &           &           &           &           &           \\
\midrule
2001 &   0.066575 & -0.007963 & -0.003727 & -0.008190 & -0.006461 & -0.008541 & -0.017974 & -0.014121 \\
2002 &   0.066856 & -0.002923 & -0.004664 & -0.006456 & -0.006470 & -0.005709 & -0.016307 & -0.010194 \\
2003 &   0.050851 & -0.003816 & -0.003875 & -0.004621 & -0.005902 & -0.005110 & -0.018396 & -0.011073 \\
2004 &   0.054747 & -0.001057 & -0.000607 & -0.001631 & -0.002233 & -0.001521 & -0.011533 & -0.005807 \\
2005 &   0.049639 &  0.000929 & -0.001320 & -0.003630 & -0.003032 & -0.002439 & -0.009933 & -0.008294 \\
2006 &   0.050999 &  0.000258 & -0.002890 & -0.004881 & -0.002383 & -0.000195 & -0.010886 & -0.010054 \\
2007 &   0.057466 & -0.000602 & -0.007887 & -0.005107 & -0.005075 & -0.005427 & -0.011720 & -0.010170 \\
2008 &   0.079346 &  0.007791 &  0.001685 & -0.002740 & -0.005126 & -0.001974 & -0.009310 & -0.009091 \\
2009 &   0.057564 &  0.006875 &  0.000776 & -0.000346 & -0.001511 & -0.000366 & -0.006603 & -0.005122 \\
2010 &   0.049717 &  0.008078 &  0.001941 &  0.001006 &  0.000292 & -0.001261 & -0.003448 & -0.005741 \\
2011 &   0.062280 &  0.003042 & -0.005923 & -0.004437 & -0.004458 & -0.005516 & -0.007797 & -0.006365 \\
2012 &   0.054373 &  0.005958 &  0.000015 & -0.002668 & -0.001153 & -0.000508 & -0.003025 & -0.005395 \\
2013 &   0.054874 &  0.008417 &  0.003258 & -0.001887 & -0.002442 & -0.000424 & -0.001421 & -0.004673 \\
2014 &   0.052137 &  0.006652 &  0.003276 &  0.000360 & -0.001941 & -0.001204 & -0.002815 & -0.006090 \\
2015 &   0.059496 &  0.009245 &  0.002060 & -0.000572 & -0.000037 &  0.000069 & -0.001524 & -0.004299 \\
2016 &   0.063560 &  0.009331 &  0.001929 & -0.000130 & -0.001100 & -0.001134 & -0.003246 & -0.004286 \\
2017 &   0.055868 &  0.006869 &  0.000914 &  0.000325 & -0.000477 &  0.000133 & -0.003720 & -0.007492 \\
2018 &   0.073691 &  0.003264 & -0.001797 & -0.002883 & -0.005033 & -0.003085 & -0.003133 & -0.004988 \\
2019 &   0.064873 &  0.006292 & -0.000756 & -0.000226 & -0.001077 & -0.000520 & -0.002273 & -0.006027 \\
\bottomrule
\end{tabular}

